Deep Learning in Human Activity Recognition with Wearable Sensors: A Review on Advances

Mobile and wearable devices have enabled numerous applications, including activity tracking, wellness monitoring, and human--computer interaction, that measure and improve our daily lives. Many of these applications are made possible by leveraging the rich collection of low-power sensors found in many mobile and wearable devices to perform human activity recognition (HAR). Recently, deep learning has greatly pushed the boundaries of HAR on mobile and wearable devices. This paper systematically categorizes and summarizes existing work that introduces deep learning methods for wearables-based HAR and provides a comprehensive analysis of the current advancements, developing trends, and major challenges. We also present cutting-edge frontiers and future directions for deep learning-based HAR.

==> 1-intro.tex <==
\section{Introduction} 
\label{sec:intro}


Since the first Linux-based smartwatch was presented in 2000 at the IEEE International Solid-State Circuits Conference (ISSCC) by Steve Mann, who was later hailed as the ``father of wearable computing," the 21st century has witnessed a rapid growth of wearables. For example, as of January 2020, 21\% of adults in the United States, most of whom are not opposed to sharing data with medical researchers, own a smartwatch. \cite{techcrunch2020}. 
 
 
In addition to being fashion accessories, wearables provide unprecedented opportunities for monitoring human physiologic signals and facilitating natural and seamless interaction between humans and machines. Wearables integrate low-power sensors that allow them to sense movement and other physiologic signals such as heart rate, temperature, blood pressure, and electrodermal activity. The rapid proliferation of wearable technologies and advancements in sensing analytics have spurred on the growth of human activity recognition (HAR). %Human activity recognition (HAR) has become more robust and practical than ever before due to the proliferation of wearable technologies (enabling a plethora of data to be collected to train models) and rapid advancements in 
% artificial intelligence.
%sensing analytic methods.
As a general understanding of the HAR shown in Fig. \ref{fig:signal}, HAR has drastically improved the quality of service in a broad range of applications spanning healthcare, entertainment, gaming, industry, and lifestyle, among others. 
% \textcolor{red}{For example, step counts during inpatient recovery after cancer surgery was shown to be an accurate predictor of 30- and 60-day hospital readmission~\cite{Low2017}}. 
Market analysts from Meticulous Research\textregistered  \cite{wearable_forecast} forecast that the global wearable devices market will grow at a compound annual growth rate of 11.3\% from 2019, reaching \$62.82 billion by 2025, with companies like Fitbit\textregistered, Garmin\textregistered, and Huawei Technologies\textregistered investing more capital into the area.


In the past decade, deep learning (DL) has revolutionized traditional machine learning (ML) and brought about improved performance in many fields, including image recognition, object detection, speech recognition, and natural language processing.
DL has improved the performance and robustness of HAR, speeding its adoption and application to a wide range of wearable sensor-based applications.
% 
%\zs{The reason behind the overwhelming performance of DL is two-folded -- its automatic feature extraction capability and the capability of modeling complex distribution. Traditional machine learning algorithms usually call for manual feature engineering which unavoidably requires expert domain knowledge and large amount of human efforts. When using a deep neural network, the representative features can be learnt automatically from raw data in a hierarchical manner, thus eliminating the challenging stage of feature engineering. Besides, deep neural networks contain a large number of parameters, which allows learning from large-scale datasets in order to model more complex distributions than traditional ML approaches and shallow neural networks. Due to the extraordinary expressive power and capability of utilizing large datasets, we have witnessed an exponential increase in DL-based HAR applications.}
There are two key reasons why DL is effective for many applications. First, DL methods are able to directly learn robust features from raw data for specific applications, whereas features generally need to be manually extracted or engineered in traditional ML approaches, which usually requires expert domain knowledge and a large amount of human effort. Deep neural networks can efficiently learn representative features from raw signals with little domain knowledge. Second, deep neural networks have been shown to be universal function approximators, capable of approximating almost any function given a large enough network and sufficient observations~\cite{cybenko1989approximation, scafer2006approximator, zhou2020universality}. Due to this expressive power, DL has seen an exponential growth in HAR-based applications.


% Deep models introduce layered architectures for data representation~\cite{deng2014tutorial}. 

Despite promising results in DL, there are still many challenges and problems to overcome, leaving room for more research opportunities. We present a review on deep learning in HAR with wearable sensors and elaborate on ongoing challenges, obstacles, and future directions in this field.



\begin{figure*}[tbh]
    \centering
    \captionsetup{justification=centering}
    \subfloat[]{
    \includegraphics[width=0.38\linewidth]{final_images/wearablesSharesOnPurpose.png}
    \label{fig:distribution}}
    \subfloat[]{
    \includegraphics[width=0.28\linewidth,height=4.1cm]{final_images/sensors2.png}
    \label{fig:signal}} 
    \subfloat[]{
    \includegraphics[width=0.32\linewidth]{final_images/wearablesSharesOnBodyPart.png}
    \label{fig:wearables_shares_on_body_part}}
    \caption{Wearable devices and their application. (a) Distribution of wearable applications~\cite{wearable_database}. (b) Typical wearable devices. (c) Distribution of wearable devices placed on common body areas \cite{wearable_database}.}
\end{figure*}



% passive sensors are defined as sensors receiving and processing signals coming for the environment.
% \textcolor{red}{Technical challenge:}
%
% From the perspective of sensor adaptability for HAR, it is common that the widely accepted wearable sensors are not able to provide valid information for inferring human activities, since their captured data can have little informative modality. (Very confusing sentence "sensor adaptability" , "informative modality". Perhaps rephrase)

% The inherent reason of their being more accepted by users \textcolor{red}{(what is the inherent reason of these sensors being widely used, despite their deficiencies?)} decides their lower capability toward the goal to infer or predict human activity. 

% That’s also embodied by the fact that in HAR studies, the ground truth is often obtained by manually observing and labeling the video recording, which represents the vision modality. However, while cyber security experts may disagree, most humans can hardly distinguish the exact activity visually from the inertial sensor data. In this case, interpreting HAR from measurements of the inertial sensor is an inherently difficult problem, which can be only accomplished by specifically targeting certain symbolic icons of human behaviors. 

% If we compare it with image recognition field, we can find that, when compared with the complexity of tasks and astonishingly high performance that image/video recognition has achieved, the performance of high-level complex human activity recognition from wearable sensors other than camera is quite preliminary and far from ready to be deployed in real life. 
 




% \textbf{Topic: Multi-modality}

% According to ensemble theory, multiple informatively weak sensors can form a strong perception method. This lays the foundation of this study combining multiple modalities for human activity recognition. 


% \begin{figure}
% \centering
%   \includegraphics[width=0.38 \columnwidth]{img/modality_rank.jpg}
%   \caption{modality rank}~\label{fig:modality}
% \end{figure}


Specifically, we focus on the recognition of physical activities, including locomotion, activities of daily living (ADL), exercise, and factory work. While DL has shown a lot of promise in other applications, such as ambient scene analysis, emotion recognition, or subject identification, we focus on HAR. Throughout this work, we present brief and high-level summaries of major DL methods that have significantly impacted wearable HAR. For more details about specific algorithms or basic DL, we refer the reader to original papers, textbooks, and tutorials~\cite{Goodfellow-et-al-2016, Sutton2018}.
\change{
Our contributions are summarized as followings.}

\begin{enumerate}[label=(\roman*)]

\item \change{Firstly, we give an overview of the background of the human activity recognition research field, including the traditional and novel applications where the research community is focusing on, the sensors that are utilized in these applications, as well as widely-used publicly available datasets.}
% 
\item \change{Then after briefly introducing the popular mainstream deep learning algorithms, we give a review of the relevant papers over the years using deep learning in human activity recognition using wearables. We categorize the papers in our scope according to the algorithm (autoencoder, CNN, RNN, etc). In addition, we compare different DL algorithms in terms of the accuracy on the public dataset, pros and cons, deployment, and high-level model selection criteria.} 
% 
\item \change{We provide a comprehensive review on the current issues, challenges, and opportunities in the HAR domain and the latest advancements towards solutions. At last, honorably and humbly, we make our best to shed light on the possible future directions with the hope to benefit students and young researchers in this field.
}
 
\end{enumerate}

% \yx{need update in the end} 


\section{Methodology} 
\label{sec:method}


\subsection{Research Question} 
\label{sec:question}

\changezs{In this work, we propose several major research questions, including $\mathsf{Q1:}$ what the real-world applications of HAR, mainstream sensors, and major public datasets are in this field, $\mathsf{Q2:}$ what deep learning approaches are employed in the field of HAR and what pros and cons each of them has, and $\mathsf{Q3:}$ what challenges we are facing in this field and what opportunities and potential solutions we may have. In this work, we review the state-of-the-art work in this field and present our answers to these questions.}


This article is organized as follows:
\changezs{
% We first propose the research question and define our research scope in Section~\ref{sec:method}. Then 
We compare this work with related existing review work in this field in Section~\ref{sec:related}.} Section~\ref{sec:applications} introduces common applications for HAR. Section~\ref{sec:sensor} summarizes the types of sensors commonly used in HAR. Section~\ref{sec:dataset} summarizes major datasets that are commonly used to build HAR applications. Section~\ref{sec:deeplearning} introduces the major works in DL that contribute to HAR. Section~\ref{sec:challenges} discusses major challenges, trends, and opportunities for future work. We provide concluding remarks in Section~\ref{sec:conclusions}.




\subsection{Research Scope} 
\label{sec:scope}



% \section{Scope of this paper} \label{sec:scope}

%
% \begin{figure}
% \centering
%   \includegraphics[width=.6\columnwidth]{img/consort.pdf}
%   \caption{Consort diagram.}~\label{fig:signal}
% \end{figure}

\change{Although this work is not aiming for a systematic survey of existing research work, we would still like to introduce our research scoping method in this section to provide an overview of this review work.}
\change{%Our inclusion criteria are:
We searched in Google Scholar with meta-keywords A) "Human activity recognition", "motion recognition", "locomotion recognition", "hand gesture recognition", "wearable" B) "Deep learning", "autoencoder" (alternatively "auto-encoder"), "deep belief network", "convolutional neural network" (alternatively "convolution neural network"), "recurrent neural network", "LSTM", "recurrent neural network", "generative adversarial network" (alternatively "GAN"), "reinforcement learning", "attention", "deep semi-supervised learning", and "graph neural network". We used an AND rule to get combinations of the above meta-keywords A) and B). For each combination, we obtained top 200 search results ranked by relevance. We didn't consider any patent or citation-only search result (no content available online).}

% \item Since the result from the search engines does not contain latest published works due to relatively low exposure and citation, we focus on the latest publications in the ubiquitous computing area including IMWUT, CHI Proceedings, SenSys Proceedings, MDPI Sensors, MDPI Informatics, and IEEE Sensors in order to follow the latest trend. 
% \end{enumerate}

% \change{We include works from 1) and 2). In the challenge and opportunity section, to cover the exploratory works focusing on the challenges of the wearable-based HAR, we also consider the works approaching challenging topics including data quality, data label acquisition, model generalizability, etc, with machine learning or deep learning.}

% \textcolor{red}{(Writing needs to be improved) } 
% \textcolor{orange}{already changed the word, please check whether this is ok}
\change{There are several exclusion criteria to build the database of the paper we reviewed.
% \begin{enumerate}[label=(\roman*)]
% \item 
First of all, we omitted image or video-based HAR works, such as~\cite{kiran2021fusion}, since there is a huge body of work in the computer vision community and the method is significantly different from sensor-based HAR. 
% We don’t include image or video based HAR works, such as~\cite{kiran2021fusion}, since there is a rather huge body of work in the computer vision community and the method is significantly different from sensor-based HAR. 
% \item 
Secondly, we removed the papers using environmental sensors or systems assisted by environmental sensors such as WiFi- and RFID- based HAR. 
% We remove the papers using environmental sensors or using systems assisted by environmental sensors such as WiFi- and RFID- based HAR. 
% \item 
Thirdly, we removed the papers with minor algorithmic advancements based on prior works. We aim to present the technical progress and algorithmic achievements in HAR, so we avoid presenting works that do not stress the novelty of methods.
In the end, as the field of wearable-based HAR is becoming excessively popular and a numerous number of papers are coming out. It is not a surprise to find that many papers share rather similar approaches and it is almost impossible and less meaningful to cover all of them. Therefore, we select, categorize, and summarize representative works to present in this review paper. We adhere to the goal of our work throughout the whole paper that is to give an overall introduction to new researchers entering this field and present the cutting-edge research challenges and opportunities.}







% We remove the papers with little algorithmic advancements based on prior works. Our aim is to present the technical progress and algorithmic achievements in HAR, so we try to avoid presenting works which do not stress on the novelty of methods.}

% \end{enumerate}



\subsection{Taxonomy of Human Activity Recognition} 
\label{sec:scope}

\change{
In order to obtain a straightforward understanding of the hierarchies under the tree of HAR, we illustrate the taxonomy of HAR as shown in Fig.~\ref{fig:taxonomy}. We categorized existing HAR works into four dimensions: \textbf{sensor}, \textbf{application}, \textbf{DL approach}, and \textbf{challenge}. There are basically two kinds of sensors: physical sensors and physiological sensors. Physical sensors include Inertial Measurement Unit (IMU), piezoelectric sensor, GPS, wearable camera, etc. Some exemplary physiological sensors are electromyography (EMG) and photoplethysmography (PPG), just to name a few. 
In terms of the applications of HAR systems, we categorized them into healthcare, fitness\&
lifestyle, and Human Computer Interaction (HCI). Regarding the DL algorithm, we introduce six approaches, including autoencoder (AE), Deep Belief Network (DBN), Convolutional Neural Network, Recurrent Neural Network (including Long Short-Term Memory (LSTM) and Gated Recurrent Units (GRUs)), Generative Adversarial Network (GAN), and Deep Reinforcement Learning (DRL). In the end, we discuss the challenges our research community is facing and the state-of-the-art works are coping with, also shown in Fig.~\ref{fig:taxonomy}.
}
% 
% \end{paracol}
\begin{figure*}[tb]
\centering
\captionsetup{justification=centering}
  \includegraphics[width= 0.95\linewidth]{img/HAR_taxonomy.pdf}
  \caption{\change{Taxonomy of Deep Learning-based Human Activity Recognition with Wearables.}}
  \label{fig:taxonomy}
\end{figure*}
% \begin{paracol}{2}
% \linenumbers
% \switchcolumn


% \begin{figure*}
% \centering
%   \includegraphics[width=\columnwidth]{img/HAR_taxonomy.pdf}
%   \caption{Taxonomy of Human Activity Recognition.}~\label{fig:taxonomy}
% \end{figure*}



% \change{Our inclusion criteria are:
% % \begin{enumerate}[label=(\roman*)]
% % \item 
% We search in Google Scholar with meta-keywords A) “Human activity recognition”, ”motion recognition”, ”locomotion recognition”, "hand gesture recognition", “wearable” B) “Deep learning”, “autoencoder” (“auto-encoder”), "deep belief network", “convolutional neural network” (“convolution neural network”), “recurrent neural network”, "LSTM", “recurrent neural network”, "generative adversarial network" ("GAN"), "reinforcement learning", "attention", "deep semi-supervised learning", and "graph neural network". We use an AND rule to get combinations of the above meta-keywords A) and B). For each combination, we obtain top 200 search results ranked by relevance. We cancelled out the checkbox for "including patents" and "including citations" to exclude patents and citation-only results.}

% % \item Since the result from the search engines does not contain latest published works due to relatively low exposure and citation, we focus on the latest publications in the ubiquitous computing area including IMWUT, CHI Proceedings, SenSys Proceedings, MDPI Sensors, MDPI Informatics, and IEEE Sensors in order to follow the latest trend. 
% % \end{enumerate}

% \change{The review includes works from 1) and 2). In the challenge and opportunity section, to cover the exploratory works focusing on the challenges of the wearable-based HAR, we also consider the works approaching challenging topics including data quality, data label acquisition, model generalizability, etc, with machine learning or deep learning.}

% \change{Our exclusion criteria are:
% % \begin{enumerate}[label=(\roman*)]
% % \item 
% We don’t include image or video based HAR works, since there’s a rather huge body of work in the computer vision community and the method is significantly different from sensor-based HAR. 
% % \item 
% We remove the papers using environmental sensors or using systems assisted by environmental sensors such as WiFi- and RFID- based HAR. 
% % \item 
% We remove the papers with little algorithmic advancements based on prior works. Our aim is to present the technical progress and algorithmic achievements in HAR, so we try to avoid presenting works which do not stress on the novelty of methods.}

% \end{enumerate}


==> 2-related.tex <==
\section{Related Work} 
\label{sec:related}

\change{
There are some existing review papers in the literature for deep learning approaches for sensor-based human activity recognition~\cite{wang2019deep,nweke2018deep,chen2021deep,ramanujam2021human}.}
% 
\change{
Nweke \etal accentuated the advancements in deep learning models by proposing a taxonomy of generative, discriminative, and hybrid methods along with further explorations for the advantages and limitations up to year 2018~\cite{nweke2018deep}. 
% 
Similarly, Wang \etal conducted a thorough analysis on different sensor-based modalities, deep learning models, and their respective applications up to year 2017~\cite{wang2019deep}. 
% 
However, in recent years, due to huge advancements in the availability and computational power of computing resources and in cutting-edge deep learning techniques, applied deep learning area has been revolutionized and reached all-time-high performance in the field of sensor-based human activity recognition. Therefore, we aim at presenting the most recent advances and most exciting achievements that took place in the community in a timely manner to our readers.}


\change{In another work, Chen \etal provided the community a comprehensive review which has done an in-depth analysis of the challenges/opportunities for deep learning in sensor-based HAR and proposed a new taxonomy for the challenges ahead of the activity recognition systems \cite{chen2021deep}. 
% 
In contrast, we view our work as more of a gentle introduction of this field to students and novices in the way that our literature review provides the community with a detailed analysis on most recent state-of-the-art deep learning architectures (i.e., CNN, RNN, GAN, Deep Reinforcement Learning, and hybrid models) and their respective pros and cons on HAR benchmark datasets. At the same time, we distill our knowledge and experience from our past works in this field and present the challenges and opportunities from a different viewpoint.
% 
Another recent work was presented by Ramanujam \etal, in which they categorized the deep learning architectures in CNN, LSTM, and hybrid methods and conducted an in-depth analysis on the benchmark datasets~\cite{ramanujam2021human}. 
% 
Compared with their work, our paper pays more attention to the most recent cutting-edge deep learning methods applied on HAR on-body sensory data, such as GAN and DRL. We also provide both new learners and experienced researchers with a profound resource in terms of model comparison, model selection and model deployment.
% 
% as a resource assisting with model selection/deployment with most recent privacy aware measures e.g., blockchain. 
% 
% 
% However, due to ubiquity of advanced low power sensors in wearable devices in recent years, this review paper failed to bring up the challenge of unlabeled data annotation which is the bottleneck to DL systems in this field due to the reason that DL approaches are reliant on large amounts of sensory data to perform acceptably in HAR platforms.
In a nutshell, our review has done a thorough analysis of most up-to-date deep learning architectures applied on various wearable sensors, elaborated on their respective applications and compared performances on public datasets. What's more, we attempt to cover the most recent advances in resolving the challenges and difficulties and shed light on possible research opportunities. 
}

% \textcolor{red}{(Farzad, also this paper: Deep learning for sensor-based activity recognition: A survey, and this: A Survey of Human Activity Recognition in Smart Homes Based on IoT Sensors Algorithms: Taxonomies, Challenges, and Opportunities with Deep Learning, and Deep Learning for Sensor-based Human Activity Recognition: Overview, Challenges, and Opportunities)
% } done

% \textcolor{red}{is this covered? Human Activity Recognition With Smartphone and Wearable Sensors Using Deep Learning Techniques: A Review https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9389739}
% done
% \vspace{10pt}


==> 3-app.tex <==
\section{Human Activity Recognition Overview}

\subsection{Applications} \label{sec:applications}
% \yx{edited. Need proofread}
% In this section, we introduce and summarize the major areas and applications that HAR has impacted. We first give a brief introduction, and then illustrate each of the areas with concrete applications and examples that HAR has improved or enabled.
%Since deep learning techniques are quickly unlocking more application scenarios that were previously attempted by traditional machine learning methods, we'll not only include the existing work using deep learning in this section, but also discuss those pivotal applications using the traditional machine learning and data mining techniques in general. (A bit wordy and unnecessary. consider removing)
%

In this section, we illustrate the major areas and applications of wearable devices in HAR. Fig.~\ref{fig:distribution}, taken from the wearable technology database~\cite{wearable_database}, breaks down the distribution of application types of 582 commercial wearables registered since 2015~\cite{wearable_database}. The database suggests that wearables are increasing in popularity and will impact people's lives in several ways particularly in applications ranging from fitness and lifestyle to medical and human-computer interaction.






\subsubsection{Wearables in Fitness and Lifestyle}
% \subsubsection{Wearables in Fitness and Wellness}
% \subsection{Daily Life Logging}



% \textbf{Physical Activity Recognition:}
% Physical activities include, but are not limited to, sitting, walking, laying down, going upstairs or downstairs, jogging, running~\cite{Physical_activity_recognition}. The duration and intensity of an individual's physical activities throughout the day can reveal and, in turn, reshape daily habits and health conditions \cite{physical_activity_health}. For example, regular physical activities can decrease the risk of many chronic diseases like obesity, diabetes, cardiovascular, and improve mental health \cite{mobility_chronicdisease}. 
% Moreover, individuals' modes of transportation, such as walking, bicycling, or driving, are also of great interest to physicians, healthcare providers, and users themselves. Being aware of daily locomotion and transportation patterns can provide physicians with the necessary information to better understand patients' conditions, while also encouraging users to engage in more exercise and lead to self-regulatory behavioral change~\cite{Fitness_Behavior_Change}. Due to the above reasons, physical activity recognition is among the most prolific HAR applications~\cite{cnnhar2014, cnn2015smc, cnn2015mm, cnn2016expert, cnn2017bigcomp, benchmarkingSHL, SHLIndRNN, TMD2018, Attention_CNN_weaklylabel}.

% Based on physical activity recognition, energy expenditure can be estimated, which represents the amount of energy people burn to support metabolism and daily activities~\cite{Zhu2015Using}. Energy expenditure estimation can be estimated and presented to users in smartphones and smartwatches, or dedicated products such as Fitbit~\cite{fitbit}.



% \yx{edited. Need proofread}
Physical activity involves activities such as sitting, walking, laying down, going up or down stairs, jogging, and running~\cite{Physical_activity_recognition}. 
Regular physical activity is increasingly being linked to reduction in risk for many chronic diseases, such as obesity, diabetes, and cardiovascular disease, and has been shown to improve mental health \cite{mobility_chronicdisease}. 
The data recorded by wearable devices during these activities include plenty of information, such as duration and intensity of activity, which further reveal an individual's daily habits and health conditions \cite{physical_activity_health}. 
For example, dedicated products such as Fitbit~\cite{fitbit} can estimate and record energy expenditure on smart devices, which can further serve as an important step in tracking personal activity and preventing chronic diseases~\cite{Zhu2015Using}. Moreover, there has been evidence of the association between modes of transport (motor vehicle, walking, cycling, and public transport) and obesity-related outcomes \cite{transport_medical}.
Being aware of daily locomotion and transportation patterns can provide physicians with the necessary information to better understand patients' conditions and also encourage users to engage in more exercise to promote behavior change~\cite{Fitness_Behavior_Change}. Therefore, the use of wearables in fitness and lifestyle has the potential to significantly advance one of the most prolific aspects of HAR applications~\cite{cnnhar2014, cnn2015smc, cnn2015mm, cnn2016expert, cnn2017bigcomp, benchmarkingSHL, SHLIndRNN, TMD2018, Attention_CNN_weaklylabel}.

Energy (or calorie) expenditure (EE) estimation has grown to be an important reason why people care to track their personal activity. Self-reflection and self-regulation of one's own behavior and habit has been an important factor in designing interventions that prevent chronic diseases such as obesity, diabetes, and cardiovascular diseases. %Accurate and real-time EE estimation using wearable sensors is a challenge primarily due to....

\subsubsection{Wearables in Healthcare and Rehabilitation}

HAR has greatly impacted the ability to diagnose and capture pertinent information in healthcare and rehabilitation domains. 
By tracking, storing, and sharing patient data with medical institutions, wearables have become instrumental for physicians in patient health assessment and monitoring. 
% 
Specifically, several works have introduced systems and methods for monitoring and assessing  Parkinson disease (PD) symptoms~\cite{parkinson2015, parkinson2016, parkinson2017, parkinson2018, parkinson2018_2, parkinson_augmentation}. 
% 
\change{Pulmonary disease, such as Chronic Obstructive Pulmonary Disease (COPD), asthma, and Covid-19, is one of leading causes of morbidity and mortality. Some recent works use wearables to detect cough activity, a major symptom of pulmonary diseases~\cite{Listen2Cough, mcc,CoughBuddy2021Nemati,zhang2021coughtrigger}}
% 
Other works have introduced methods for monitoring stroke in infants using wearable accelerometers~\cite{infant_stroke} and methods for assessing depressive symptoms utilizing wrist-worn sensors~\cite{depression}.
% 
In addition,  detecting muscular activities and hand motions using electromyography (EMG) sensors has been widely applied to enable improved prostheses control for people with missing or damaged limbs \cite{EMG_review, EMG_armband, EMG_prosthese, EMG_prosthese2}.

% \textcolor{red}{Restless legs syndrome (RLS)}

% The cardinal motor symptoms of PD are bradykinesia, rigidity, tremor, and postural instability.

% tremor \cite{pakinson2018_2}


\subsubsection{Wearables in Human Computer Interaction (HCI)}

% \yx{edited. Need proofread}
Modern wearable technology in HCI has provided us with flexible and convenient methods to control and communicate with electronics, computers, and robots. 
For example, a wrist-worn wearable outfitted with an inertial measurement unit (IMU) can easily detect the wrist shaking~\cite{seg_cnn, dynamichandgesturerecognition, fingerping} to control smart devices to skip a song by shaking the hand, instead of bringing up the screen, locating, and pushing a button. 
%
Furthermore, wearable devices have played an essential role in many HCI applications in entertainment systems and immersive technology.
One example filed is augmented reality (AR) and virtual reality (VR), which has changed the way we interact and view the world. Thanks to accurate activity, gesture, and motion detection from wearables, these applications could induce feelings of cold or hot weather by providing an immersive experience by varying the virtual environment and could enable more realistic interaction between the human and virtual objects~\cite{EMG_review, EMG_armband}. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% re organized by yaxuan.  Here is the old version
% Augmented reality (AR) and virtual reality (VR) are two emerging fields that will change the way we interact and view the world around us. Many of the services provided by AR and VR are made possible only through HAR. For instance, a major method of interacting with AR and VR systems will be through arm or body gestures. Robust HAR to recognize these gestures will be crucial for effective and practical AR and VR systems. Several works and products have been introduced that can detect muscular activities and hand motions using electromyography (EMG) sensors embedded in an armband~\cite{EMG_review, EMG_armband}. Works such as these have impacts beyond just AR and VR, but can enable improved prostheses control for people with missing or damaged limbs \cite{EMG_prosthese, EMG_prosthese2}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
% What's worth mentioning is that these application domains are not absolutely separate. There could be overlap between them. For example, energy expenditure estimation contains the locomotion recognition as the first step. % Human computer interaction and 
%

% \textcolor{red}{(I think it doesn't hurt to include this section, but it is somewhat out of scope for the topic of "Human Activity Recognition)}
% Identity authentication is the way to secure access to the physical or digital resources through personal biological characteristics. Aside from traditional biometrics such as fingerprint, iris, voice, and face, etc., motion sensor based solutions require no active interaction or interruption. The currently proposed solutions include breathing-based authentication, PPG-based~\cite{DBN3} authentication, gait-based authentication, and motion pattern-based authentication~\cite{motionid2016}. In summary, sensor-based authentication has been under continuous development since it embodies the advantage of allowing remote authentication~\cite{shoes}.
%

%The wearable industry has been surging since recent years. The widespread deployment of wearables is deeply influencing and transforming the healthcare industry, the medical industry, and the entertainment industry, as well as reshaping the human lifestyle. 
% ~\textcolor{red}{(Haik: That is all true! Another option is to cover the adherence and even privacy issues in wearable sensors. I'm sure there are many works along these lines)}


==> 4-sensor.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Background} \label{sec:background}


% \begin{figure}
% \centering
%   \includegraphics[width=0.7 \columnwidth]{img/wordcloud.png}
%   \caption{Word cloud representation from the contents of XX papers. \textcolor{red}{SHIBO: is such a figrue providing useful information to readers?}}~\label{fig:wordcloud}
% \end{figure}



% [A figure showing the number of deep learning CV papers v.s. deep learning wearable papers (intersection as deep learning ego-centric papers) v.s. DL NLP papers V.S. speech recognition] 
 
 
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Wearable Sensors}
\label{sec:sensor}
Wearable sensors are the foundation of HAR systems. As shown in Fig.~\ref{fig:signal}, there are a large number of off-the-shelf smart devices or prototypes under development today, including smartphones, smartwatches, smart glasses, smart rings~\cite{ring}, smart gloves~\cite{nature_gloves}, smart armbands~\cite{armband}, smart necklaces~\cite{necklace2015, necksense, NeckFace2021Chen}, smart shoes~\cite{shoes}, and E-tattoos~\cite{e-tattoo}. These wearable devices cover the human body from head to toe with a general distribution of devices shown in Fig.~\ref{fig:wearables_shares_on_body_part}, as reported by \cite{wearable_database}.
% remove smart headsets, wearable cameras~\cite{sensecam},
The advance of micro-electro-mechanical system (MEMS) technology (microscopic devices, comprising a central unit such as a microprocessor and multiple components that interact with the surroundings such as microsensors) has allowed wearables to be miniaturized and light weight to reduce burden on adherence to the use of wearables and Internet of Things (IoT) technologies. In this section, we introduce and discuss some of the most prevalent MEMS sensors commonly used in wearables for HAR.
\change{The summary of wearable sensors is represented as a part of Fig. \ref{fig:taxonomy}.}






%They usually consist of a central unit that processes data (an integrated circuit chip such as microprocessor) and several components that interact with the surroundings (such as microsensors)
%Their data collection reliability, sensor robustness, device usage feasibility, function configuration, as well as the comfort level of wearables jointly determine the effectiveness of the whole system. 

%Sensors built from Micro-Electro-Mechanical Systems (MEMS) are the pillars of support for the IoT era. Consider that Bosch, one of the world's leading MEMS sensor providers, has produced over 9.5 billion MEMS sensors since 1995 \cite{Bosch}. Among various MEMS sensors, no matter wearable or environmental, the Inertial Measurement Unit (IMU) is among the most fundamental and popular sensors on the stage of IoT. Especially in the area of wearable HAR, IMU is the leading widely-adopted sensor with the most popularity.

\subsubsection{Inertial Measurement Unit (IMU)}
% \yx{passed. Need proofread}
Inertial measurement unit (IMU) is an integrated sensor package comprising of accelerometer, gyroscope, and sometimes magnetometer. Specifically, an accelerometer detects linear motion and gravitational forces by measuring the acceleration in 3 axes (x, y, and z), while a gyroscope measures rotation rate (roll, yaw, and pitch). The magnetometer is used to detect and measure the magnetic fields of the earth. Since a magnetometer is often used to obtain the posture and orientation in accordance with the geomagnetic field, which is typically outside the scope of HAR, the magnetometer is not always included in data analysis for HAR.  
% 
By contrast, accelerometers and gyroscopes are commonly used in many HAR applications. We refer to an IMU package comprising a 3-axis accelerometer and 3-axis gyroscope as a 6-axis IMU. This component is often referred to as a 9-axis IMU if a 3-axis magnetometer is also integrated. Owing to mass manufacturing and the widespread use of smartphones and wearable devices in our daily lives, IMU data are becoming more ubiquitous and more readily available to collect. % through APIs of wearable devices such as smartphones, smartwatches, and Google Glasses, etc. 
In many HAR applications, researchers carefully choose the sampling rate of the IMU sensors depending on the activity of interest, often choosing to sample between 10 and several hundred Hz. 
In \cite{SampleRate}, Chung \etal have tested a range of sampling rates and given the best one in his application. 
Besides, it's been shown that higher sampling rates allow the system to capture signals with higher precision and frequencies, leading to more accurate models at the cost of higher energy and resource consumption. 
For example, the projects presented in~\cite{ViBand, Laput2} utilize sampling rates above the typical rate. These works sample at 4 kHz to sense the vibrations generated from the interaction between a hand and a physical object. 
% There is generally no consensus on the best choice of sampling rates for different sensors. 


%which is referred to as bio-acoustic signals.
% 
% \textcolor{red}{In \cite{cnn1}, a single accelerometer is used to collect data from 3 different body parts: cloth pocket, trouser pocket and waist. Self-collected data on 100 subjects including 8 activities such as falling, running, jumping, walking, walking quickly, step walking, walking upstairs, and walking downstairs.}





\subsubsection{Electrocardiography (ECG) and Photoplethysmography (PPG)}

Electrocardiography (ECG) and photoplethysmography (PPG) are the most commonly used sensing modalities for heart rate monitoring. ECG, also called EKG, detects the electrical activity of the heart through electrodes attached to the body. The standard 12-lead ECG attaches 10 non-intrusive electrodes to form 12 leads on the limbs and chest. ECG is primarily employed to detect and diagnose cardiovascular disease and abnormal cardiac rhythms. PPG relies on the use of a low-intensity infrared (IR) light sensor to measure blood flow caused by the expansion and contraction of heart chambers and blood vessels. Changes in blood flow are detected by the PPG sensor as changes in the intensity of light; filters are then applied on the signal to allow us to obtain an estimate of heart rate. 
Since ECG directly measures the electrical signals that control heart activity, it typically provides more accurate measurements for heart rate and often serves as a baseline for evaluating PPG sensors.



% \begin{figure}[tb]
% \centering
%     \captionsetup{justification=centering}
%   \includegraphics[width=\linewidth]{img/taxonomy_sensor.png}
%   \caption{\change{Taxonomy of wearable sensors}}
%   \label{fig:tax_sensor}
% \end{figure}


\subsubsection{Electromyography (EMG)}
Electromyography (EMG) measures the electrical activity produced by muscle movement and contractions. EMG was first introduced in clinical tests to assess and diagnose the functionality of muscles and motor neurons. There are two types of EMG sensors: surface EMG (sEMG) and intramuscular EMG (iEMG). sEMG uses an array of electrodes placed on the skin to measure the electrical signals generated by muscles through the surface of the skin~\cite{wiki:emg}. 
There are a number of wearable applications that detect and assess daily activities using sEMG~\cite{EMG_armband, EMG_handmotion}. 
In~\cite{cnn12}, researchers developed a neural network that distinguishes ten different hand motions using sEMG to advance the effectiveness of prosthetic hands.
iEMG places electrodes directly into the muscle beneath the skin. Because of its invasive nature, non-invasive wearable HAR systems do not typically include iEMG.


\subsubsection{Mechanomyography (MMG)}
Mechanomyography (MMG) uses a microphone or accelerometer to measure low-frequency muscle contractions and vibrations, as opposed to EMG, which uses electrodes. For example, 4-channel MMG signals from the thigh can be used to detect knee motion patterns \cite{cnn11}. Detecting these knee motions is helpful for the development of power-assisted wearables for powered lower limb protheses. The authors create a convolutional neural network and support vector machine (CNN-SVM) architecture comprising a 7-layer CNN to learn dominant features for specific knee movements. The authors then replace the fully connected layers with an SVM classifier trained with the extracted feature vectors to improve knee motion pattern recognition.
Moreover, Meagher et al \cite{meagher2020new} proposed developing an MMG device as a wearable sensor to detect mechanical muscle activity for rehabilitation after stroke.


% 
% 2016 A convolutional neural network for robotic arm guidance using sEMG based frequency-features
% 2016 Multiday EMG-Based Classification of Hand Motions with Deep Learning Techniques
% 2017 Transfer Learning for sEMG Hand Gestures Recognition Using Convolutional Neural Networks: TL_CNN2
% 2018 Deep Learning for Electromyographic Hand Gesture Signal Classification Using Transfer Learning
% 2018 Worker Activity Recognition in Smart Manufacturing Using IMU and sEMG Signals with Convolutional Neural Networks:
% 2018 EMG Pattern Recognition in the Era of Big Data and Deep Learning: EMG_review
% 2019 An sEMG-Based Human–Robot Interface for Robotic Hands Using Machine Learning and Synergies: EMG_armband (non-deep learning)





 % \textcolor{red}{(Haik: I believe that EEG, EMG, ECG in particular are all very related concepts that could be separated from the discussion and discussed independently)} for recording the electrical stimulus produced by skeletal muscles, 
Other wearable sensors used in HAR include (but are not limited to) \change{piezoelectric sensor \cite{khalifa2017harke, cha2018flexible} for converting changes in pressure, acceleration, temperature, strain, or force to electrical charge, barometric pressure sensor \cite{masse2015improving} for atmospheric pressure, temperature measurement \cite{barna2019study},} electroencephalography (EEG) for measuring brain activity \cite{salehzadeh2020human}, respiration sensors for breathing monitoring \cite{ramos2016using}, ultraviolet (UV) sensors \cite{filippoupolitis2016activity} for sun exposure assessment, GPS for location sensing, \change{microphones for audio recording \cite{jin2021sonicasl, ntalampiras2018transfer, CoughBuddy2021Nemati}}, and wearable cameras for image or video recording \cite{NeckFace2021Chen}. 
% Specifically, images and videos are often recorded by wearable cameras, which are often referred to as egocentric cameras. 
% 
It is also important to note that the wearable camera market has drastically grown with cameras such as GoPro becoming mainstream \cite{GoPro1, GoPro2, alharbi2018can, alharbi2019mask} over the last few years. However, due to privacy concerns posed by participants related to video recording, utilizing wearable cameras for longitudinal activity recognition is not as prevalent as other sensors. Additionally, HAR with image/video processing has been extensively studied in the computer vision community \cite{voulodimos2018deep, xu2020computer}, and the methodologies commonly used differ significantly from techniques used for IMUs, EEG, PPG, etc. For these reasons, despite their significance in applications of deep learning methods, this work does not cover image and video sensing for HAR. 


% measure changes in pressure, acceleration, temperature, strain, or force by converting them to an electrical charge

% \begin{figure}[!h]
% \centering
%   \includegraphics[width=\columnwidth]{img/sensors.pdf}
%   \caption{Typical devices and application domains of wearables. \textcolor{red}{Where is this referenced in text?}}~\label{fig:signal}
% \end{figure}


% \begin{figure}[!h]
% \centering
%   \includegraphics[width=0.63\columnwidth]{final_images/wearables_shares_on_body_part.png}
%   \caption{Distribution of wearable devices placed on common body areas \cite{wearable_database}.  \textcolor{red}{Where is this referenced in text?}}
%   \label{fig:wearables_shares_on_body_part}
% \end{figure}


% \subsection{Problem Definition}
% %
% %
% Conventionally, we convert the detection task to a classification problem by pre-defining classes of interest and the NULL class. With a sliding window manner and classification approach,
% %

% The way that it's transformed to a classification problem
% is similar to the object detection problem in computer vision area and keyword spotting problem in speech recognition area.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> 5-1-auto_encoder.tex <==
\section{Deep Learning Approaches}
\label{sec:deeplearning}

In recent years, DL approaches have been shown to outperform traditional ML approaches in a wide range of HAR tasks. There are three key factors behind deep learning's success: increasingly available data, hardware acceleration, and algorithmic advancements. The growth of datasets publicly shared through the web has allowed developers and researchers to quickly develop robust and complex models. Development of GPUs and FPGAs have drastically shortened the training time of complex and large models. Finally, improvements in optimization and training techniques have also improved training speed. In this section, we will describe and summarize HAR works from six types of deep learning approaches. 
\change{
We also present an overview of deep learning approaches in Fig. \ref{fig:taxonomy}.}


% \begin{figure}[t]
% \centering
% \captionsetup{justification=centering}
%   \includegraphics[width=\linewidth]{img/taxonomy_ml_approaches.png}
%   \caption{\change{Taxonomy of deep learning approaches. }}
%   \label{fig:tax_ml}
% \end{figure}


%\textcolor{purple}{In recent years, DL approaches outperform traditional ML approaches in a wide range of HAR tasks. There are three key factors behind the arisal of deep learning: increasingly available data, hardware acceleration, and algorithmic advancements. Data-wise, the web-scaled data explosion provides the opportunity to train a large model with an exponential number of parameters. From hardware aspect, the prevalent usage of GPUs and FPGAs in training deep neural networks has dramatically shorten the training time from a formidable amount of time to a reasonable level. Besides, the development of deep neural models, the advancement of optimization techniques, and a bag of training tricks have collectively underpinned the boom of deep learning. In this section, we will describe 6 types of mainstream deep learning approaches that are applied in HAR tasks.}


\subsection{Autoencoder}




The autoencoder, originally called ``autoassociative learning module", was first proposed in the 1980s as an unsupervised pre-training method for artificial neural networks (ANN) ~\cite{AE0}.
Autoencoders have been widely adopted as an unsupervised method for learning features. As such, the outputs of autoencoders are often used as inputs to other networks and algorithms to improve performance \cite{AE420, AE437, AE440, AE460, AE463}. An autoencoder is generally composed of an encoder module and a decoder module. The encoding module encodes the input signals into a latent space, while the decoder module transforms signals from the latent space back into the original domain. As shown in Figure \ref{fig:fig_ae}, the encoder and decoder module is usually several dense layers (i.e., fully connected layers) of the form 

$$
\begin{array}{l}
f_{\theta}(\mathbf{x}): \mathbf{z}=\sigma\left(W_{e} \mathbf{x}+b_{e}\right) \\
g_{\theta^{\prime}}(\mathbf{z}): \mathbf{x}^{\prime}=\sigma\left(W_{d} \mathbf{z}+b_{d}\right)
\end{array}
$$

where $\theta=\left\{W_{e}, b_{e}\right\}$, $\theta^{\prime}=\left\{W_{d}, b_{d}\right\}$ are the learnable parameters of the encoder and decoder. $\sigma$ is the non-linear activation function, such as Sigmoid, tanh, or rectified linear unit (ReLU). $W_{e}$ and $W_{d}$ refer to the weights of the layer, while $b_e$ and $b_d$ are the bias vectors. By minimizing a loss function applied on $\mathbf{x}$ and $\mathbf{x}^{\prime}$, autoencoders aim at generating the final output by imitating the input. Autoencoders are efficient tools for finding optimal codes, $\mathbf{z}$, and performing dimensionality reduction. An autoencoder's strength in dimensionality reduction has been applied to HAR in wearables \cite{AE1, AE2, AE3, AE4, AE437, AE6, AE7, AE8, AE423} and functions as a powerful tool for denoising and information retrieval.

\begin{figure}
\centering
\captionsetup{justification=centering}
  \includegraphics[width=0.53\linewidth]{img/fig_ae}
  \caption{Illustration of an autoencoder network~\cite{autoencoder_graph}.}
  \label{fig:fig_ae}
\end{figure}


As such, autoencoders are most commonly used for feature extraction and dimensionality reduction \cite{AE1, AE416, AE417, AE419, AE420, AE422, AE426, AE427, AE432, AE436, AE440, AE445, AE452, AE460, AE463, AE464}. Autoencoders are generally used as is, or in a stacked architecture with multiple autoencoders.
\textit{Mean squared error} or \textit{mean squared error plus KL divergence} loss functions are typically used to train autoencoders. Li \etal presents an autoencoder architecture where a sparse autoencoder and a denoising autoencoder are used to explore useful feature representations from accelerometer and gyroscope sensor data, and then they perform classification using support vector machines~\cite{AE1}. Experiments are performed on a public HAR dataset \cite{UCI-HAR} from the UCI repository, and the classification accuracy is compared with that of Fast Fourier Transform (FFT) in the frequency domain and Principal Component Analysis (PCA). The result reveals that the stacked autoencoder has the highest accuracy of 92.16\% and provides a 7\% advantage over traditional methods with hand-crafted features. Jun and Choi \cite{AE481} studied classification of newborn and infant activities into four classes: sleeping, moving in agony, moving in normal condition, and movement by an external force. Using the data from an accelerometer attached to the body and a 3-layer autoencoder combined with k-means clustering, they achieve 96\% weighted accuracy in an unsupervised way. 
Additionally, autoencoders have been explored for feature extraction in domain transfer learning \cite{AE439}, detecting unseen data \cite{AE434}, and recognizing null classes \cite{AE435}. \change{For example, \citet{prabono2021atypical} propose a two-phase autoencoder-based approach of domain adaptation for human activity recognition. In addition, \citet{garcia2021ensemble} proposed an effective multi-class algorithm which consists of an ensemble of autoencoders where each autoencoder is associated with a separate class. This modular structure of classifiers makes models more flexible when adding new classes, which only calls for adding new autoencoders instead of re-training the model.}


Furthermore, autoencoders are commonly used to sanitize and denoise raw sensor data \cite{AE3, AE8, AE467}, a known problem with wearable signals that impacts our ability to learn patterns in the data.
Mohammed and Tashev in \cite{AE3} investigated the use of sensors integrated into common pieces of clothing for HAR.
However, they found that sensors attached to loose clothing are prone to contain large amounts of motion artifacts, leading to low mean signal-to-noise ratios (SNR). % as low as \zs{(commonly SNR in range of ...?)}. \yx{I didn't found "commonly range" in their paper. I think they conducted experiments and found that mean is -12 in their setup.} \zs{got it.}
To remove motion artifacts, the authors propose a deconvolutional sequence-to-sequence autoencoder (DSTSAE). The weights for this network are trained with a weighted form of standard VAE loss function. Experiments show that the DSTSAE outperforms traditional Kalman Filters and improves the SNR from -12 dB to +18.2 dB, with the F1-score of recognizing gestures improved by 14.4\% and locomotion activities by 55.3\%. 
Gao \etal explores the use of stacking autoencoders to denoise raw sensor data to improve HAR using the UCI dataset \cite{UCI-HAR}~\cite{AE8}. Then, LightGBM (LBG) is used to classify activities using the denoised signals.

Autoencoders are also commonly used to detect abnormal muscle movements, such as those resulting from Parkinson's Disease and Autism Spectrum Disorder (ASD).
% 
Rad \etal in \cite{AE4} utilizes an autoencoder to denoise and extract optimized features of different movements and use a one-class SVM to detect movement anomalies. To reduce overfitting the autoencoder, the authors inject artificial noise, to simulate different types of perturbations, into the training data. Sigcha \etal in \cite{AE478} uses a denoising autoencoder to detect freezing of gait (FOG) in Parkinson's disease patients. The autoencoder is only trained using data labelled as normal movement. During the testing phase, samples with significant statistical differences from training data are classified as abnormal FOG events.

As autoencoders map data into a nonlinear and low-dimensional latent space, they are well-suited for applications requiring privacy preservation. Malekzadeh \etal developed a novel replacement autoencoder that removes prominent features of sensitive activities, such as drinking, smoking, or using the restroom~\cite{AE437}. Specifically, the replacement autoencoder is trained to produce a non-sensitive output from a sensitive input via stochastic replacement while keeping characteristics of other less sensitive activities unchanged. Extensive experiments are performed on Opportunity \cite{Opportunity}, Skoda \cite{Skoda}, and Hand-Gesture \cite{ActRecTut} datasets. The result shows that the proposed replacement autoencoder can retain the recognition accuracy of non-sensitive tasks using state-of-the-art techniques while simultaneously reducing detection capability for sensitive tasks. 

Mohammad \etal introduces a framework called Guardian-Estimator-Neutralizer (GEN) that attempts to recognize activities while preserving gender privacy~\cite{AE6}. 
The rationale behind GEN is to transform the data into a set of features containing only non-sensitive features. 
The Guardian, which is constructed by a deep denoising autoencoder, transforms the data into representation in an inference-specific space. 
% The Guardian part of the architecture is a deep denoising autoencoder that provides an inference-specific transformation. 
The Estimator comprises a multitask convolutional neural network that guides the Guardian by estimating sensitive and non-sensitive information in the transformed data. It attempts to recognize an activity without disclosing a participant's gender due to privacy concerns. 
The Neutralizer is an optimizer that helps the Guardian converge to a near-optimal transformation function. 
Both the publicly available MobiAct \cite{MobiAct} and a new dataset, MotionSense, are used to evaluate the proposed framework's efficacy. 
Experimental results demonstrate that the proposed framework can maintain the usefulness of the transformed data for activity recognition while reducing the gender classification accuracy to 50\% (random guessing) from more than 90\% when using raw sensor data. 
Similarly, the same authors have proposed another anonymizing autoencoder in \cite{AE7} for classifying different activities while reducing user identification accuracy. Unlike most works, where the output to the encoder is used as features for classification, this work utilizes both the encoder and decoder outputs. Experiments performed on a self-collected dataset from the accelerometer and gyroscope showcased excellent activity recognition performance (above 92\%), while keeping user identification accuracy below 7\%.




==> 5-2-cnn.tex <==
\subsection{Convolutional Neural Network (CNN)}

% \begin{table*}[t]
% \centering 
% \caption{Comparing the literature on in-wild eating detection to this work.}
% \begin{small}
% \begin{tabular*}{\textwidth}{p{0.5cm}p{4.5cm}p{0.5cm}p{4.8cm}cc c}
% \toprule
%     {Study} & {Architecture} & \mc{\stackon{kernel}{Conv.}} & {Activity of interest} & \mc{\stackon{classes}{Num. of}} &  {Sensors} & {Dataset} \\
%     \midrule
%     {[89]} & C-P-C-P-C-P-S & 12*2 & daily activities including brush teeth, comb hair, get up from bed, etc & 12 & S1, S2, S3 & WHARF \\
    
%     {[1]} &  &  & locomotion activities including falling, running, jumping, etc &  & S1 & self \\
% % 2014  & Fontana et al.~\cite{fontana2014automatic} & S1, S4, S6	 & Ear, wrist, chest & 12 & 24.0 &  \xmark & \cmark & \cmark\\
% % 2015& {Thomaz et al.~\cite{Thomaz2015}}&S1&Wrist&7+1&5.7/13.6&\xmark&\xmark&\xmark\\
% \bottomrule
% \end{tabular*}
% \end{small}
% \begin{captiontext}
% \begin{small}
% C - convolutional layer, P - max pooling layer, FC - fully connected layer, S - softmax\\
%  S1 - accelerometer, S2 - gyroscope, S3 - magnetometer, S4 - piezo, S5 - proximity, S6 - radio frequency, S7 - microphone, S8 - electromyography, S9 - light, S10 - camera
% \end{small}
% \end{captiontext}
% \label{tbl:eating_detect_table}
% \end{table*}



% \newgeometry{margin=.2cm} % modify this if you need even more space
% \begin{landscape}

% S1 - accelerometer, S2 - gyroscope, S3 - magnetometer, S4 - piezo, S5 - proximity, S6 - radio frequency, S7 - microphone, S8 - electromyography, S9 - light, S10 - camera
% \begin{minipage}
% \begin{adjustbox}{angle=90}
\begin{table*}[tbh]
\centering
\captionsetup{justification=centering}
\caption{\changezs{Summary of typical studies that use layer-by-layer CNN structure in HAR and their configurations. \change{We aim to present the relationship of CNN kernels, layers, and targeted problems (application and sensors)}.} Key: C - convolutional layer, P - max-pooling layer, FC - fully connected layer, S - softmax, S1 - accelerometer, S2 - gyroscope, S3 - magnetometer, S4 - EMG, S5 - ECG}

\begin{tabular}{c|c|c|c|c|c|c}
\hline
Study    & Architecture & \thead{Kernel\\ Conv.}   & Application       & \# Classes & Sensors  & Dataset \\ \hline
{\cite{cnn10}} & C-P-FC-S    & \begin{tabular}[c]{@{}c@{}}1$\times$3, 1$\times$4,\\ 1$\times$5\end{tabular}  & locomotion activities     & 3 & S1   & Self     \\ \hline
{\cite{gholamrezaii2021time}} & \change{C-P-C-P-S}  & \change{4$\times$4} & \change{locomotion activities}  & \change{6, 12}   & \change{S1} & \change{UCI, mHealth}   \\ \hline
{\cite{cnn9}}  & C-P-FC-FC-S & 1$\times$20 & \begin{tabular}[c]{@{}c@{}}daily activities,\\ locomotion activities\end{tabular}                                                   & -                          & -& \begin{tabular}[c]{@{}c@{}c@{}}Skoda, \\ Opportunity, \\ Actitracker\end{tabular}           \\ \hline
{\cite{xu2021human}} & \change{C-P-C-P-FC-S}  & \change{5$\times$5} & \change{locomotion activities}  & \change{6}   & \change{S1} & \change{WISDM}   \\ \hline
{\change{\cite{uddin2018activity}}} & \change{C-P-C-P-C-FC}   &  \change{$1\times5, 1\times9$} & \change{locomotion activities}  & \change{12}   & \change{S5} & \change{mHealth}   \\ \hline
{\cite{cnn13}} & C-P-C-P-FC-FC-S & -               & \begin{tabular}[c]{@{}c@{}}daily activities,\\ locomotion activities\end{tabular}                    & 12      & \begin{tabular}[c]{@{}c@{}}S1, S2, S3 \\ ECG\end{tabular} & mHealth          \\ \hline
{\cite{cnn89}} & C-P-C-P-C-P-S & 12$\times$2            & \begin{tabular}[c]{@{}c@{}}daily activities including \\ brush teeth, comb hair, \\ get up from bed, etc\end{tabular}               & 12                                                               & S1, S2, S3                                                                   & WHARF                                                                                \\ \hline
{\cite{cnn1}}  & C-P-C-P-C-P-S                                                                                         &   12$\times$2      & locomotion activities   & 8 & S1    & Self  \\ \hline
{\cite{cnn5}}  & \begin{tabular}[c]{@{}c@{}}C-P-C-P-U-FC-S, \\ U: unification layer\end{tabular}                       & 1$\times$3, 1$\times$5        & \begin{tabular}[c]{@{}c@{}}daily activities,\\ hand gesture\end{tabular}  & \begin{tabular}[c]{@{}c@{}}18 (Opp)\\ 12 (hand)\end{tabular} & \begin{tabular}[c]{@{}c@{}}S1, S2 \\ (1 for each)\end{tabular}               & \begin{tabular}[c]{@{}c@{}}Opportunity\\ Hand Gesture\end{tabular}                   \\ \hline
% {[}2{]}  & leave for later    &     &  & &  &   \\ \hline
{\cite{cnn12}} & C-C-P-C-C-P-FC  & 1$\times$8  & hand motion classification & 10    & S4     & \begin{tabular}[c]{@{}c@{}}Rami EMG\\Dataset\end{tabular}       \\ \hline
% {\cite{cnn11}} & C-P-C-P-FC-FC-SVM     &  &  & &     &     \\ \hline
{\cite{cnn17}} & \begin{tabular}[c]{@{}c@{}}C-C-P-C-C-\\P-FC-FC-S \\ (one branch \\ for each sensor)\end{tabular} & 1$\times$5             & \begin{tabular}[c]{@{}c@{}}daily activities,\\  locomotion activities,\\  industrial ordering \\ picking recognition task\end{tabular} & \begin{tabular}[c]{@{}c@{}}18 (Opp)\\ 12 (PAMAP2)\end{tabular}   &   S1, S2, S3     & \begin{tabular}[c]{@{}@{}c@{}}Opportunity,\\PAMAP2,\\ Order Picking\end{tabular} \\ \hline
% {[}20{]} &   &                 &   &   &   &      \\ \hline
% {[}37{]} &   &                 &   &   &   &  \\ \hline
{\cite{cnn35}} & \begin{tabular}[c]{@{}c@{}}C-P-C-P-C-P-\\ FC-FC-FC-S\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1$\times$4, 1$\times$10,\\ 1$\times$15\end{tabular}  & locomotion activities  & 6   & S1, S2, S3 & Self   \\ \hline
\end{tabular}
\label{tab:CNN}
\end{table*}
% \end{adjustbox}
% \end{landscape}
% \restoregeometry
% \end{minipage}


% \textcolor{red}{Haik: I think we should decide once again who the target audience is for this paper. Because readers unfamiliar with the material will not be able to follow your explanation: its a very complex topic to condense into three paragraphs. And those which do know, probably don't need it. So either a much more thorough explanation is needed for those with no background, or a simple sentence (with citations) will be enough, and your paper should be emphasizing the applications instead}
A CNN comprises convolutional layers that make use of the convolution operation, pooling layers, fully connected layers, and an output layer (usually Softmax layer). The convolution operation, with a shared kernel, enables the learning process of space invariant features. Because each filter in a convolutional layer has a defined receptive field, CNN is good at capturing local dependency, compared with a fully-connected neural network. Though each kernel in a layer covers a limited size of input neurons, by stacking multiple layers, the neurons of higher layers will cover a larger more global receptive field. The pyramid structure of CNN contributes to its capability of gathering low-level local features into high-level semantic meanings. This allows CNN to learn excellent features as shown in \cite{cnn91}, which compares the features extracted from CNN to hand-crafted time and frequency domain features (Fast Fourier Transform and Discrete Cosine Transform).

% The mechanism of CNN resembles the biological processes of the animal visual cortex~\cite{cnn_origin}. 
% Featured by incorporating convolutional operation, CNN is composed of convolutional layers, pooling layers, fully connected layers, and a softmax layer. 
% The convolutional operation, with a shared kernel, enables the learning process of space invariant features. 
% 
% Compared with a fully-connected neural network, CNN is good at capturing local dependency since each filter in one convolutional layer has a defined receptive field. Though each kernel in a layer covers a limited size of input neurons, by stacking multiple layers, the neurons of higher layers turn to cover a large area of the reception field. 
% and with convolutional layers stacked together, the overall receptive field can be derived. 


CNN incorporates a pooling layer that follows each convolutional layer in most cases. A pooling layer compresses the representation it is learning and strengthens the model against noise by dropping a portion of the output to a convolutional layer. Generally a few fully connected layers follow after a stack of convolutional and pooling layers that reduces feature dimensionality before it is fed into the output layer. A softmax classifier is usually selected as the final output layer. But as an exception, some studies explored the use of traditional classifiers as the output layer in a CNN \cite{cnn11,cnn115}. 

% 
% \textcolor{red}{[91] compared hand-craft time domain and frequency domain features, Fast Fourier Transform, Discrete Cosine Transform and CNN features. They extract features from accelerometer data collected from wrist and thigh.} 


% In this part, we will exhibit different types of CNNs used for HAR and guide the introduction of existing works with a handful of research questions during this survey work. We pay special attention to questions of these aspects: 1). What format are the input data used in? 2). How many layers are used? What is the loss function? 3). What datasets are used in these work? Identify the application and categorize them.


% \begin{itemize}
%     \item $\mathsf{Q1:}$ \textbf{Input data}
% \end{itemize}

Most CNNs use univariate or multivariate sensor data as input. Besides raw or filtered sensor data, the magnitude of 3-axis acceleration is often used as input, as shown in \cite{cnn10}. Researchers have tried encoding time-series data into 2D images as input into the CNN. In \cite{cnn35}, the Short-time Fourier transform (STFT) for time-series sensor data is calculated and its power spectrum is used as the input to a CNN. Since time series data is generally 1-dimensional, most CNNs adopt 1D-CNN kernels. Works that use frequency domain inputs (e.g. spectrogram), which have an additional frequency dimension, will generally use 2D-CNN kernels \cite{cnn69}. The choice of 1D-CNN kernel size normally falls in the range of 1$\times$3 to 1$\times$5 (with exceptions in \cite{cnn9,cnn11,cnn12} where kernels of size 1$\times$8, 2$\times$101, and 1$\times$20 are adopted). 

% 1*8: [46] An Improved Performance of Deep Learning Based on Convolution Neural Network to Classify
% 2*101: cnn-svm - [47]
% 1*20: CNN-HAR-MS - [119]

% Researchers also tried encoding time-series data into 2D images and then taking 2D images as input. % apply 2D CNN to classify human activities [105]. %They use HHAR and MHEALTH dataset. 
% In \cite{cnn35}, since human activities differ largely among individuals, they adapt their model to each individual with a small amount of his/her data. 
% Short-time Fourier transform (STFT) for time-series sensor data is calculated in pre-processing and its power spectrum is used as an input to a CNN. 
% It inserts several hidden unit layers in the network and customized the weights using a small amount of user-dependent data. Recognition performance was improved by 3\%. 

% Novel weight sharing method in convolutional operation was also proposed. In the CNN model of [13], partial and full weight sharing, which was called CNN-pff, was used in first convolutional layer and \textbf{full weight sharing} in the second convolutional layer. The novel weight sharing method outperforms normal 1D-CNN and 2D-CNN on dataset Mhealth, which contains 3 accelerometers (chest, right wrist, left ankle) and 2 gyroscopes (right wrist, left ankle). 
% In [9], They proposed \textbf{CNN partial weight sharing} and showed it outperforms traditional CNN and traditional ML methods.

%
% In [84], they use a set of lower-dimensional filters as Lego bricks to be stacked for conventional filters, which can greatly reduce memory and computation cost over CNN, while achieving higher accuracy. 

% A public dataset (R. N. Khushaba, M. Takruri, S. Kodagoda, and G. Dissanayake, "Toward Improved Control of Prosthetic Fingers Using Surface Electromyogram (EMG) Signals", Expert Systems with Applications, vol 39, no. 12, pp. 10731–10738, 2012.) % 8-layer architecture with 4 conv layers used


% \begin{itemize}
%     \item $\mathsf{Q2:}$ \textbf{Network structure}
% \end{itemize}

To discover the relationship between the number of layers, the kernel size, and the complexity level of the tasks, we picked and summarized several typical studies in table \ref{tab:CNN}.
%
A majority of the CNNs consist of 5 to 9 layers \cite{cnn1,cnn2, cnn5, cnn11, cnn12, cnn17, cnn31}, \cite{huang2021shallow}, \cite{gao2021deep}, usually including 2 to 3 convolutional layers, 2 to 3 max pooling layers, followed by 1 to 2 fully connected layers before feeding the feature representation into the output layer (softmax layer in most cases). \changezs{\citet{dong2019harnet} demonstrated performance improvements by leveraging both handcrafted time and frequency domain features along with features generated from a CNN, called HAR-Net, to classify six locomotion activities using accelerometer and gyroscope signals from a smartphone.} \citet{cnn66} used a shallow 3-layer CNN network including a convolutional layer, a fully connected layer, and a softmax layer to perform on-device activity recognition on a resource limited platform and shown its effectiveness and efficiency on public datasets. \citet{cnn9} and \citet{cnn10} also used a small number of layers (4 layers). 
% 
The choice of loss function is an important decision in training CNNs. In classification tasks, cross-entropy is most commonly used, while in regression tasks, mean squared error is most commonly used. %~\cite{cnn11}\textcolor{red}{[X]}.
\change{Most CNN models process input data by extracting and learning channel-wise features separately while \citet{huang2021shallow} first propose a shallow CNN that considers cross-channel communication.
The channels in the same layer interact with each other to obtain discriminative features of sensor data.
}
% 
% 
% 
% In \cite{cnn9}, the authors built a 4-layer model with 1 convolutional layer, 1 pooling layer and 2 fully connected layers on three public datasets: Skoda, Opportunity, Actitracker. They proposed \textbf{CNN partial weight sharing} and showed it outperforms traditional CNN and traditional ML methods. Experiments also showed the influence of different pooling sizes, dropout, weight decay and momentum in optimization.


The number of sensors used in a HAR study can vary from a single one to as many as 23 \cite{Opportunity}. In \cite{cnn1}, a single accelerometer is used to collect data from 3 locations on the body: cloth pocket, trouser pocket and waist. The authors collect data on 100 subjects including 8 activities such as falling, running, jumping, walking, walking quickly, step walking, walking upstairs, and walking downstairs. 
Moreover, HAR applications can involve multiple sensors of different types. 
To account for all these different types of sensors and activities, \citet{cnn49} proposed a multi-branch CNN architecture. 
% Thus, a variety of sensor fusion designs are proposed. Typical fusion methods include uni-branch structure [66] and multi-branch structure [49]. 
% Uni-branch structure [66] ...
A multi-branch design adopts a parallel structure which trains separate kernels for each IMU sensor and concatenates the output of branches at a late stage, after which one or more fully connected layers are applied on the flattened feature representation before feeding into the final output layer. For instance, a CNN-IMU architecture contains \textit{m} parallel branches, one per IMU. Each branch contains 7 layers, then the outputs of each branch are concatenated and fed into a fully connected and a softmax output layer.
% 
\change{\citet{GAO2021107728} has introduced a novel dual attention module including channel and temporal attention to improve the representation learning ability of a CNN model. Their method has outperformed regular CNN considerably on a number of public datasets such as PAMAP2 \cite{PAMAP2}, WISDM \cite{WISDM}, UNIMIB SHAR \cite{SHAR}, and Opportunity \cite{Opportunity}.}

Another advantage of DL is that the features learned in one domain can be easily generalized or transferred to other domains. The same human activities performed by different individuals can have drastically different sensor readings. To address this challenge, \citet{cnn35} adapted their activity recognition to each individual by adding a few hidden layers and customizing the weights using a small amount of individual data. They were able to show a 3\% improvement in recognition performance.



% % 
% Opportunity dataset: gesture task - 92.4 accuracy, 92.3 weighted F1. Opportunity-Locomotion - 89.8 accuracy, 89.7 weighted F1; PAMAP2 dataset - 93.1 accuracy, 93.2 weighted F1. 
% % 
% In [1], a single accelerometer is used to collect data from 3 different body parts: cloth pocket, trouser pocket and waist. Self-collected data on 100 subjects including 8 activities such as falling, running, jumping, walking, walking quickly, step walking, walking upstairs, and walking downstairs.



% In [10], a 4-layer CNN (1 convolutional layer, 1 max pooling layer, 1 FC and 1 softmax) was constructed. Data are collected from 5 participants using one accelerometer. The input is the magnitude of the 3-axis acceleration. In the convolutional layer, 3 kernel sizes are used to extract features from the acc magnitude input signal, then the output is passed through a max pooling layers, after which they are combined into a single feature vector and sent to FC and softmax layers. 


% In [5], a 7-layer CNN, including 3 convolutional layers, 2 subsampling (pooling) layers, 1 unification layer, and 1 FC layer is proposed. 
% The kernels in the 3 convolutional layers have the size of 1*5, 1*5, and 1*3. 
% A special layer called unification layer, which is a fully-connected layer for unifying the outputs of all the sensors and followed by a ReLU layer and normalization layer, is proposed to construct the CNN for HAR. 
% On two HAR dataset Opportunity and ActRecTut, improvements have been shown over traditional approaches SVM and KNN as well as the DBN method from~\cite{DBN0}.
% \zs{In [5], a special layer called unification layer, which is a fully-connected layer for unifying the outputs of all the sensors and followed by a ReLU layer and normalization layer, is proposed to construct the CNN for HAR.}


% Besides, The authors in~\cite{rokni2018personalized} has utilized a discretization layer to reduce sensitivity of the CNN model to subtle changes and increase the robustness of the model. 



% \textcolor{orange}{for shibo summary. 1d cnn}
% In [89], 3 layers of convolutional + max pooling + softmax. the authors propose to apply 1D CNN on accelerometer data in WHARF dataset to classify human activities. 


% \textcolor{orange}{for shibo summary. 1d cnn}
% In [97], researchers use tri-axial accelerometer data from WISDM dataset and apply \textbf{1D-CNN} to classify six kinds of human daily activities. 


% \zs{doubtful}
% In [111], researchers extract features from imu and audio data and feed into 1D CNN. For imu data, they achieve 91.98\% on UCI-HAR, 67.51\% on real-world Extrasensory dataset. For audio data, they achieve 92.30\% on the DCASE 2017 dataset and 35.24\% on the Extrasensory dataset. 



% \zs{In [31], instead of end-to-end training, we incorporated greedy-wise tuning starting from (the number of layers).}

% \begin{itemize}
%     \item $\mathsf{Q3:}$ \textbf{Application and dataset}
% \end{itemize}




% Some key points for each paper: \\
% \begin{itemize}
% \item INPUT: [FAZARD] What sensors and how many sensors are used? Are the input data multi-variant time series data? For example some papers use FFT and spectragram as input data. (fazard, need to briefly mention data augmentation if used) \\

% \item ARCH: [SHIBO] How many layers are used? We can draw some conclusion about the most used number of layers. What is the loss function? (shallow or deep, wide or narrow, arch, batch norm, Resnet, combined network)\\ 

% \item DATASET: [YAXUAN] What dataset are used, did they test on public dataset?\\

% \item APPlications: [YAXUAN] Identify the application and categorize them? Like Parkinson disease or infant activity recognition\\

% \item NOTES: [ALL] Is there any interesting finding in the paper?

% \end{itemize}


% \zs{In [31], instead of end-to-end training, we incorporated \textbf{greedy-wise tuning} starting from the number of layers. Dataset: HAR smartphone dataset from the UCI repository, 94.8\% accuracy. 7-layer with 3 conv layers.} 



% Modularized deep learning blocks are introduced to HAR. 
% % 
% In~\cite{innohar}, they have used GoogLeNet’s Inception module combined with GRU layer to build a HAR model. The proposed model was tested on three public dataset (Opportunity, PAMAP2 and Smartphones datasets) and better performance (F-Score) presented.

% Loss function is an important block of deep learning network.
% With respect to loss function, cross-entropy is the most widely used loss function in classification tasks. When regression model is built, mean squared error is used [11].



% Some studies explored the use of CNN in combination with other traditional classifiers. In [115], researchers proposed to use 1D CNN as feature extractor, following a LSTM module and then an extreme learning machine (ELM) classifier and outperform 8\% by other previous work. 


% \zs{transfer learning} \\
% Transfer learning  framework.
% In [20], the authors using convolutional neural networks to build a personalized activity recognition model with minimal user supervision. Having a trained network for a group of users as the source domain, we devise a personalized model by reusing the lower layers of the network and retrained the upper layer with a few number of instances in the target domain. 
% Dataset: Sport and Daily Activity (SDA) (Altun, Barshan 2010) and WISDM. 
% We showed that using representation learning, we can reuse the general features learned from available training data and construct a personalized model with only few labeled instances.
% % 
% In~\cite{rokni2018personalized}, they validated the transferrability of the trained model by re-using the lower layers of the network and re-training upper layers with a fractional number of data in target domain. 


% In addition to the applications discuss in Section XX, there are a few innovative applications for human activity recognition using CNN. 
% % 
% In [24], accurately predicting human locomotion intent is beneficial in controlling wearable robots and in assisting humans to walk smoothly on different terrains.
% % 
% Researchers in [38], attach IMU on healthy legs for obtaining data within the early swing phase to identify the motion intention by feeding data into the CNN model. Then the model can help to adaptively calibrate the control strategy for actuating powered intelligent prosthesis in advance for both unilateral amputees and the able-bodied. The results achieve 94.15\% for the able-bodied and 89.23\% for amputees on 13 classes of motion intent.
% % 
% Moreover, researchers use Steady StateVisually Evoked Potentials (SSVEP) to extract discriminated features from real-time electroencephalographic (EEG) data through CNN, which is then utilized to control the avatar to navigate and walk in an immersive virtual environment through Brain-Computer Interface (BCI). 
% % 
% In [108], the researcher installed IMUs on the healthy leg of lower limb amputees for monitoring its locomotion state and use CNN to predict the motion intent of both unilateral amputees and the able-bodied. 
% % 
% In [90], the researchers apply 1D CNN on data from a wrist-worn tri-axial accelerometer-based food and drink intake monitoring system. 
% % 
% In [2], locomotion mode recognition can contribute to precise control of active lower-limb prostheses in different environments. The strain gauge only provides one-dimensional signals and is also used in the control strategy of the robotic prosthesis. The convolutional neural network takes the raw noisy signals as inputs. Three transtibial amputee subjects were recruited in the experiments, and three locomotion modes were recognized. 6-layer with 2 convolutional layers. %Loss function: cross-entropy, Adam optimizer










% Deep Neural Network based Human Activity Recognition for the Order Picking Process\\
 
% \zs{parallel channel for each sensor: conv+mpool+conv+mpool+fc, then stack -) fc+fc+softmax}

% In [49], a CNN architecture is proposed to analyze the order picking process utilizing HAR data. Two \textbf{data augmentation} approaches are. First, gaussian noise has been added to the sensor samples. Second, samples from a given window are resampled. The CNN architecture is as follows: parallel processing blocks are used to process the IMU data independently. Each block is processed by a temporal convolution. Each channel has two 5*1 convolutions followed by 2*1 max pooling layer. Two of these blocks are combined resulting in 4 convolution layers. Then, one fully connected layer is at the end of each processing channel. Data from each IMU channel is stacked and flows in two fully connected layer followed by softmax layer.  The dataset is comprised of two warehouses and contain recording from three people. Walking, searching, picking, scanning, info, carrying, and acknowledge. 27 sensors (gyroscope, accelerometer, and magnetometer) were used to collect the sensory samples at the rate of 100Hz.  
% The proposed CNN architecture outperformed the traditional methods, Bayes, Random Forest, Linear SVM, and recent CNNs. \\


% Interpretable and Accurate Convolutional Neural Networks for Human Activity Recognition\\

% \zs{16+1 layer?}\textcolor{red}{Farzad: 16 Layers (4 Conv+4 pooling + 4 Conv+4 pooling) + 3 Layers (fully connected) -----> 19 Layers}

% This paper [61] proposed an interpretable convolutional neural network (I-CNN) to assess sensory signal importance since all the signals obtained from different sensors are not important and some could be redundant in a specific context. This is enabled by Spatial Group Lasso (SGL). The experimental results are obtained from Opportunity dataset. I-CNN is composed of two blocks of 4 layered temporal convolutions followed by two blocks of 4-layered temporal pooling. Then it comes to sensor-signal selection imposed by SGL followed by flattening and fully connected layers. This combination of spatial and temporal convolutions will assist with feature extraction and enhance the recognition performance compared to baseline CNN. It also helps remove the uninformative and redundant signals from being fed into the classification.\\


%  Deep Learning for Human Activity Recognition: A Resource Efficient Implementation on Low-Power Devices\\

% \zs{3 layer: 1 conv + 1 fully connected + 1 softmax}

% This paper [66] proposed a deep learning network for real-time classification on HAR data for resource-limited devices like smart phones. Their architecture has been tested on 4 different datasets. The datasets are WISDM v1.1, Daphnet FoG, Skoda, and their own dataset ActiveMiles. In input data is fed to spectrogram filters which provides interpretable features in obtaining intensity variability around inertial sensory samples. The spectrograms output values are fed to temporal convolution layer, a fully connected layer, and a softmax layer. This architecture outperformed classification methods such as neural network and linear classifier with the data attributed varying between 23 and 102 features using wrapper methods. Finally, computation time on several resource-limited devices are calculated.\\


% Comparison of Feature Learning Methods for Human Activity Recognition Using Wearable Sensors\\

% % \begin{figure}[h]
% % \includegraphics[width=0.5\textwidth]{final_images/feature learning.JPG}
% % \caption{\label{fig:postprocessing}On OPPORTUNITY DATASET}
% % \end{figure}
% % \begin{figure}[h]
% % \includegraphics[width=0.5\textwidth]{final_images/featurelearning results.jpg}
% % \caption{\label{fig:postprocessing}On OPPORTUNITY DATASET}
% % \end{figure}
% % \begin{figure}[h]
% % \includegraphics[width=0.5\textwidth]{final_images/feature learning unimib shar.jpg}
% % \caption{\label{fig:postprocessing}ON UNIMIBSHAR}
% % \end{figure}
% % \begin{figure}[h]
% % \includegraphics[width=0.5\textwidth]{final_images/feature learning unimib shar results.jpg}
% % \caption{\label{fig:postprocessing}ON UNIMIBSHAR}
% % \end{figure}


% This paper [57] analyzes different feature extraction/representation approaches e.g., hand-crafted feature extraction methods, codebook, multi-layer perceptron, convolutional neural nets, recurrent neural nets - LSTM, hybrid convolutional and recurrent neural nets, and autoencoders. These approaches are implemented on Opportunity and UnimiB-SHAR datasets. The paper’s selected method is the hybrid
% CNN and LSTM model (Hybrid), with a weighted F1-score of 70.86 percent on the OPPORTUNITY dataset even with different sensor modalities with various window sizes T. Also, fusing the features learnt by hybrid method with codebook approach showed further improvement as well. \\

% Transition-Aware Detection of Modes of Locomotion and Transportation Through Hierarchical Segmentation\\

% This paper [69] proposes a platform using CNN which is trained on accelerometer and gyroscope data that is converted to 2D images to account for inter-axial dependencies and feature extraction as well as signals’ temporal characteristics. After segmentation with a sliding window of 1 minute long is applied on the sensory data, segmented data is fed into a 2-D CNN network directly to extract features. In parallel, it is fed into a feature extraction section to acquire the hand-crafted features with later is fed into a DNN with 128 neurons. In order to recognize different transportation locomotion mode, the segmented data’s PSD \zs{what is pSD?} \textcolor{red}{Farzad: power spectral density (PSD).
% The PSD is used as a feature to assist with distinguishing between challenging modes of motorized transportation that do not have a clear and distinct pattern in the time domain signals. e.g., standing in bus, standing in train} will be calculated and then is fed into a DNN with 128 neurons paralleled. The output of each flow is fed into This RNN is trained on the whole training dataset and learns the temporal order of activities. This RNN contains one layer with 25 long-short-term-memory (LSTM) neurons. The results are obtained on SHL dataset. Also, they proposed a search algorithm finds the transition time for change in modes transportation locomotion which reduces complexity of the algorithms compared to naïve search.
% Results are shown in three different scenarios: 
% Scenario1: Five classes as still, walk, run, bike, and vehicle. The vehicle class contains all car, bus, train, and subway activities.
% Scenario2: Six classes including still, walk, run, bike, road, and rail. The road class contains bus and car
% activities while the rail class contains train and subway activities.
% Scenario3: Eight classes considering each activity as a separate class.\\


% \begin{figure}[h]
% \includegraphics[width=0.5\textwidth]{final_images/scenarios.JPG}
% \caption{\label{fig:postprocessing}scenario}
% \end{figure}


% Environmental Features Recognition for Lower Limb Prostheses Toward Predictive Walking\\
% Sensors: IMU + Depth camera \zs{How is IMU sensor used in the framework?}\\
% Preproccessing: point cloud after offsetting + dimension reduction + binary image generation\\
% Contribution: experimental verification for the indoor and {outdoor experiments}.\\
% Network Architecture: This convolutional neural network included an image input layer, three convolutional layers, three batch normalization layers, three Relu layers, two max-pooling layers, a fully connected layer, a softmax layer,
% and a classification layer.\\
% Dataset: their own, the training dataset included 7500 images and each
% type of environments had 1500 images\\
% Classes: up stairs, down stairs, up ramp, down ramp, and level ground
% Results: The accuracy of classification results in simulation, indoor
% experiments, and outdoor experiments was 99.3percent for
% amputees, and 98.5percent amputee.\\

% Personal Authentication and Hand Motion Recognition based on Wrist EMG
% Analysis by a Convolutional Neural Network\\

% sensor: wrist EMG\\
% sampling rate: 1 KHz\\
% Preprocessing: removing hum noise, drift noise, outliers\\
% dataset: their own (hand motion recognition(3 classes) + personal authentication(8 classes))\\
% architecture: 3 conv + 1 reshape (flatten I think) + 2 fully connected \zs{Do they have pooling layers?}\\
% Accuracy: 94.6 percent hand motion, 95 percent personal authentication\\

% Toward Minimal-Sensing Locomotion Mode Recognition for a Powered Knee-Ankle Prosthesis\\
% sensors: IMU\\
% dataset: self-collected\\
% classes\\standing, walking on level ground, walking up and down ramps, and walking up and down stairs\\
% significance:This framework would potentially lead to less frequent clinical visits needed for sensor replacement and calibrations, which may save health care costs and the prosthesis user’s time and energy. \zs{Is this a benefit of all locomotion HAR app or just this paper? Did the author do anything special to gain this benefit?} \\
% Architecture: We use a DNN with three hidden layers, a stacked hidden layer, and
% an output layer. , rectified linear unit (ReLU) activation functions, and a softmax function\\




% \vspace{50pt}






























==> 5-3-rnn.tex <==
\subsection{Recurrent Neural Network (RNN)}
Initially, the idea of using temporal information was proposed in 1991 \cite{rnn4} to recognize a finger alphabet consisting of 42 symbols and in 1995 \cite{rnn21} to classify 66 different hand shapes with about 98\% accuracy. 
%%%%%%%%%%% PURE RNN
Since then, the recurrent neural network (RNN) with time series as input has been widely applied to classify human activities or estimate hand gestures \cite{rnn35, rnn6, rnn91, rnn95, rnn96, rnn104, rnn71}, \cite{alessandrini2021recurrent}. 

%%%%%%%%%%%%%% Structure of RNN
Unlike feed-forward neural networks, a RNN processes the input data in a recurrent behavior. Equivalent to a directed graph, RNN exhibits dynamic behaviors and possesses the capability of modeling temporal and sequential relationships due to a hidden layer with recurrent connections. A typical structure for an RNN is shown in Figure \ref{fig:RNN_LSTM} with the current input, $x_t$, and previous hidden state, $h_{t-1}$. The network generates the current hidden state, $h_t$, and output, $y_t$, is as follows:

\begin{equation}
\begin{array}{c}
h_{t}=\mathscr{F}\left(W_{h} h_{t-1}+U_{h} x_{t}+b_{h}\right) \\
y_{t}=\mathscr{F}\left(W_{y} h_{t}+b_{y}\right)
\end{array}
\end{equation}

where $W_{h}$, $U_{h}$, and $W_{y}$ are the weights for the hidden-to-hidden recurrent connection, input-to-hidden connection, and hidden-to-output connection, respectively. $b_h$ and $b_y$ are bias terms for the hidden and output states, respectively. Furthermore, each node is associated with an element-wise non-linearity function as an activation function $\mathscr{F}$ such as the sigmoid, hyperbolic tangent (tanh), or rectified linear unit (ReLU).



In addition, many researchers have undertaken extensive work to improve the performance of RNN models in the context of human activity recognition and have proposed various models based on RNNs, including Independently RNN (IndRNN) \cite{rnn5}, Continuous Time RNN (CTRNN) \cite{rnn17}, Personalized RNN (PerRNN) \cite{rnn64},  Colliding Bodies Optimization RNN (CBO-RNN) \cite{rnn58}. 
Unlike previous models with 1-dimension time-series input, \citet{rnn31} builds a CNN+RNN model with stacked multisensor data in each channel for fusion before feeding into CNN layer. 
\citet{rnn74} uses an RNN to address the domain adaptation problem, caused by intra-session, sensor placement, and intra-subject variances. 



%%%%%%%%%%%%%% Structure of LSTM
HAR improves with longer context information and longer temporal intervals. However, this may result in vanishing or exploding gradient problems while backpropagating gradients \cite{bengiogradient}.
In an effort to address these challenges, long short-term memory (LSTM)-based RNNs \cite{LSTM}, and Gated Recurrent Units (GRUs) \cite{GRU} are introduced to model temporal sequences and their broad dependencies. 
The GRU introduces a reset and update gate to control the flow of inputs to a cell \cite{rnn23,rnn28, rnn61, rnn48, rnn113}.
The LSTM has been shown capable of memorizing and modeling the long-term dependency in data. Therefore, LSTMs have taken a dominant role in time-series and textual data analysis. It has made substantial contributions to the field of human activity recognition, speech recognition, handwriting recognition, natural language processing, video analysis, etc. 
As illustrated in Figure \ref{fig:RNN_LSTM} \cite{rnn3}, a LSTM cell is composed of: (1). input gate, $i_t$, for controlling flow of new information; (2). forget gate, $f_t$, setting whether to forget content according to internal state; (3). output gate, $o_t$, controlling output information flow; (4). input modulation gate, $g_t$, as main input; (5). internal state, $c_t$, dictates cell internal recurrence; (6). hidden state, $h_t$, contains information from samples encountered within the context window previously. The relationship between these variables are listed as Equation \ref{equ:lstm} \cite{rnn3}. 

\begin{equation}
\left\{ 
\begin{array}{c}
i_{t}=\sigma\left(b_{i}+U_{i} x_{t}+W_{i} h_{t-1}\right) \\
f_{t}=\sigma\left(b_{f}+U_{f} x_{t}+W_{f} x_{t-1}\right) \\
o_{t}=\sigma\left(b_{o}+U_{o} x_{t}+W_{o} h_{t-1}\right) \\
g_{t}=\sigma\left(b_{g}+U_{g} x_{t}+W_{g} h_{t-1}\right) \\
c_{t}=f_{t} c_{t-1}+g_{t} i_{t} \\
h_{t}=\tanh \left(c_{t}\right) o_{t}
\end{array}
\right.
\label{equ:lstm}
\end{equation}


\begin{figure}[h!]
\centering
\captionsetup{justification=centering}
  \includegraphics[width=.67\linewidth]{rnn_img/rnn_lstm_structure.png}
  \caption{Schematic diagram of an RNN node and LSTM cell \cite{rnn3}. Left: RNN node where $h_{t-1}$ is the previous hidden state, $x_t$ is the current input sample data, $h_t$ is the current hidden state, $y_t$ is the current output, and $\mathscr{F}$ is the activation function. Right: LSTM cell with internal recurrence $c_t$ and outer recurrence $h_t$.}
  \label{fig:RNN_LSTM}
\end{figure}




As shown in Figure \ref{fig:lstm}, the input time series data is segmented into windows and fed into the LSTM model. For each time step, the model computes class prediction scores, which are then merged via late-fusion and used to calculate class membership probabilities through the softmax layer. 
Previous studies have shown that LSTMs have high performance in wearable HAR \cite{rnn61, rnn3, rnn76}.
Researchers in \cite{rnn19} rigorously examine the impact of hyperparameters in LSTM with the fANOVA framework across three representative datasets, containing movement data captured by wearable sensors. 
The authors assessed thousands of settings with random hyperparameters and provided guidelines for practitioners seeking to apply deep learning to their own problem scenarios \cite{rnn19}. Bidirectional LSTMs, having both past and future recurrent connections, were used in \cite{rnn30, rnn80} to classify activities.


\begin{figure}[h!]
\centering
\captionsetup{justification=centering}
  \includegraphics[width=0.8\linewidth]{rnn_img/lstm.png}
  \caption{The structure of LSTM and bi-directional LSTM model \cite{rnn19}. (a). LSTM network hidden layers containing LSTM cells and a final softmax layer at the top. (b) bi-directional LSTM network with two parallel tracks in both future (green) and past (red) directions.}
  \label{fig:lstm}
\end{figure}



Researchers have also explored other architectures involving LSTMs to improve benchmarks on HAR datasets. Residual networks possess the advantage that they are much easier to train as the addition operator enables gradients to pass through more directly. Residual connections do not impede gradients and could help to refine the output of layers. For example, \cite{rnn48} proposes a harmonic loss function and \cite{rnn16} combines LSTM with batch normalization to achieve 92\% accuracy with raw accelerometer and gyroscope data.
\cite{lstm7} proposes a hybrid CNN and LSTM model (DeepConvLSTM) for activity recognition using multimodal wearable sensor data. DeepConvLSTM performed significantly better in distinguishing closely-related activities, such as ``Open/Close Door" and ``Open/Close Drawer".
Moreover, Multitask LSTM is developed in \cite{lstm38} to first extract features with shared weight, and then classify activities and estimate intensity in separate branches. Qin \etal proposed a deep-learning algorithm that combines CNN and LSTM networks \cite{lstm114}. They achieved 98.1\% accuracy on SHL transportation modes classification dataset with CNN-extracted and hand-crafted features as input. Similarly, other researchers \cite{lstm25, lstm26, lstm12, lstm133, lstm130, lstm121, lstm100, lstm64}, \cite{saha2021deep} have also developed the CNN-LSTM model in varios application scenarios by taking advantage of the feature extraction ability of CNN and the time-series data reasoning ability of LSTM. 
\change{Interestingly, utilizing CNN and LSTM combined model, researchers in \cite{saha2021deep} attempt to eliminate sampling rate variability, missing data, and misaligned data timestamps with data augmentation when using multiple on-body sensors. Researchers in \cite{mekruksavanich2021placement} explored the placement effect of motion sensors and discovered that the chest position is ideal for physical activity identification.}



Raw IMU and EMG time series data are commonly used as inputs to RNNs \cite{rnn1, rnn26, rnn41, rnn55, rnn74, rnn121}. A number of major datasets used to train and evaluate RNN models have been created, including the Sussex-Huawei Locomotion-Transportation (SHL) \cite{rnn5, rnn28}, PAMAP2 \cite{rnn27, rnn31} and Opporunity\cite{rnn76}. In addition to raw time series data \cite{rnn61}, 
Besides raw time series data, custom features are also commonly used as inputs to RNNs. \cite{rnn23} showed that training a RNN with raw data and with simple custom features yielded similar performance for gesture recognition (96.89\% vs 93.38\%).

However, long time series may have many sources of noise and irrelevant information. 
The concept of attention mechanism was proposed in the domain of neural machine translation to address the problem of RNNs being unable to remember long-term relationships. The attention module mimics human visual attention to build direct mappings between the words/phrases that represent the same meaning in two languages. It eliminates the interference from unrelated parts of the input when predicting the output. This is similar to what we as humans perform when we translate a sentence or see a picture for the first time; we tend to focus on the most prominent and central parts of the picture. An RNN encoder attention module is centered around a vector of importance weights. The weight vector is computed with a trainable feedforward network and is combined with RNN outputs at all the time steps through the dot product. The feedforward network takes all the RNN immediate outputs as input to learn the weights for each time step. 
\cite{rnn113} utilizes attention in combination with a 1D CNN Gated Recurrent Units (GRUs), achieving HAR performances of 96.5\% ± 1.0\%, 93.1\% ± 2.2\%, and 89.3\% ± 1.3\% on Heterogeneous \cite{Heterogeneous}, Skoda \cite{Skoda}, and PAMAP2 \cite{PAMAP2} datasets, respectively. 
\cite{rnn27} applies temporal attention and sensor attention into LSTM to improve the overall activity recognition accuracy by adaptively focusing on important time windows and sensor modalities.


In recent years, block-based modularized DL networks are gaining traction. Some examples are GoogLeNet with an Inception module and Resnet with residual blocks. The HAR community is also actively exploring the application of block-based networks. In~\cite{innohar}, the authors have used GoogLeNet’s Inception module combined with a GRU layer to build a HAR model. The proposed model was showed performance improvements on three public datasets (Opportunity, PAMAP2 and Smartphones datasets). \change{\citet{qian2019novel} developed the model with $SMM_{AR}$ in statistical module to learn all orders of moments statistics as features, LSTM in spatial module to learn correlations among sensors placements, and LSTM+CNN in temporal module to learn temporal sequence dependencies along the time scale.
}










% \textbf{Farzad's papers:} \\
% \textcolor{blue}{Orange Labs Contribution to the Sussex-Huawei Locomotion-Transportation Recognition Challenge \zs{RNN}}\\
% \textcolor{blue}{In [41], Orange Labs proposed an LSTM and GRU recurrent neural network on Sussex-Huawei Locomotion Transportation (SHL) dataset. SHL dataset is created by using multi-model smartphone sensors. This dataset contains 8 modes of transportation in real-life settings with 3 different participants which is composed of 750 hours of labelled locomotion data i.e., Car (88 h), Bus (107 h), Train (115 h), Subway (89 h), Walk (127 h), Run (21 h), Bike (79 h), and still (127 h) in 2017. 
% The input data batch size is selected to include 32 observations and each observation is composed of a 2-dimensional signal \zs{which two dimensions?} of 500 time steps. The RNN network includes 2 bidirectional LSTM layers and each layer has 128 neurons. 
% The preliminary results show that the proposed method reaches the accuracy of 60.4 percent for the user transportation mode recognition by using hand validation data as testing data.}\\


==> 5-4-dbn.tex <==


\subsection{Deep Belief Network (DBN)}
%
%
A DBN, as illustrated in Fig. \ref{fig:fig_dbn}, is formed by stacking multiple simple unsupervised networks, where the hidden layer of the preceding network serves as the visible layer for the next. The representation of each sub-network is generally the restricted Boltzmann machine (RBM), which is an undirected generative energy-based model with a ``visible'' input layer, a hidden layer, and intra-layer connections in between. The DBN typically has connections between the layers but not between units within each layer. This structure leads to a fast and layer-wise unsupervised training procedure, where contrastive divergence (a training technique to approximate the relationship between a network's weights and its error) is applied to every pair of layers in the DBN architecture sequentially, starting from the ``lowest'' pair.
%

\begin{figure}[h!]
\centering
\captionsetup{justification=centering}
  \includegraphics[width= 0.7\linewidth]{img/fig_dbn.png}
  \caption{The greedy layer-wise training of DBNs. The first level is trained on triaxial acceleration data. Then, more RBMs are repeatedly stacked to form a deep activity recognition model \cite{DBN4}.
  }
  \label{fig:fig_dbn}
\end{figure}



The observation that DBNs can be trained greedily led to one of the first effective deep learning algorithms \cite{DBN0}. There are many attractive implementations and uses of DBNs in real-life applications such as drug discovery \cite{DBN8}, natural language understanding \cite{DBN9}, fault diagnosis \cite{DBN10}, etc. There are also many attempts to perform HAR with DBNs. In early exploratory work back in 2011 \cite{DBN1}, a 5-layer DBN is trained with the input acceleration data collected from mobile phones.
% , and the HAR recognition time is less than 0.15 ms for an data frame time of 1 s
The accuracy improvement ranges from 1\% to 32\% when compared to traditional ML methods with manually extracted features. %compared with 8 traditional ML methods
%
 
In later works, DBN is applied to publicly available datasets \cite{DBN2, DBN4, DBN7} \cite{mahmoodzadeh2021human}. In \cite{DBN2}, two 5-layer DBNs with different structures are applied to the Opportunity dataset \cite{Opportunity}, USC-HAD dataset \cite{USC-HAD}, and DSA dataset \cite{DSA}, and the results demonstrate improved accuracy for HAR over traditional ML methods for all the three datasets. Specifically, the accuracy for the Opportunity, USC-HAD, and DSA datasets are 82.3\% (1.6\% improvement over traditional methods), 99.2\% (13.9\% improvement), and 99.1\% (15.9\% improvement), respectively. 
% (REMOVE Heart Rate Monitoring from our scope)
% In \cite{DBN3}, the effectiveness of DBN is validated with the TROIKA dataset \cite{TROIKA} via a two-stage technique: 1) clustering individuals into different groups using partition around medoids (PAM); 2) performing biometric identification (gender, weight, current movement, etc.) using DBN with unsupervised training. The validation accuracy with TROIKA is as high as 96.1\%. 
In addition, Alsheikh \emph{et al.} \cite{DBN4} tested the activity recognition performance of DBNs using different parameter settings. Instead of using the raw acceleration data similar to \cite{DBN1}, they used spectrogram signals of the triaxial accelerometer data to train the deep activity recognition models. They found that deep models with more layers outperform the shallow models, and the topology of layers having more neurons than the input layer is shown to be more advantageous, which indicates overcompete representation is essential for learning deep models. The accuracy of the tuned DBN was 98.23\%, 91.5\%, and 89.38\% on the WISDM \cite{WISDM}, Daphnet \cite{Daphnet}, and Skoda \cite{Skoda} benchmark datasets, respectively. In \cite{DBN7}, a RBM is used to improve upon other methods of sensor fusion, as neural networks can identify non-intuitive predictive features largely from cross-sensor correlations and thus offer a more accurate estimation. The recognition accuracy with this architecture on the Skoda dataset reached 81\%, which is around 6\% higher than the traditional classification method with the best performance (Random Forest).
%

In addition to taking advantage of public datasets, there are also researchers employing DBNs on human activity or health-related recognition with self-collected datasets \cite{DBN2a, DBN5}. In \cite{DBN2a}, DBNs are employed in Parkinson's disease diagnosis to explore if they can cope with the unreliable labelling that results from naturalistic recording environments. The data was collected with two tri-axial accelerometers, with one worn on each wrist of the participant. The DBNs built are 2-layer RBMs, with the first layer as a Guassian-binary RBM (containing gaussian visible units) and the second layer as binary-binary (containing only binary units) (please refer to \cite{hinton2012practical} for details). In \cite{DBN5}, a unsupervised 5-layer DBM-DNN is applied for the automatic detection of eating episodes via commercial bluetooth headsets collecting raw audio signals, and demonstrate classification improvement even in the presence of ambient noise. The accuracy of the proposed DBM-DNN approach is 94\%, which is significantly better than SVM with a 75.6\% accuracy. 
% There are also research seeking to accurately determine the heart rate with DBN during intensive motion \cite{DBN6}, which is accomplished by classifying PPG signals obtained from smartphones or wearable devices combined with motion-related signals obtained from accelerometers.





==> 5-4-drl.tex <==
\subsection{Deep Reinforcement Learning (DRL)}

AE, DBN, CNN\changezs{, and RNN} fall within the realm of supervised or unsupervised learning. Reinforcement learning is another paradigm where an agent attempts to learn optimal policies for making decisions in an environment. At each time step, the \textit{agent} takes an \textit{action} and then receives a \textit{reward} from the \textit{environment}. The \textit{state} of the environment accordingly changes with the action made by the agent. The goal of the agent is to learn the (near) optimal policy (or probability of action, state pairs) through the interaction with the environment in order to maximize a cumulative long-term reward. The two entities - agent and environment, the three key elements - action, state and reward collectively form the paradigm of RL. The structure of RL is shown in Fig.~\ref{fig:rl}. 


\begin{figure}[!h]
\centering
\captionsetup{justification=centering}
  \includegraphics[width=0.56\columnwidth]{final_images/RL.png}
  \caption{A typical structure of a reinforcement learning network~\cite{rl-img}.}
  \label{fig:rl}
\end{figure}

% Arguably, supervised learning can be reduced to reinforcement learning. When viewing the classifier as an agent, the classifier giving a prediction to each sample as an action, and the evaluation of the prediction as the reward, supervised learning is transformed to be a simplified version or a specific case of reinforcement learning. 

In the domain of HAR, \cite{rl11} uses DRL to predict arm movements with 98.33\% accuracy.
\cite{rl2} developed a reinforcement learning model for imitating the walking pattern of a lower-limb amputee on a musculoskeletal model. The system showed 98.02\% locomotion mode recognition accuracy. Having a high locomotion recognition accuracy is critical because it helps lower-limb amputees prevent secondary impairments during rehabilitation.
In \cite{bhat2018online}, Bhat et al. propose an HAR online learning framework which takes advantage of reinforcement learning utilizing policy gradient algorithm for faster convergence achieving 97.7\% in recognizing 6 activities. 


==> 5-5-gan.tex <==
\subsection{Generative Adversarial Network (GAN)}
\label{sec:gan}



% \begin{figure*}[H]
% \centering
% \captionsetup{justification=centering}
%   \includegraphics[width=0.8\linewidth]{final_images/GAN.png}
%   \caption{The structure of generative adversarial network}
%   \label{fig:gan}
% \end{figure*}



% \yx{new}
Originally proposed to generate credible fake images that resembles the images in the training set, %with the same statistics as the training image set, 
GAN is a type of deep generative model, which is able to create new samples after learning from real data \cite{goodfellow2014generative}. 
It comprises two networks, the generator ($\mathbf{G}$) and the discriminator ($\mathbf{D}$), competing against each other in a zero-sum game framework as shown in Fig. \ref{fig:gan}. During the training phase, the generator takes as input a random vector $\mathbf{z}$ and transforms $\mathbf{z}\in \mathbb{R^\mathbf{n}}$ to plausible synthetic samples $\mathbf{\hat{x}}$ to challenge the discriminator to differentiate between original samples $\mathbf{x}$ and fake samples $\mathbf{\hat{x}}$. In this process, the generator strives to make the output probability $\mathbf{D(G(z))}$ approach one, in contrast with the discriminator, which tries to make the function's output probability as close to zero as possible. The two adversarial rivals are optimized by finding the Nash equilibrium of the game in a game zero-sum setting which means the adversarial rivals' gains would be maintained regardless of what strategies are selected. However, it is not theoretically guaranteed that GAN zero-sum games reach Nash Equilibria \cite{farnia2020gans}.



GAN model has shown remarkable performance in generating synthetic data with high quality and rich details. In the field of HAR, GAN has been applied as a semi-supervised learning approach to deal with unlabeled or partially labeled data for improving performance by learning representations from the unlabeled data which later will be utilized by the network to generalize to the unseen data distribution \cite{madani2018semi, springenberg2015unsupervised, odena2016semi} \cite{shi2021gan}, \cite{wang2021multimodal}. 
Afterward, GAN has shown the ability to generate balanced and realistic synthetic sensor data. 
\cite{gan12} utilizes GANs with a customized network to generate synthetic data from the public HAR dataset HASC2010corpus \cite{HASC2011corpus}. 
Similarly, \cite{gan78} assesses synthetic data with CNN or LSTM models as a generator. In two public datasets, Sussex-Huawei Locomotion (SHL) and Smoking Activity Dataset (SAD), the discriminator is built with CNN layers, and the results demonstrate synthetic data with high quality and diversity with two public datasets. Moreover, by oversampling and adding synthetic sensor data into the training, researchers augment and alleviate the originally imbalanced training set to achieve better performance. 
\cite{gan26, gan69} generate verisimilar data of different activities and \cite{gan27} uses the Boulic kinematic model which aims to capture the three dimensional positioning trend to synthesize personified walking data.
%%%%%
\change{Due to the ability of generating new data, GAN has been widely applied in transfer learning in HAR to help with the dramatic performance drop when the pre-trained model are tested against unseen data from new users.
In transfer learning techniques, the learned knowledge from the source domain (subject) is transferred to the target domain to decrease the lack of performance of the models within the target domain. 
Moreover, \cite{gan6} is an attempt that utilizes GAN to perform cross-subject transfer learning for HAR since collecting data for each new user is infeasible. 
With the same idea, cross-subject transfer learning based on GAN outperformed those without GAN on Opportunity benchmark dataset in \cite{soleimani2021cross} and outperformed unsupervised learning on UCI and USC-HAD dataset \cite{abedin2021guidedgan}. Even more, transfer learning under conditions of cross-body, cross-user, and cross-sensor has been demonstrated superior performance in \cite{sanabria2021contrasgan}.}



However, much more effort is needed in generating verisimilar data to alleviate the burden and cost of collecting sufficient user data.
Additionally, it is typically challenging to obtain well-trained GAN models owing to the wide variability in amplitude, frequency, and period of the signals obtained from different types of activities.




% \end{paracol}
\begin{figure}[h!]	
\centering
\includegraphics[width=0.83\linewidth]{final_images/GAN.png}
\caption{The structure of generative adversarial network.}
\label{fig:gan}
\end{figure}  
% \begin{paracol}{2}
% \linenumbers
% \switchcolumn




==> 5-6-hybrid.tex <==
\subsection{\change{Hybrid Models}}
\label{sec:hybrid}

\change{
As an advancement of machine learning models, researchers take advantage of different methods and propose hybrid models.
The combination of CNN and LSTM endows the model capability of extracting local features as well as long-term dependencies in sequential data, especially for HAR time series data. For example, \citet{challa2021multibranch} proposed a hybrid of CNN and bidirectional long short-term memory (BiLSTM). The accuracy on UCI-HAR, WISDM\cite{WISDM}, and PAMAP2\cite{PAMAP2} datasets achieved 96.37\%, 96.05\%, and 94.29\%, respectively. \citet{dua2021multi} proposed a model with CNN combined with GRU and obtained accuracy of 96.20\%, 97.21\%, and 95.27\% on UCI-HAR, WISDM\cite{WISDM}, and PAMAP2\cite{PAMAP2} datasets, respectively.
% 
In order to have a straightforward view of the functionality of hybrid models, we list several papers with CNN only, LSTM only, CNN+GRU, and CNN+LSTM in Table \ref{tab:UCI-HAR_hybrid} and Table \ref{tab:PAMAP2_hybrid}.
In addition, \citet{zhang2018multi} proposed to combine reinforcement learning and LSTM model to improve the adaptability of different kinds of sensors including EEG (EID dataset), RFID (RSSI dataset)\cite{yao2017compressive}, and wearable IMU (PAMAP2 dataset)\cite{PAMAP2}.
\cite{zhang2019know} employed CNN for feature extraction and a reinforced selective attention model to automatically choose the most characteristic information from multiple channels.
}

\begin{table*}[ht]
\centering
\captionsetup{justification=centering}
    \resizebox{\linewidth}{!}{
\begin{minipage}{.5\linewidth}
    \captionsetup{justification=centering}
     \caption{\change{Comparison of models on\\ UCI-HAR dataset}}
    \begin{tabular}{lcc}
    \toprule
    Model & F1-Score (\%) & Accuracy (\%)  \\
    \midrule
    CNN \cite{wan2020deep} &	92.93 &	92.71 \\
    Res-LSTM \cite{zhao2018deep} & 91.50 & 91.60  \\
    Stacked-LSTM \cite{ullah2019stacked} &	-- &	93.13 \\
    CNN-LSTM \cite{mutegeki2020cnn} & -- &	92.13 \\
    Bidir-LSTM \cite{hernandez2019human}  &	-- &	92.67 \\
    Residual-BiLSTM \cite{zhao2018deep} &	93.5 &	93.6 \\
    LSTM-CNN \cite{xia2020lstm}  &	-- &	95.78 \\ 
    % Dilated-TCN &	93.8 &	93.8 \\
    CNN‑GRU \cite{dua2021multi} &	-- & 96.20 \\
    CNN‑GRU \cite{challa2021multibranch} &	94.54 & 94.58 \\
    CNN-LSTM \cite{challa2021multibranch} & 94.76 & 94.80 \\
    CNN‑BiLSTM \cite{challa2021multibranch} &	96.31 &	96.37 \\
    \bottomrule
    \end{tabular}
    \label{tab:UCI-HAR_hybrid}
\end{minipage}
\begin{minipage}{.5\linewidth}
    \captionsetup{justification=centering}
     \caption{\change{Comparison of models on\\ PAMAP2 dataset}}
    \begin{tabular}{lcc}
    \toprule
    Model & F1-Score (\%) & Accuracy (\%)  \\
    \midrule
    CNN\cite{wan2020deep} & 91.16 & 91.00 \\
    BiLSTM \cite{hernandez2019human} & 89.40 & 89.52   \\
    % ARC-NET  &	90.76  &90.91 \\
    LSTM-F \cite{hammerla2016deep}  &	 92.90  & -- \\
    COND-CNN \cite{cheng2020real} &	--  &94.01 \\
    CNN‑GRU \cite{dua2021multi} & 	-- & 95.27 \\
    CNN‑GRU  \cite{challa2021multibranch} &	93.16 & 93.20 \\
    CNN-LSTM \cite{challa2021multibranch} & 92.77 & 92.81 \\
    CNN‑BiLSTM \cite{challa2021multibranch} &	94.27  & 94.29 \\
    \bottomrule
    \end{tabular}    
    \label{tab:PAMAP2_hybrid}
\end{minipage}
}
\end{table*}













==> 5-7-benchmark.tex <==
% \subsection{\textcolor{red}{Benchmarking on Public Datasets}}
% \label{sec:Benchmark}

% \change{Traditionally, there are a large number of application scenarios and contexts, thus it is difficult to make a head-to-head performance comparison of different approaches. Owing to the popularity of public datasets in HAR field, we could possibly evaluate these different approaches easily on a standard test bed. Here we compare different DL approaches in aspect of the prediction performance with two selected public datasets - \textit{Opportunity} and \textit{Skoda} as shown in Fig.~\ref{fig:opp_gesture_papers} and \ref{fig:skoda_papers}. As we can observe from the figure, the F1 score achieve 88\% in 2016 since the development of CNN model. Afterwards, the models combing CNN and LSTM outperform CNN only with F1 score of over 90\%. Similar trends can also be observed from the performance of Skoda dataset in Fig. \ref{fig:skoda_papers}.
% }
% % \textcolor{red}{(TO CONTINUE}


% %
% \begin{figure}
% \centering
%   \includegraphics[width=0.75\columnwidth]{img/opp_gesture.pdf}
%   \caption{Performance (weighted F1-Score) comparison on Opportunity (gesture) dataset. \textcolor{red}{(NEEDS MODIFICATION)}}~\label{fig:opp_gesture_papers}
% \end{figure}
% %

% \begin{figure}
% \centering
%   \includegraphics[width=0.75\columnwidth]{img/skoda.pdf}
%   \caption{Performance (weighted F1-Score) comparison on Skoda dataset. \textcolor{red}{(NEEDS MODIFICATION)}}~\label{fig:skoda_papers}
% \end{figure}
%

\subsection{Summary and Selection of Suitable Methods }
% \textcolor{green}{Stephen - How about this?}
\label{sec:summary}

\change{
Since the last decade, DL methods have gradually dominated a number of artificial intelligence areas, including sensor-based human activity recognition, due to its automatic feature extraction capability, strong expressive power, and the high performance rendered. 
% 
When a sufficient amount of data are available, we are becoming prone to turn to DL methods. 
% 
With all these types of available DL approaches discussed above, we need to get a full understanding of the pros and cons of these approaches in order to select the appropriate approach wisely. To this end, we briefly analyze the characteristics of each approach and attempt to give readers a high-level guidance of how to choose the DL approach according to the needs and requirements.} 

\change{The most salient characteristic of auto-encoder is that it does not require any annotation. Therefore, it is widely adopted in the paradigm of unsupervised learning. Due to its exceptional capability in dimension reduction and noise suppression, it is often leveraged to extract low-dimensional feature representation from raw input. However, auto-encoders may not necessarily learn the correct and relevant characteristics of the problem at hand. There is also generally little insight that can be gained for sensor-based auto-encoders, making it difficult to know which parameters to adjust during training.
% 
Deep belief networks are a generative model generally used for solving unsupervised tasks by learning low-dimensional features. Today, DBNs have been less often chosen compared with other DL approaches and are rarely used due to the tedious training process and increased training difficulty with DBN when the network goes deeper~\cite{Goodfellow-et-al-2016}.
}

\change{ 
CNN architecture is powerful to extract hierarchical features owing to its layer-by-layer hierarchical structure. 
When compared with other approaches like RNN and GAN, CNN is relatively easy to implement. 
Besides, as one of the most studied DL approaches in image processing and computer vision,  there are a large range of CNN variants existing that we can choose from to transfer to sensor-based HAR applications. 
When sensor data are represented as 2-dimensional input, we can directly start with pre-trained models on large image dataset (e.g., ImageNet) to fasten the convergence process and achieve better performance. 
% 
Therefore, adapting CNN approach enjoys the high degree of flexibility in the available network architecture (e.g., GoogLeNet, MobileNet, ResNet, etc) than other DL approaches.
% 
However, CNN architecture has the requirement of fixed-sized input, in contrast to RNN which accepts flexible input size.
% 
% ... More CONS of CNN?
In addition, compared with unsupervised learning methods such as auto-encoder and DBN, a large number of annotated data are required, which usually demands expensive labeling resource and human effort to prepare the dataset. 
% 
The biggest advantage of RNN and LSTMs is that they can model time series data (nearly all sensor data) and temporal relationships very well. Additionally RNN and LSTMs can accept flexible input data size. The factors that prevent RNN and LSTMs from becoming the defacto method in DL-based HAR is that they are difficult to train in multiple aspects. They require long training time and are very susceptible to diminishing/exploding gradients. It is also difficult to train them to efficiently model long time series.
}

\change{
GAN, as a generative model, can be used as a data augmentation method. Because it has strong expressive capability to learn and imitate the latent data distribution of the targeted data, it outperforms traditional data augmentation methods~\cite{parkinson_augmentation}. 
% 
Owing to its inherent data augmentation ability, GAN has the advantage of alleviated data demands at the beginning. 
%
However, GAN is often considered as hard to train because it alternatively trains a generator and a discriminator. Many variants of GAN and special training techniques have been proposed to tackle the converging issue~\cite{arjovsky2017wasserstein, gulrajani2017improved, che2016mode}.
}

\change{
Reinforcement learning is a relatively new area that is being explored for select areas in HAR, such as modeling muscle and arm movements~\cite{rl11, rl2}. Reinforcement learning is a type of unsupervised learning because it does not require explicit labels. Additionally, due to its online nature, reinforcement learning agents can be trained online while deployed in a real system. However, reinforcement learning agents are often difficult and time-consuming to train. Additionally, in the realm of DL-based HAR, the reward of the agent has to be given by a human, as in the case of~\cite{rl11,bhat2018online}. In other words, even though people do not have to give explicit labels, humans are still required to provide something akin to a label (the reward) to train the agent.
}

\change{
When starting to choose a DL approach, we have a list of factors to consider, including the complexity of target problem, dataset size, the availability and size of annotation, data quality, available computing resource, as well as the requirement of training time. 
% 
% === complexity of targeted problem ===
Firstly, we have to evaluate and examine the problem complexity to decide upon promising venues of machine learning methods. For example, if the problem is simple enough to resolve with the provided sensor modality, it's very likely that manual feature engineering and traditional machine learning method can provide satisfying results thus no DL method is needed. 
% 
% === dataset size ===
Secondly, before we choose the routine of DL, we would like to make sure the dataset size is sufficient to support a DL method. 
The lack of a sufficiently large corpus of labeled high-quality data is a major reason why DL methods cannot produce an expected result.
Normally, when training a DL model with a limited size of dataset, the model will be prone to overfitting and the generalizability will be sacrificed, thus using a very deep network may not be a good choice. One option is to go for a shallow neural network or a traditional ML approach. Another option is utilize specific algorithms to make the most out of the data. To be specific, data augmentation methods such as GAN can be readily implemented.
% 
% === availability and size of annotation ===
Thirdly, another determining factor is the availability and size of annotation. When there are a large corpus of unlabeled sensor data at hand, semi-supervised learning scheme is a promising direction one could consider, which will be discussed later in this work. 
% 
% === data quality ===
Besides the availability of sensor data, the data quality also influences the network design. If the sensor is vulnerable to environmental noise, inducing a small SNR, some type of denoising structure (e.g., denoising auto-encoder) and increasing depth of the model can be considered to increase the noise-resiliency of the DL model.
% 
% === available computing resource and the requirement of training time
At last, a full evaluation of available computing resources and expected model training time cannot be more important for developers and researchers to choose a suitable DL approach.
}

==> 5-dataset.tex <==
\subsection{Major Datasets} \label{sec:dataset}
%
%
\begin{table*}[]
\centering
\captionsetup{justification=centering}
    \caption{Major Public Datasets for Wearable-based HAR}
    \resizebox{\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
Dataset & Application & Sensor & \# Classes & Spl. Rate & Citations/yr \\
\midrule
WISDM \cite{WISDM} & Locomotion & 3D Acc. & 6 & 20 Hz &  217 \\
ActRecTut \cite{ActRecTut} & Hand gestures & 9D IMU & 12 & 32 Hz & 153 \\
UCR(UEA)-TSC \cite{UCRArchive, UEA} & 9 datasets (e.g., uWave \cite{uWave}) & Vary & Vary & Vary & 107* \\ %UCR(UEA)-TSC Archive 
UCI-HAR \cite{UCI-HAR} & Locomotion & Smartphone 9D IMU  & 6 & 50 Hz & 78 \\
Ubicomp 08   \cite{Ubicomp_08} & Home activities &  Proximity sensors & 8 & N/A & 69 \\
% TROIKA \cite{TROIKA} & Heart rate monitoring & PPG, ECG, 3D Acc. &  6 & 125 Hz & 55  \\
SHO  \cite{SHO} & Locomotion & Smartphone 9D IMU & 7 & 50 Hz & 52 \\
UTD-MHAD1/2  \cite{UTD-MHAD1/2} & Locomotion \& activities & 3D Acc. \& 3D Gyro. & 27 & 50 Hz & 39 \\
HHAR \cite{Stisen} & Locomotion & 3D Acc. & 6 & 50--200 Hz & 37 \\
Daily \& Sports Activities \cite{DSA} & Locomotion & 9D IMU & 19 & 25 Hz & 37  \\
MHEALTH  \cite{mHealth1, mHealth2} & Locomotion \& gesture & 9D IMU \& ECG & 12 & 50 Hz & 33 \\
Opportunity \cite{Opportunity} & Locomotion \& gesture  & 9D IMU & 16 & 50 Hz & 32 \\
PAMAP2 \cite{PAMAP2} & Locomotion \& activities & 9D IMU \& HR monitor & 18 & 100 Hz & 32 \\
Daphnet \cite{Daphnet} & Freezing of gait & 3D Acc. & 2 & 64 Hz & 30 \\
SHL  \cite{SHL} & Locomotion \& transportation & 9D IMU & 8 & 100 Hz & 23 \\
SARD \cite{SARD} & Locomotion & 9D IMU \& GPS & 6 & 50 Hz & 22 \\
Skoda Checkpoint \cite{Skoda} & Assembly-line activities & 3D Acc. & 11 & 98 Hz & 21 \\
UniMiB SHAR \cite{SHAR} & Locomotion \& gesture & 9D IMU & 12 & N/A & 20 \\
USC-HAD \cite{USC-HAD} & Locomotion & 3D ACC. \& 3D Gyro. &  12 & 100 Hz & 20 \\
ExtraSensory \cite{ExtraSensory} & Locomotion \& activities & 9D IMU \& GPS & 10 & 25--40 Hz & 13 \\
HASC \cite{HASC} & Locomotion & Smartphone 9D IMU & 6 & 100 Hz & 11 \\
% BreathPrint \cite{BreathPrint} & Breathing activities & Smartphone audio & 3 & 8 kHz & 9 \\
Actitracker  \cite{Actitracker} & Locomotion & 9D IMU \& GPS & 5 & N/A & 6 \\
FIC \cite{FIC} & Feeding gestures  & 3D Acc. & 6 & 20 Hz & 5 \\
WHARF  \cite{WHARF} & Locomotion & Smartphone 9D IMU & 16 & 50 Hz & 4 \\
\bottomrule
\end{tabular}
}
\label{tab:datasets}
\end{table*}
%
%

We list the major datasets employed to train and evaluate various ML and DL techniques in Table~\ref{tab:datasets}, ranked based on the number of citations they received per year according to Google Scholar. 
% All of the three-star datasets have been cited more than 200 times, indicating a particularly vibrant and concentrated research focus in the field of HAR. 
As described in the earlier sections, most datasets are collected via IMU, GPS, or ECG. While most datasets are used to recognize physical activity or daily activities \cite{Opportunity, USC-HAD, UCI-HAR, DSA, TROIKA, SHO, WISDM, WHARF, HASC, SARD, Stisen, mHealth1, mHealth2, UTD-MHAD1/2, ExtraSensory, SHAR, Actitracker, PAMAP2, Ubicomp_08}, there are also a few datasets dedicated to hand gestures~\cite{ActRecTut, FIC}, breathing patterns~\cite{BreathPrint}, and car assembly line activities \cite{Skoda}, as well as those that monitor gait for patients with PD \cite{Daphnet}.
%
% \end{paracol}
\begin{figure}%[h!]
% \widefigure
\centering
\captionsetup{justification=centering}
  \includegraphics[width= 0.9\linewidth]{img/HAR_diagram.pdf}
  \caption{Placement of inertia sensors in different datasets: (a) WISDOM; (b) ActRecTut; (c) UCI-HAR; (d) SHO; (e) PAMAP2; and (f) Opportunity.}
  \label{fig:location}
\end{figure}
% \begin{paracol}{2}
% \linenumbers
% \switchcolumn

% %
% %\end{paracol}
% \begin{figure}
% \centering
% \captionsetup{justification=centering}
%   \includegraphics[width=\linewidth]{img/HAR_location.pdf}
%   \caption{Placement of inertia sensors in different datasets: (a) WISDOM; (b) ActRecTut; (c) UCI-HAR; (d) SHO; (e) PAMAP2; and (f) Opportunity.}~\label{fig:location}
% \end{figure}
% %\begin{paracol}{2}
% %\linenumbers
% %\switchcolumn


Most of the datasets listed above are publicly available. The University of California Riverside-Time Series Classification (UCR-TSC) archive is a collection of datasets collected from various sensing modalities \cite{UCR}. The UCR-TSC archive was first released and included 16 datasets, which grew to 85 datasets by 2015 and to 128 by October 2018. Recently, researchers from the University of East Anglia have collaborated with UCR to generate a new collection of datasets, which includes 9 categories of HAR: \textit{BasicMotions}, \textit{Cricket}, \textit{Epilepsy}, \textit{ERing}, \textit{Handwriting}, \textit{Libras}, \textit{NATOPS}, \textit{RacketSports}, and \textit{UWaveGestureLibrary} \cite{UEA}.
One of the most commonly used datasets is the OPPORTUNITY dataset \cite{Opportunity}. This dataset contains data collected from 12 subjects using 15 wireless and wired networked sensor systems, with 72 sensors and 10 modalities attached to the body or the environment. 
Existing HAR papers mainly focus on data from on-body sensors, including 7 IMUs and 12 additional 3D accelerometers for classifying 18 kinds of activities. Researchers have proposed various algorithms to extract features from sensor signals and to perform activity classification using machine-learned models like K Nearest Neighbor (KNN) and SVM \cite{knn_har1, knn_har2, SVM_har1, cnn5, cnn9, cnn17, cnn57, cnn61, cnn84, cnn115}.
% \textcolor{red}{[X, X, X, X, 5, 9, 17, 57, 61, 84, 115]}.
Another widely-used dataset is PAMAP2 \cite{PAMAP2}, which is collected from 9 subjects performing 18 different activities, ranging from jumping to house cleaning, with 3 IMUs (100-Hz sampling rate) and a heart rate monitor (9 Hz) attached to each subject. Other datasets such as Skoda \cite{Skoda} and WISDM \cite{WISDM} are also commonly used to train and evaluate HAR algorithms.


==> 5-dl_by_domain.tex <==
\section{Deep Learning Approaches} \label{sec:deeplearning}


% \subsection{The Emergence of Deep Learning}
%

With the tremendous opportunities afforded by HAR applications come the challenges of inferring human activities from sensor data. Traditional machine learning approaches have exhibited promising results in many different scenarios. However, they still leave room for improvement to the aim of an industry-level product with full readiness to deploy. 

In recent years, deep learning approaches outperformed classical machine learning approaches in a wide range of HAR tasks in many domains such as computer vision, speech recognition, and natural language processing~\cite{nature_dl}. Specifically, deep learning techniques support the development of much larger and more powerful models that deal with unstructured environments and raw sensor observations. 
With the capability of modeling complex non-linear relationship in data, deep learning is the best fit for complicated and challenging HAR problems. This can be attributed to its ability to leverage more parameters and build more sophisticated models, which distinguishes deep learning approaches from conventional machine learning techniques. 
% As an example, being both belonging to sequential models, RNN is much more powerful than Hidden Markov Model (HMM) in multiple domains, including natural language processing, speech recognition and HAR.  (This sentence can possibly be removed. But if not, cite it.)
There are 3 key factors behind the rapid popularity and prevalence of deep learning: increasingly available data, hardware acceleration, and algorithmic advancements. Data-wise, the data explosion and the emergence of the crowdsource-based data annotation mechanism provide the oppotunity to learn the hidden pattern and ?? from In hardware aspect, the prevalent usage of GPUs in training neural networks has ????.



Provided with a sufficient amount of annotated data, DL algorithms have achieved the state-of-the-art performance in almost all of its applied areas (if there is any exception). 
% Automatic feature extraction: No need for feature engineering. 
Traditional machine learning algorithms usually call for sophisticated manual feature engineering which unavoidably involves expert domain knowledge and numerous human effort. However, when using a deep network, the representative features can be learnt automatically through supervised or unsupervised paradigm. 
% as one can just pass the data directly to the network and usually achieve good performance right off the bat. 
This eliminates the requirements for human expertise in very specific domains and tedious manual feature engineering. 
%
\textcolor{red}{(This section goes back to the very high level writing style of explaining what deep learning is: but a few paragraphs before we were discussing image optical flow, crowdsourced labeling, and lots of other complex concepts that a reader at this level would not understand. If they do understand- then this kind of material is obvious to them. So perhaps we can discuss what our target audience should be for this paper and adapt accordingly.)}
%

\subsection{Auto-encoder}
%
%
\begin{figure}
\centering
  \includegraphics[width=0.9 \columnwidth]{img/fig_ae}
  \caption{Illustration of an auto-encoder network~\cite{gan2018synthesizingAR}.}~\label{fig:fig_ae}
\end{figure}
%
%

The Auto-encoder was first proposed in 1980s as a method of unsupervised pre-training method for ANN ~\cite{AE0}, although originally it was called 'autoassociative learning module', not exactly the same terminology we are using today. After evolving for decades, auto-encoder has become widely adopted as an unsupervised feature learning method and a greedy layer-wise neural network pre-training method. 
%

The training process of a one hidden layer auto-encoder is illustrated in Fig. \ref{fig:fig_ae}. An auto-encoder is trained from an ANN, which composes of two parts: the encoder and the decoder. The output of the encoder is fed into the decoder as input. The ANN takes the mean square error between the original input and output as a loss function, which essentially aims at imitating the input as the final output. After this ANN is trained, the decoder part is dropped and the encoder part is kept. Therefore the output of the encoder is the feature representation that can be employed in the next-stage classifiers.
%

The auto-encoder has been widely used as a powerful dimension reduction and information retrieval tool, in part due to its efficacy at reducing signal noise. Several research efforts have been carried out to deploy auto-encoders on HAR with wearable sensors \cite{AE1, AE2, AE3, AE4, AE5, AE6, AE7, AE8}. One such effort is presented in \cite{AE1}, where a sparse auto-encoder and denoising auto-encoder are used to explore useful feature representations from accelerometer and the gyroscope sensor data, and perform classification using Support Vector Machines. Experiments were performed on a public HAR dataset \cite{UCI-HAD} from the UCI repository, and the classification accuracy is compared with that of FFT in the frequency domain and PCA. The result reveals the stacked auto-encoder has the highest accuracy of 92.16\% and brings a 7\% advantage over the traditional methods with hand-crafted features. 
%
% In addition to sensors that can be directly worn or attached to the human body, which some people may not feel comfortable with in their daily life, the (I don't think this is the best place to describe differences between on-skin vs. on-clothing HAR. Just segue into another application of using autoencoders)
Microsoft Research AI Lab investigated the use of sensors integrated into common pieces of clothing for HAR \cite{AE3}. However, they've found that signals in such free-mode sensor networks can be contaminated  with motion artifacts leading to the signal-to-noise ratio (SNR) as low as -12 dB. To fully leverage the data collected by these free-mode sensors, a deconvolutional sequence-to-sequence auto-encoder (DSTSAE) is proposed, and its parameters are trained using a weighted-variant of the standard variational auto-encoder (VAE) framework. The experimental result indicates that the DSTSAE is able to effectively alleviate motion artifacts in free-mode sensors and shows that it outperforms the traditional Kalman Filter with a higher average SNR improvement of 11.92 dB. Additionally, instead of feeding the auto-encoder with raw sensor measurements, the work presented in \cite{AE2} conducted some pre-processing techniques on the same public HAR dataset \cite{UCI-HAD} as the one used in \cite{AE1}, the proposed approach includes median filters for noise reduction and Butterworth low-pass filters for separating the body acceleration and gravity. Finally, fixed-width sliding windows of 2.56 sec and 50\% overlap are employed, and the output is fed into a stacked auto-encoder, which enables the classification accuracy to increase by 1\% and the average recognition time to be reduced by around tenfold. \textcolor{red}{(Is the intention to discuss the details of their implementation in this section, or specifically the use of autoencoders?)} Another similar work is reported in \cite{AE8} to identify three typical HAR application scenarios in the UCI dataset \cite{UCI-HAD}, which are human moving modes, current static, and dynamic behaviors of users. Specifically, the stacked denoising auto-encoder is used to sanitize the noise in raw sensor data and extract the most effective characteristic expression with unsupervised learning, and the LightGBM (LGB) is applied to reveal the inherent feature dependencies among categories for accurate activity recognition.


Besides daily activities, auto-encoders are also widely used in recognizing \textcolor{red}{physiological activities}, such as the abnormal muscular movements as a result of the Parkinson's Disease and Autism Spectrum Disorder (ASD). Specifically, the stereotypical motor movement (SMM) dataset \cite{SMM} collected from 6 individuals with ASD and the Daphnet Freezing of Gait dataset \cite{Daphnet} are used in this study. The denoising auto-encoder is used to reconstruct the original IMU signals and extract optimized features of normal movements from their noisy versions, and a one-class SVM is used for detecting anomalies \cite{AE4}.   


Despite the success of recognizing human activities with data collected from many wearable sensors, a wide range of potentially sensitive information may be also revealed in an unintentional manner to the users themselves. For example, it may be non-sensitive to interpret some daily activities such as walking, jogging, and running, but sometimes it's not the case for drinking, smoking, or using the restroom. In order to extract the necessary non-sensitive information for accurate activity recognition while protecting individuals’ privacy, a novel replacement auto-encoder is proposed in \cite{AE5}, in which the sensitive sections of the time-series wearable sensor measurement can be safely replaced with non-sensitive real sections in a way that no information about the replacement operation could leak to the other party. As an extension of the classical denoising auto-encoder, the replacement auto-encoder is trained to produce a non-sensitive output from a sensitive input via stochastic replacement, while keeping other types of input unchanged. Extensive experiments are performed on Opportunity \cite{Opportunity}, Skoda \cite{Skoda}, and Hand-Gesture \cite{ActRecTut} datasets, and the result shows that the  proposed replacement auto-encoder can retain the recognition accuracy of state-of-the-art techniques while simultaneously preserving the privacy of sensitive information. Another work \cite{AE6} attempts to recognize an activity without disclosing a participant's gender due to privacy concerns. The specific framework of the algorithm is a Guardian-Estimator-Neutralizer (GEN), which is designed to share only a transformed version of the sensor data based on privacy considerations. The Guardian, which is constructed by a deep denoising auto-encoder, provides an inference-specific transformation. The Estimator is composed of a multitask convolutional neural network that guides the Guardian by estimating sensitive and non-sensitive information in the transformed data, while the Neutralizer is an optimizer that helps the Guardian converge to a near-optimal transformation function. Both the publicly available MobiAct \cite{MobiAct} and a new dataset MotionSense are used to evaluate the efficacy of the proposed privacy-enhancement method. Experimental results demonstrate that the proposed framework is able to maintain the usefulness of the transformed data for activity recognition, while reducing the possibility of gender classification to around the random guess of 50\%, from more than 90\% when using raw sensor data \cite{AE6}. Similarly, the same authors have proposed another anonymizing auto-encoder in \cite{AE7}. Different from the training process of the classical auto-encoder that only preserves the encoder part as the output feature representation while dropping the decoder part, this paper preserves both the encoder and the decoder output for data transformation. Experiments performed on a self-collected dataset from the accelerometer and gyroscope showcased a promising trade-off between utility and privacy, with an accuracy for activity recognition above 92\% and an accuracy for user identification below 7\%.

% (A shallow auto-encoder is proved to have a similar paradigm as PCA. [cite])


\subsection{Deep Belief Network (DBN)}
%
%
\begin{figure}
\centering
  \includegraphics[width= 0.9\columnwidth]{img/fig_dbn.png}
  \caption{The greedy layer-wise training of DBNs. The first level is trained on triaxial acceleration data. Then, more RBMs are repeatedly stacked to form a deep activity recognition model until forming a high-level representation~\cite{DBN4}.}~\label{fig:fig_dbn}
\end{figure}
%
%

A deep belief network (DBN), as illustrated in Fig. \ref{fig:fig_dbn}, is formed by stacking multiple simple unsupervised networks, where the hidden layer of the preceding network serves as the visible layer for the next. The representation of each sub-network is generally the restricted Boltzmann machine, which is an undirected generative energy-based model with a ``visible'' input layer, a hidden layer, and intra-layer connections in between. This structure leads to a fast and layer-wise unsupervised training procedure, where contrastive divergence is applied to every pair of layers in the DBN architecture sequentially, starting from the ``lowest'' pair.
%

The observation that DBNs can be trained greedily led to one of the first effective deep learning algorithms \cite{DBN0}. There are many attractive implementations and uses of DBNs in real-life applications such as drug discovery, natural language understanding, fault diagnosis, etc. There are also many attempts to perform HAR with DBNs, in an early exploratory work back in 2011 \cite{DBN1}, a 5-layer DBN is trained with the input acceleration data collected from mobile phones
% , and the HAR recognition time is less than 0.15 ms for an data frame time of 1 s
. The accuracy improvement ranges from 1\% to 32\% when compared to traditional ML methods with manually extracted features. %compared with 8 traditional ML methods
%
 
In later works, DBN has been also applied to publicly available datasets \cite{DBN2, DBN4, DBN7}. In \cite{DBN2}, two 5-layer DBNs with different structures are applied to the Opportunity dataset \cite{Opportunity}, USCHAD dataset \cite{USC-HAD}, and DSA dataset \cite{DSA}, and the results demonstrate better accuracy for HAR when compared with traditional ML methods for all the three datasets. Specifically, the accuracy for the Opportunity, USCHAD, and DSA datasets are 82.3\%, 99.2\%, and 99.1\%, respectively. 
% (REMOVE Heart Rate Monitoring from our scope)
% In \cite{DBN3}, the effectiveness of DBN is validated with the TROIKA dataset \cite{TROIKA} via a two-stage technique: 1) clustering individuals into different groups using partition around medoids (PAM); 2) performing biometric identification (gender, weight, current movement, etc.) using DBN with unsupervised training. The validation accuracy with TROIKA is as high as 96.1\%. 
In addition, Alsheikh \emph{et al.} \cite{DBN4} tested the activity recognition performance of DBNs using different parameter settings. Instead of using the raw acceleration data similar to \cite{DBN1}, they used spectrogram signals of the triaxial accelerometer data to train the deep activity recognition models. They found that deep models with more layers outperform the shallow models, and the topology of layers having more neurons than the input layer is shown to be more advantageous. The accuracy of the tuned DBN was 98.23\%, 91.5\%, and 89.38\% on the WISDM \cite{WISDM}, Daphnet \cite{Daphnet}, and Skoda \cite{Skoda} benchmark datasets, respectively. In \cite{DBN7}, RBM is used to better perform sensor fusion, as neural networks can identify non-intuitive features largely from cross-sensor correlations and thus offer a more accurate estimation. The recognition accuracy with the Skoda dataset reaches 81\%, which is higher than the traditional classification methods.
%

In addition to taking advantage of public datasets, there are also researchers employing DBNs on human activity or health-related recognition with self-collected datasets \cite{DBN2a, DBN5}. In \cite{DBN2a}, DBNs are employed in Parkinson's disease diagnosis to explore if they can cope with the unreliable labelling that results from naturalistic recording environments. The data were collected with two tri-axial accelerometers, with one worn on each wrist of the participant. Deep belief networks employed are 2 layer RBMs, with the first layer as Guassian-binary and the second layer as binary-binary. In \cite{DBN5}, a unsupervised 5-layer DBM-DNN is applied for the automatic detection of eating episodes via commercial bluetooth headsets collecting raw audio signals, which demonstrates classification improvement even with the presence of ambient noise. The accuracy of the proposed DBM-DNN approach is 94\%, which is significantly better than SVM with a 75.6\% accuracy. 
% There are also research seeking to accurately determine the heart rate with DBN during intensive motion \cite{DBN6}, which is accomplished by classifying PPG signals obtained from smartphones or wearable devices combined with motion-related signals obtained from accelerometers.
%

\subsection{Convolutional Neural Network (CNN)}
%
\textcolor{red}{Haik: I think we should decide once again who the target audience is for this paper. Because readers unfamiliar with the material will not be able to follow your explanation: its a very complex topic to condense into three paragraphs. And those which do know, probably don't need it. So either a much more thorough explanation is needed for those with no background, or a simple sentence (with citations) will be enough, and your paper should be emphasizing the applications instead}

The mechanism of CNN resembles the biological processes of the animal visual cortex~\cite{cnn_origin}. The convolutional operation, with shared kernel, enables the learning process of space invariant features. Although each kernel of a layer covers a limited size of input neurons, by stacking multiple layers, the neurons of higher layers turn to be able to cover a quite large area of reception field. 
% 
Compared with fully-connected neural network, CNN can capture local dependency since each filter in one convolutional layer has a defined receptive field and with convolutional layers stacked together, the overall receptive field can be derived. 
%

CNN also incorporates pooling layer that follows each convolutional layer as a standard manner. By dropping part of the output of convolutional layer, pooling layer compresses the representation it is learning and strengthen the model with extra noise resistance capability. 

A large volume of papers have applied CNN to locomotion recognition and daily activity recognition~\cite{cnn2015mm, cnn2015smc, cnn2016expert, cnn2017bigcomp, cnn2018informatics}. A fixed-length of multi-channel sensor data is sent to CNN architecture including a stack of convolutional layers, pooling layers, fully connected layers, and softmax layer. Sometimes pooling layers are omitted. In~\cite{laput2, cnn2015mm, cnn2015smc, cnn2016expert, cnn2017bigcomp}, they have shown that the CNN approach outperform traditional machine learning approaches (SVM, decision trees, Random Forest, \emph{et al.}) on a large range of locomotion datasets such as \textcolor{red}{UCI, SHO, USC} and self-collected datasets. In~\cite{cnn2017embc}, the CNN approach is used in recognizing actions in the process of making a cup of tea.
~\cite{cnn_pamap2_2017iswc} has tested on both locomotion and semantic gesture in dataset PAMAP2~\cite{PAMAP2}.
%

In the work of~\cite{cnn2016bsn}, CNN is applied with spectrogram of inertial sensor data as input data. It was tested on mobile platforms with different window sizes of the data input and a group of hyperparameters of CNN. 
Authors of ~\cite{cnn2017jbhi} utilized CNN to learn features from the spectragram of inertial sensor data, then combined the learnt features with statistical features to achieve real-time activity classification on a wearable embedded system with higher accuracy than using traditional ML methods with statistical features, a DBN-based method~\cite{DBN4}, and the CNN-based method in~\cite{cnn2016bsn}. They tested on locomotion dataset as well as complex working place activity dataset, Skoda.

~\cite{cnn2018informatics} used a late fusion manner that construct separate CNN structure for each IMU sensor at first and then fuse the outputs together with a fully connected layer. 
\textcolor{red}{~\cite{mccnn2015ijcai}: multichannel
Even though the outputs are not merged explicitly, all of the filters are shared over all channels, and hence influence each other.} 
% multi-scale CNN~\cite{multiscale_cnn}: 
To resolve the variant length problem, multi-scale convolutional neural networks (MCNN) is proposed.

% The segmentation 
% segment using self-correlation then cnn~\cite{seg_cnn}: hand gesture detection using wrist-worn sensor

In another work~\cite{iss2image}, the author converted the 1D time series input data to 2D. They showed the convertibility between sequential data and static data form resembling the manner of image and the advantage of applying CNN on 2D input over 1D input in some applications.


\subsection{Recurrent Neural Network (RNN)}
% 
Unlike feed-forward neural networks, a recurrent neural network (RNN) processes the input data in a recurrent behavior, and its architecture is shown in Fig. \ref{fig_rnn}. Equivalent to a directed graph, RNN exhibits dynamic behaviors and possesses the capability of modeling temporal and sequential relationship. In HAR domain, the processed data are inherently time series data. However, CNN adopts fixed size window to segment the time series data, which sometimes causes the ignorance of long range temporal dependency. 
% 
In addition, the long short-term memory (LSTM) has shown an astonishing capability in memorizing and modeling the long-term dependency in data, and therefore taken a dominant role in time-series and textual data analysis. It has made substantial contributions to the field of speech recognition, handwriting recognition, natural language processing, video analysis, etc. 

\cite{alex_RNN} 

\begin{figure}
\centering
  \includegraphics[width=0.9\columnwidth]{img/fig_rnn.png}
  \caption{Unidirectional LSTM-based DRNN model consisting of an input layer, several hidden layers, and an output layer. The number of hidden layers is a hyperparameter that is tuned during training~\cite{DRNN_HAR}.}~\label{fig:fig_rnn}
\end{figure}
%

In 2013, Lefebvre \emph{et al.} have applied RNN to 3D gesture classification \cite{BLSTM-RNN}. 
% B-LSTM-S: 

Hammerla \emph{et al.} has tested both bi-directional LSTM with frame as input and bi-directional LSTM with sample as input~\cite{B-LSTM-S}. 
It has compared the discriminative classification capability between CNN and LSTM, and \textcolor{red}{indicated a high accuracy of CNNs for continuous periodic activities compared to RNN.}
What's worth mentioning, 

% CNN + LSTM \cite{deepconvlstm}: 
In 2016, an architecture combining CNN and LSTM was presented in \cite{deepconvlstm}, which significantly outperformed traditional algorithms and peer deep learning algorithms and still acts as state-of-the-art work until today in many scenarios. The framework is composed of 4 convolutional layers, 2 recurrent LSTM layers and 1 softmax layer, and thus called DeepConvLSTM. Based on the design of DeepConvLSTM, \cite{TMD2018} has proposed an architecture of CNN and Bidirectional-LSTM.

% Ensemble of LSTMs: 
\cite{ensembleLSTM} has shown an ensemble algorithm of LSTMs. It is originated from the observation that due to randomness during the stochastic gradient training processing, by taking each LSTM as a meta-classifier, if we run multiple LSTMs in parallel and then combine the collected results with majority vote, it will intrinsically deliver better performance than any of the single meta-classifier.
\cite{DRNN_HAR} proposed a cascaded unidirectional and bidirectional LSTM, which takes advantage of both the fast speech of cascade classifier and extraordinary classification capability of bidirectional LSTM.

% Deep Residual Bi-LSTM: 

% LSTM with attention, 

% CTC: 
% \cite{CTC} has applied CTC in sign language recognition. CTC is a method that aligns

% Semi-supervised


The method of LSTM is also applied in other specific human activity detection, such as eating detection. \cite{swallownet} depicted a smart necklace equipped with a piezoelectric sensor to detect vibration around throat area during chewing activity, and utilized LSTM networks to classify chewing and non-chewing activities based on raw sensor signals. The result demonstrated that the LSTM outperformed traditional machine learning algorithms such as Random Forest \cite{eating2017, eatingsemisupervised2018, eatingend2end2018, eatingmicromovement2019}. 
\cite{eatingmicromovement2019} used a predefined micromovement based LSTM to detect a whole process of feeding gesture and exhibited the best performance on the FIC dataset. Other than the application of eating detection, \cite{sleep2016, sleep2016arxiv} have applied LSTM and several variants to sleeping mode detection and sleep quality assessment. 


% Although RNN is more suitable to time series classification problem, it has a disadvantage of longer training time than CNN. 




%
\subsection{Generative Adversarial Network (GAN)}
%
Generative Adversarial Network (GAN) was proposed by Goodfellow \emph{et al.} \cite{ganorigin} in 2014 and rapidly became one of the most exciting breakthroughs in the field of machine learning. A GAN is composed of two components: generator ($F_G$) and discriminator ($F_D$). %, as illustrated in Fig. % need a figure for GAN 
 GAN artfully takes the concept of competition \textcolor{red}{(sentence fragment)}. The Generator ($F_G$) and Discriminator ($F_D$) are competing with each other, in the manner that $F_G$ is trying to confuse the discriminator and $F_D$ is trying to distinguish samples generated by $F_G$ and the samples from the original dataset. GAN is set up as a zero-sum game framework, where both $F_G$ and $F_D$ are competing to individually gain stronger and stronger capability of imitating original data samples and discrimination capability iteratively.
%
Despite its relatively short history, GAN has been rapidly applied to the field of HAR. \textcolor{red}{(If we can't find a substantial body of work it may be a good idea to omit this subsection (as generally providing an overview of GAN is probably out of scope for this work))}


% \subsection{Other models}
% \subsubsection{Deep Residual network}

\subsection{Deep Transfer Learning}\label{DTL}

The success of machine learning and deep learning based HAR relies on massive annotated data. [domain adaption applied no HAR]

Instead of domain adaption model, adversarial model is proposed to realize domain transfer issue. For example, ~\cite{liang2019additive} focuses on authentication that recognize the mobile device user when the setting changes, such as the hardware device is upgraded. What's worth mentioning, a new area called fairness-based machine learning (FML) is dedicated to solve the fairness issue related to gender, race, and color with transfer learning paradigm utilized. 
%



\subsection{Deep Reinforcement Learning}
%
Reinforcement learning is particularly useful employing unlabeled datasets to learn the  correct policy and develop correct strategy based on the reward. However, it is seldom used in classification tasks, especially the supervised ones. Since reinforcement learning doesn't make use of the specific knowledge of class labels, it typically takes a very large amount of time to converge. However, if the HAR dataset collected is properly labeled, it would be much faster and easier to use regular supervised learning. \textcolor{red}{(I think its pretty well written but I couldn't find many concrete examples of how this relates to HAR. So one possibility is to omit it from your paper, or find various works that specifically employ DRL to HAR)}
%

However, reinforcement learning can be employed in many elements of HAR beyond classification. For example, both \cite{RL1} and \cite{RL2} apply deep reinforcement learning schemes to improve the adaptability of the trained classifiers across different application domains. Specifically, a selective attention mechanism is applied to the reinforcement learning scheme to focus on the crucial dimensions of the data, which is able to capture extra information from the signal and significantly improve the discriminative power of the classifier \cite{RL1}. In addition, since a classifier or device can rarely be trained on all end-users' data aforehand, online HAR is necessary in real applications. In \cite{RL2}, an artificial neural network is trained and used to classify human activities at an initial stage, and then an online reinforcement learning framework based on policy gradients is used to recognize the activities of new users that are previously unseen by the model. The result shows that the initial accuracy for new users is only about 60--70\%.  which can be improved to around 92\% by using reinforcement learning to continuously adapt the HAR system to each new user.
%

While many deep learning techniques have been applied on HAR problems, as introduced in the earlier sections, researchers and engineers have to make numerous design choices for the selected network, such as the number of layers of each type, the ordering of layers, and the hyper-parameters for each type of layer. 
% Although not directly related to HAR, some works have proposed the use of reinforcement learning to search for optimal deep learning network typologies within the space of network architectures. Remarkable contributions include the MetaQNN from Baker \emph{et al.} \cite{RL4} employing RL to search for optimal CNN typologies, as well as a similar work by Zoph and Le \cite{RL3} from the Google Brain team to optimize an RNN with reinforcement learning.
%
%
% \subsection{Other networks}
% %
% STFNets: Learning Sensing Signals from the Time-Frequency Perspective with Short-Time Fourier Neural Networks~\cite{STFNets}

% Siamese Neural Network based Similarity Metric for Inertial Gesture Classification and Rejection~\cite{Siamese}






\subsection{Physical Activity Recognition}



DBN: early explorations

Auto-encoder: another trial, introduced effects for other objectives like donoising. 

CNN: achieved significant improvements, boosted the adoptation of DL from other fields like image recognition to HAR. 


RNN(LSTM) combined with CNN: better performance, further enhanced the performance. 

GAN: 


Other 



\subsection{Deep Semi-supervised Learning}

Due to the excessive time and effort required to label sufficient data to train a deep neural network accurately in HAR, various semi-supervised learning algorithms have been applied to deploy the huge amount of unlabelled data that are readily available from many wearable sensors. 

Specifically, \cite{semisupervised_DL} has proposed using temporal ensembling of deep LSTM to recognize human activities with smartphone inertial sensors. Besides extracting for local dependencies in the recurrent framework, the proposed ensemble approach is applied to both the labeled and unlabeled data. Unsupervised losses are combined with supervised losses to make good use of unlabeled data that the supervised learning method cannot leverage. The effectiveness of the proposed semi-supervised learning scheme is validated by comparing its performance on dataset~\cite{UCI-HAD} against other semi-supervised learning approaches, such as Co-training-SVM, Co-training-KNN, and temporal emsembling CNN, etc. 

To tackle the same problem, \cite{VAE} has proposed a joint framework of variational auto-encoders (VAE) and convolutional neural networks (CNN). In particular, the VAE intends to extract the salient characteristics of human activity data and to provide the useful criteria for the compressed sensing reconstruction, while the CNN aims for extracting the discriminative features and for producing the low-dimension latent codes. The input data is given as a combination of labeled and unlabelled time-series data, and the proposed architecture utilizes compressed samples from the latent vector in a deconvolutional decoder to reconstruct the input time-series. The preliminary study has shown that with a small amount of labeled data, the proposed semi-supervised learning framework outperforms the conventional supervised learning. 
In addition, the authors in \cite{eatingsemisupervised2018} adapts a pretrained IMU-based food intake cycle detection model, which is trained using standard supervised learning techniques. The model is then fine-tuned with an enhanced decision boundary using unlabeled samples via a semi-supervised learning scheme. Increased recall scores accompanied by a small tradeoff in precision is reported by comparing the proposed semi-supervised adaptation method over the baseline method, upon a publicly available eating-behavior dataset. 
To further resemble the nature of many unlabelled real-world data, \cite{Semiunsupervised0} has proposed a ``semi-unsupervised learning" scheme based on Gaussian mixture deep generative model, which is more related to transfer learning and zero-shot learning where, in the training data, some classes are sparsely labelled and others entirely unlabelled. Besides demonstrating a superior semi-unsupervised classification performance on the MNIST dataset, the model is also applied to perform human activity classification and structure discovery using a highly unbalanced CAPTURE-24 dataset, in which the rarest class (running) is 80 times less prevalent than the commonest (sleep).




==> 6-challenges.tex <==
\section{Challenges and Opportunities} \label{sec:challenges}
% %
% HOW TO CONSTRUCT THIS CHAPTER SURROUNDING DEEP LEARNING

Though HAR has seen rapid growth, there are still a number of challenges that, if addressed, could further improve the status quo, leading to increased adoption of novel HAR techniques in existing and future wearables. In this section, we discuss these challenges and opportunities in HAR. 
Note that the issues discussed here are applicable to general HAR, not only DL-based HAR. We look to discuss and analyze the following \change{four questions under our research question $\mathsf{Q3}$ (challenges and opportunities)}, which overlap with the \change{four major constituents} of machine learning.
%from general HAR domain, not only DL-based HAR, and we give an overview of the current methods and progress with an emphasis on DL-based solutions. 
%In accordance with the three composites in machine learning applications: data, label, and model, we formulate this section in the following three questions.

\begin{itemize}
    \item $\mathsf{Q3.1:}$ What are the challenges in data acquisition? How do we resolve them? 
    \item $\mathsf{Q3.2:}$ What are the challenges in label acquisition? What are the current methods for them? 
    \item $\mathsf{Q3.3:}$ What are the challenges in modeling? What are potential solutions?
    \item $\mathsf{Q3.4:}$ \change{What are the challenges in model deployment? What are potential opportunities?}
\end{itemize}


\subsection{Challenges in Data Acquisition and Sample Size}

Data is the cornerstone of artificial intelligence. Models only perform as well as the quality of the data used during training. If the expectation is to ensure that the data is generalizable, then careful attention should be made in data collection to ensure the participants are representative of the population of interest. Moreover, showing sufficient sample size is an important problem. In HAR there currently is no well-defined method for determining sample size of training data, however, showing convergence of the error rate as a function of the number of samples in the training data is one approach shown by 
Yang \etal~\cite{voice_in_ear}.  Acquiring a massive amount of high-quality data at a low cost is a critical problem in every domain. There have been extensive efforts to collect and create publicly available datasets in some domains, such as computer vision and natural language processing. As such, researchers in these domains have access to ample amounts of data. However, in HAR, collecting raw data is labor-intensive considering a large number of different sensors and types of wearables that could be used. Therefore, proposing and developing innovative approaches to augmenting data with synthetic data all while ensuring high-quality data collection is imperative for the growth of HAR research. 
% \textbf{Opportunity:} 
To address this challenge, research in methods to simplify or improve HAR sensors and their robust performance in real-world scenarios are needed to enable modeling of humans in the real-world. 
% \textcolor{red}{(Stephen, DO WE HAVE MORE THOUGHTS ABOUT THE POTENTIAL SOLUTION???).} \textcolor{green}{Stephen - Why don't we remove this? There are a bunch of subsubsections later that present opportunities.}


\subsubsection{The Need for More Data}
\label{subsubsec:the_need_for_more_data}

Raw data collection requires a considerable amount of time and effort for projects in HAR. Particularly when researchers propose their original hardware, it is inevitable to collect data on users. 
Data augmentation is commonly used to generate synthetic data during training when there is a shortage of collected data. Data augmentation applies synthetic noise, typically observed in real situations, to real data to obtain new training samples. In general, using the dataset augmented with synthetic training samples yield higher classification accuracy when compared to using the same dataset without augmentation. Giorgi \etal augmented their dataset by varying each signal sample with translation drawn from a small uniform distribution and showed improvements in accuracy using this augmented dataset \cite{shoes}. Many DL-based methods also augment their datasets to improve performance \cite{parkinson_augmentation, lstm_augmentation, T-CGAN, resnet_augmentation}.
\textbf{Opportunity:} To address this challenge, research is needed in quantifying the benefits of different data augmentation methods to assess their benefits and limitations as a function of different data sets. \changezs{Another avenue of research is to utilize transfer learning, borrowing well-trained models from domains with high performing classifiers (i.e. images), and adapting them using a few samples of sensor data.}

%\textcolor{red}{(Stephen, DO WE HAVE MORE THOUGHTS ABOUT THE POTENTIAL SOLUTION???)}



\subsubsection{Data Quality and Missing Data}

The quality of models is highly dependent on the quality of the data used for training. Many real-world collection scenarios introduce different sources of noise that may significantly degrade data quality, such as electromagnetic interference or uncertainty in task scheduling for devices that perform sampling~\cite{mDebugger}.

In addition to developing robust noise-resistant systems for data collection, multiple algorithms have been proposed to clean or impute poor-quality data. Data imputation is one of the most common methods to replace poor quality data or fill in missing data when sampling rates fluctuate greatly. For example, Cao \etal introduced a bi-directional recurrent neural network to impute time series data on the UCI localization dataset \cite{NIPS_BRITS}. Luo \etal utilized a GAN to infer missing time series data \cite{NIPS2018_GAN}. Saeed \etal proposed an adversarial autoencoder (AAE) framework to perform data imputation \cite{imputation}. \textbf{Opportunity:} To address this challenge, more research into automated methods for evaluating and quantifying the quality is needed in order to better identify, remove, and/or correct for poor quality data. \changezs{Additionally, it has been experimentally shown that deep neural networks have the ability to learn well even if trained with noisy data, given that the networks are large enough and the dataset is large enough~\cite{rolnick2017DL}. This motivates the need for HAR researchers to focus on other areas of importance, such as how to efficiently deploy larger models in real systems (Section~\ref{subsec:challenges_in_model_deployment}) and generating more data (Section~\ref{subsubsec:the_need_for_more_data}), which could potentially aid in solving this problem.}

%\textcolor{red}{(Stephen, DO WE HAVE MORE THOUGHTS ABOUT THE POTENTIAL SOLUTION???)}


\subsubsection{\changezs{Privacy Protection}}

% FULL MATERIALS: sight (vision), hearing (audition), taste (gustation), smell (olfaction) and touch (somatosensation), as well as temperature (thermoception), kinesthetic sense (proprioception), (equilibrioception), vibration (mechanoreception), etc.
%
With the growing number and inference potential of novel sensors, privacy is increasingly becoming a concern among users~\cite{chen2021deep}. In general, the more inference potential a sensor has, the less willing a person is to agree to its collection of data, not at-least without some measure of control.
% 
% For example, human obtain over 70\% information from vision, meanwhile, video camera is also the most unaccepted sensor from a list of existing pervasive sensors.
%
To address this issue, multiple works have introduced methods for preserving user privacy while classifying human activities, including the replacement auto-encoder, the guardian, estimator, and neutralizer (GEN) architecture \cite{AE6}, and the anonymizing autoencoder \cite{AE7}. For example, replacement auto-encoders learn to replace features of time-series data that correspond to sensitive inferences with values that correspond to non-sensitive inferences. Ultimately, these works obfuscate features that can identify the individual, while preserving features common to each activity or movement. 
% 
\changezs{
Federated learning is a trending approach to resolve privacy issue in learning problems~\cite{mothukuri2021survey, briggs2021review, sozinov2018human, Meta-HAR}. It can enable the collaborative learning of a global model without the need to expose users' raw data. 
% 
~\citet{XIAO2021107338} realized a federated averaging method combined with a perceptive extraction network to improve the performance of the federated learning system.
% 
~\citet{tu2021feddl} designed a dynamic
layer sharing scheme which assisted the merging of local models to speed up the model convergence and achieved dynamic aggregation of models. 
% 
~\citet{bettini2021personalized} presented a personalized semi-supervised federated learning method that built a global activity model and leveraged transfer learning for user personalization.
% 
Besides, \citet{gudur2021resource} implemented on-device federated learning using model distillation update and so-called weighted $\alpha$-updates strategies to resolve model heterogeneities on a resource-limited embedded system (Raspberry Pi), which proved its effectiveness and efficiency. 
}
% 
\changezs{
\textbf{Opportunity:} 
% 
Recently, blockchain is a new hot topic around the world. Blockchain is a peer-to-peer network where peers can communicate without the need for centralized authority. It has been explored to facilitate the privacy-preserving data collection and sharing ~\cite{8001731, bdiwi2018blockchain, 10.3389/fbloc.2020.497985}.
% 
\citet{CHEN2021102011} reviewed mobile crowdsourcing solutions with blockchain technology to resolve the data quality, privacy, and security issues. 
The combination of federated learning and blockchain is also a potential solution towards privacy protection~\cite{nguyen2021federated} and currently still in its very early stage. More collaboration between ubiquitous computing community and networking community should be encouraged so as to prosper in-depth and practical research in novel directions.
}


%===================================================================
\subsection{Challenges in Label Acquisition}

Labeled data is crucial for deep supervised learning. Image and audio data is generally easy to label by visually confirming or hearing the images or audio streams, respectively. However, labeling and distinguishing different types of human activities simply by looking at different time series from HAR sensors is difficult as unique patterns in raw data can be difficult to identify, especially as the number of potential confounding activities increases. Therefore, ground truth acquisition for HAR sensors generally requires an extra wearable or sensing source to provide video or audio data combined with synchronization methods to align timestamps from the ground truth video/audio with the HAR sensor data. This makes ground truth acquisition for HAR much more labor-intensive. Moreover, accurate time synchronization between wearable devices and video cameras is challenging and an emerging research problem in ubiquitous computing because different devices are equipped with independent (and often drifting) clocks. A number of attempts have been made to address this issue, such as \cite{SynchronizationLex} and the Window Induced Shift Estimation method (SyncWISE) \cite{SyncWISE}. 
% \textbf{Opportunity:} 
\changezs{Two areas that require more research into by the DL-HAR community are shortages in labeled and difficulties in obtaining data from real-world scenarios.} 
% \textcolor{red}{(Stephen,can you expand this part??).} \textcolor{green}{Stephen - Why don't we remove this? There are a bunch of subsubsections later that present opportunities.}


\subsubsection{Shortage of Labeled Data}


As annotating large quantities of data is expensive, there have been great efforts to develop various methods to reduce the need for annotation, including data augmentation, semi-supervised learning, weakly supervised learning, and active learning to overcome this challenge.

% \begin{enumerate}
% \item Semi-supervised Learning
% \textit{(a) } 

Semi-supervised learning utilizes both labeled data and unlabeled data. By leveraging the abundance of unlabeled data, it is able to learn a more generalizable feature representation. % optimal and generalizable feature representation.
\citet{semi1} presented two semi-supervised CNN methods that utilizes unlabeled data during training: the convolutional encoder-decoder and the convolutional ladder network. They showed that the convolutional ladder network had a better classification performance, achieving 18\% F1-score improvement compared to the supervised CNN approach on ActiTracker dataset.
% 
Dmitrijs demonstrated on the SHL dataset, with a CNN and AAE architecture, that semi-supervised learning on unlabeled data could achieve high accuracy \cite{semi_aae}. \changezs{Chen \etal proposed an encoder-decoder based method that reduces distribution discrepancies between labeled and unlabeled data, that arise due to differences in biology and behavior from different people, while preserving the inherent similarities of different people performing the same task~\cite{chen2019people}.}
% 
\changezs{Bettini \etal combined active learning and federated learning to proactively annotate the unlabeled sensor data and build personalized models in order to cope with data scarcity problem~\cite{bettini2021personalized}.
% 
}

% \cite{semisupervised_DL}
% \cite{Semiunsupervised0}
% \cite{eatingsemisupervised2018}

% \textcolor{purple}{Self-supervised learning is another kind of semi-supervised learning. Saeed \etal designed ~\cite{self-supervised}.}


% \item Active Learning
% \textit{(b) Active Learning} 
\changezs{As a specialized version of semi-supervised learning, active learning builds model using a relatively small-sized labeled dataset while implicitly takes advantage of the data distribution of unlabeled data corpus. }
Active learning is an advanced ground-truthing technique that, based on an objective function, selectively chooses unlabeled data for a human-in-the-loop annotator to label. In active learning, the model predicts the label and generates a confidence measurement. Samples with low prediction confidence are sent to human annotators to provide labels. In recent years, researchers have tried to combine DL approaches with an active learning framework, in order to gain the benefit of establishing labels on-the-fly while leveraging the extraordinary classification capability of DL. Gudur \etal utilized active learning by combining a CNN with Bayesian techniques to represent model uncertainties (B-CNN)~\cite{DAL1}. \textbf{Opportunity:} Though active learning has demonstrated that fewer labels are needed to build an effective model, it is unknown if this method of working with an oracle to select the best data samples to segment truly saves annotator time and cost. A time-cost analysis is needed with varying datasets to truly determine the benefits of active learning. Moreover, given the many existing labeled datasets, another area of opportunity is developing methods that leverage characteristics of labeled datasets to generate labels for unlabeled datasets (i.e., transfer learning).

% \textcolor{purple}{A non-DL active learning work. Deep Active Learning \cite{DeActive}.}

% Multi-modal active learning and active learning for personalized models are possible promising directions. 

% \subsubsection{Label Quality}
% \textit{Weakly Supervised Learning}
% % Weakly Supervised Human Activity Recognition from Wearable Sensors by Recurrent Attention Learning
% ~\cite{Weakly_Attention} He \etal 

% explored the weakly supervised dataset~\cite{Weakly_Supervised}. 

% Attention model is utilized to learn from weakly labeled data and locate the activity part. 

% Inspired by ~\cite{2018learn}, which applied a attention-based CNN model on image recognition, \cite{Attention_CNN_weaklylabel} only needs a big chunk of time series data to be labeled as if there is a specific human activity in it and does not require the location of the activity in the time series. 

% Combined with CNN extracted representative features, .....
% \end{enumerate}



\subsubsection{Issues of In-the-field Dataset}

Traditionally, HAR research has been conducted primarily in-lab. Recently, HAR research has been moving towards in-field experimentation. Unlike in-lab settings, where the ground truth of activities can be collected with surveillance cameras and annotated by human annotators, in-field experiments may have people moving around in daily life. A static camera deployment would not be sufficient to capture all the places a person may go. Alharbi \etal used ground truth wearable cameras placed at the wrist, chest, and shoulders to record subject movements and surroundings as subjects moved around outside of a lab setting~\cite{barriers}. \textbf{Opportunity:} More research in leveraging human-in-the-loop to provide in-field labeling is required to generate more robust datasets for in situ activities. Additionally, there are opportunities for semi-supervised learning methods that leverage the sparse labels provided by humans-in-the-loop to generate high quality labels for the rest of the dataset.



% % 
% In~\cite{sensecam}, 
% In~\cite{Laput2}, the authors adopt using ...

% \subsubsection{Sensor Synchronization}
% The temporally-precise annotation of sensor data is necessary in order to build models that can passively sense and infer behavior from sensor signals. For behaviors involving limb movements, such as smoking, eating, and brushing, video-recordings from wearable cameras are increasingly being used to obtain temporally-precise ground truth labels.



%===================================================================

% \subsubsection{Transfer learning}
% As we discussed in \ref{DTL}, transfer learning 
% UnTran: Recognizing Unseen Activities with Unlabeled Data Using Transfer Learning~\cite{UnTran}
% Deep Convolutional Feature Transfer Across Mobile Activity Recognition Domains, Sensor Modalities and Locations~\cite{TL_CNN}
% Transfer Learning for sEMG Hand Gestures Recognition Using Convolutional Neural Networks~\cite{TL_CNN2}


%===================================================================
%===================================================================
\subsection{Challenges in Modeling}

\changezs{
In this section, we discuss the challenges and opportunities in the modeling process in several aspects, including data segmentation, semantically complex activity recognition, model generalizability, as well as model robustness. 
}

\subsubsection{Data Segmentation}

As discussed in~\cite{review_Plotz}, many methods segment time series using traditional static sliding window methods. A static time window may either be too large, capturing more than is necessary to detect certain activities, or too small and not capturing enough of the series to detect long movements and activities. Recently, researchers have been looking to segment time series data more optimally. Zhang \etal used reinforcement learning to find more optimal activity segments to boost HAR performance~\cite{RL1}. 
\change{\citet{qian2021weakly} proposed weakly-superviseds sensor-based activity segmentation and recognition method.}
\textbf{Opportunity:} More experimentation and research into dynamic activity segments or methods that leverage both short term and long term features (i.e., wavelets) are needed to create robust models at all timescales. \changezs{Although neural networks such as RNNs and LSTMs can model time series data with flexible time scales, their inherent issues such as exploding/vanishing gradients and training difficulty, make widespread adoption difficult. As such, more research into other methods that account for these issues are necessary.}
% \textcolor{red}{Shibo:FINAL THINKING TO ADD SOMETHING...}

%===================================================================
\subsubsection{Semantically Complex Activity Recognition}

Current HAR methods achieve high performance for simple activities such as running. However, complex activities such as eating, that could be composed of many different movements, is still challenging. To tackle this challenge, \citet{eatingmicromovement2019} break down complex gestures into a series of simpler (atomic) gestures that, when combined, form the complex gesture. \citet{hierarchical2016} proposes a hierarchical architecture that constructs high-level human activities from low-level activities. \citet{aroma} proposes AROMA, a complex human activity recognition method that leverages deep multi-task learning to learn simple activities that make up more complex activities. \textbf{Opportunity:} Though hierarchical methods have been introduced for various complex tasks, there are still opportunities for improvements. Additionally novel black-box approaches to complex task recognition, where individual steps in complex actions are automatically learned rather than specifically identified or labeled by designers, have yet to be fully explored; such a paradigm has the potential to achieve higher accuracy than methods where humans identify the higher-level attributes to learn and classify, much like the relationship between deep learning (where features are automatically learned) and classical machine learning (where features are engineered).

% zero-shot learning: Attributes’ Importance for Zero-Shot Pose-Classification Based on Wearable Sensors~\cite{zsl}
% Multi-Label Zero-Shot Human Action Recognition via Joint Latent Embedding~\cite{multilabel_zsl}


%===================================================================
\subsubsection{Model Generalizability}
% Generalization in a large population
% Intraclass variance 
% Interclass similarity
% Transfer Learning: \cite{liang2019additive}

A model has high generalizability when the model performs well on data that it has never seen before. Overfitting occurs when it performs well on training data, but poorly on new data. K-fold cross validation or leave-one-participant-out cross validation is generally used to improve the generalizability of the model.
In wearable based HAR, many factors will affect the generalizability of the model; we group them into two categories: \textit{User Variability} and \textit{Sensing Heterogeneity}. During recent years, many efforts have been put into improving the generalizability of models in HAR~\cite{Heterogeneities1,Heterogeneities2, Heterogeneities3}. 
% 
Most research on generalizability in HAR has been focused on creating models that can generalize to a larger population. Creating highly generalizable models generally requires a large amount of data and high model complexity. We would like to point out that another direction is to adaptively adjust model parameters to new users as they use the system. Rather than having a model that has many parameters and is intensive to train, we have a smaller model that adaptively adjusts to the current user using this model.
% 
Siirtola and Röning propose an online incremental learning approach that continuously adapts the model with the user's individual data as it comes in \cite{incremental}. \change{\citet{qian2021latent} introduce Generalizable Independent Latent Excitation (GILE), which greatly enhances the cross-person generalization capability of the model.}
\changezs{\textbf{Opportunity:} Another avenue of generalizability that has yet to be fully explored for DL-based HAR are new training methods that can adapt and learn predictors across multiple environments, such as invariant risk minimization~\cite{arjovsky2020invariant} or federated learning methods~\cite{konevcny2015federated}. Incorporating these areas into DL-based HAR could not only improve the generalizability of HAR models, but accomplish this in a model-agnostic way.}

%\textbf{Opportunity:} However, combining incremental learning with DL in wearable HAR systems remains an open problem. \textcolor{red}{(STEPHEN, Can we expand this?)}



%===================================================================
%===================================================================
\subsubsection{Model Robustness}
% \subsubsection{Model Reliability}
% \textcolor{red}{(One further improvement: add more related papers)}

\changezs{
A key issue that the community is paying increasing attention to is model robustness and reliability. That is, how to adapt the model in a dynamic environment without significant performance degradation~\cite{multisensor_review, ahad2021sensor}. 
% 
To tackle the model robustness issue, one feasible trending method is \textit{multi-sensory} that increases the number of sensors and improves the model reliability by introducing sensing redundancy. 
% 
Out of the consideration of device portability and user comfort level, a single sensor is commonly desired to achieve decent recognition performance. 
% 
However, compared with single sensor based activity recognition, multi-sensor systems generally have higher reliability and robustness.
% 
Nowadays, multi-sensor based HAR and sensor fusion has become a trend to improve the robustness and generalization of recognition systems~\cite{abedin2021attend,Physical_Activity2021,sd_multisensory,ijcai2018-859,RL1,sena2021human}.
% 
\citet{Physical_Activity2021} has proposed an architecture called DeepFusionHAR to incorporate the handcrafted features and deep learning extracted features from multiple sensors to detect daily life activities and sports activities and outperformed traditional deep learning baselines.
% 
\citet{sd_multisensory} has proposed a multi-sensory approach for basic and complex human activity recognition. To be specific, they utilized built-in sensors of smartphones and smartwatches to classify 25 physical
activities (including 5 basic activities and 20 complex ones). 
% 
\citet{ijcai2018-859} demonstrated a mobile application that ran on a multi-sensor mobile platform for daily living activity classification using a combination of accelerometer, gyroscope, magnetometer, microphone and GPS.
% 
Multi-sensory networks in some cases are integrated with attention modules as they can automatically learn the most representative and discriminative sensor modality. For example, \citet{RL1} utilized attention-based reinforcement learning to classify human activities.
% Vid2Sensor
}
% 
\changezs{\textbf{Opportunity:} Although there are works that utilize multiple sensors to improve robustness, these works require users to be wearing or have access to all of the sensors they utilize. An exciting new direction is to create generalized frameworks that can adaptively utilize data from whatever sensors happens to be availble, such as this smarthome intelligence system~\cite{xiadia2021}. Creating such systems would not only greatly improve the practicality of HAR-based systems, but would also contribute significantly to general artificial intelligence.}


% \textit{Multi-sensor Algorithms}

% \textit{Multi-modal Algorithms}

% Multi-modality Sensor Data Classification with Selective Attention


% \textit{From Video to Sensor}

% IMUTube

%===================================================================

\subsection{Challenges in Model Deployment}

\label{subsec:challenges_in_model_deployment}

\changezs{
There are two stages in developing deep learning applications: model training and model inference.
Deep learning model training normally take place on powerful workstations with GPUs, while model inference can be conducted on much less powerful edge devices or on cloud servers with user data uploaded to cloud.
% 
There are three layers in an edge device-based deep learning system: hardware, library, and algorithm. At the bottom is the hardware layer.
% 
The major computational units in hardware infrastructure include CPU, GPU, and DSP co-processors~\cite{survey_on_device_ml}. % , and other hardware accelerators
% 
Many of modern mobile devices integrate these units in a single chip called System-On-Chips (SOCs)~\cite{aamodt2018general}.
% 
Nowadays there are three main CPU architectures for mobile devices (e.g., smartphones and smartwatches): ARM, ARM64, and x86. 
% 
GPU is designed to enable and accelerate the graph processing. When designing SOC GPU architectures, great efforts are paid to improve energy efficiency and area efficiency. 
% 
DSP co-processor is designed with signal processing operation optimization to accelerate the processing speed. 
% 
% hardware accelerator: 
% 
% Libraries
On top of the hardware layer is the library layer. Some popular neural network libraries widely used in deep learning communities include TensorFlow Lite, ONNX Runtime, CMSIS NN, etc. Each of them is compatible with certain types of CPU or GPU architecture. In most cases, developers need to select a suitable machine learning library according to the platform, API language, CPU architecture, and GPU configuration. These libraries provide users with APIs to directly manipulate the hardware to perform computing.  
% 
On top of the library layer, researchers and developers build the algorithms. When the deep learning models are deployed in real world scenarios, mobile platforms are most commonly used out of the consideration of Internet availability and latency, energy consumption of data transfer, as well as privacy concern.}

\change{There are several works that focus on deploying deep learning based HAR on mobile platforms.~\citet{deepx} proposes a SOC-based architecture for optimizing deep neural network inference, while~\citet{DeepEar} utilizes the smartphone's digital signal processor (DSP) to reduce power consumption and improve inference time on smartphones.~\citet{MobiRNN} proposes a smartphone-based architecture that offloads DNN computations onto the mobile GPU to improve inference time.~\citet{DeepSense} proposes a light-weight CNN and RNN-based system that accounts for noisy sensor readings from smartphones and automatically learns more local and global features between sensor windows to improve classification and regression performance on smartphones.}

\change{A second class of works focus on reducing the complexity of neural networks, so that they can run on resource-limited mobile platforms.~\citet{Sparsification} reduces the amount of computation required at each layer by encoding layers into a lower-dimensional space, thereby improve inference speed while maintaining accuracy.~\citet{Binarized-BLSTM-RNN} reduces computation by utilizing binary weights rather than fixed-point or floating weights.}

\change{Emerging trends in deploying neural networks include offloading computation onto application-specific integrated circuits or lower power consumption microcontrollers.~\citet{bhat2019asic, wang2008asic} developed custom integrated circuits and hardware accelerators that perform the entire HAR pipeline, from sampling to DNN inference with significantly lower power consumption than mobile or GPU-based platforms. The downside to these application-specific systems is that they cannot be reconfigured for other types of tasks.~\citet{islam2020zygarde} presents an architecture for embedded systems or other batteryless methods that dynamically schedules DNN inference tasks (i.e. when to compute each layer) to improve inference time, accuracy, and task completion rate in such systems.}

\change{\textbf{Opportunity:} Though there are works that explore the deployment of DNNs practical systems, more research is needed for society to fully benefit from the advances in DNNs for HAR. Many of the works discussed leverage a single platform (i.e. either smartphone or ASIC), but there are still many opportunities for improving the practical use of HAR by exploring intelligent ways to partition computation across the cloud, mobile platforms, and other edge devices. DNN-based HAR systems can largely benefit by incorporating methodologies proposed by works such as~\cite{xia2021csafe, xia2019improving, godoy2018paws, nie2020spiders, nie2021spidersplus, nie2020facial, chandrasekaran2016seus, xia2018smartphone}, that carefully partition computation and data across multiple devices and the cloud.}

\change{
Lane \etal performed a small-scale exploration into the performance of DNNs for HAR applications on a mobile platforms in various configurations, including utilizing the phone's CPU and DSP and offloading computation onto remote devices~\cite{lane2015mobile}.} 
\change{This work demonstrates that mobile devices running DNN inference can scale gracefully across different compute resources available to the mobile platform, and also supports the need for more research into optimal strategies for partitioning DNN inference across mobile and edge systems to improve latency, reduce power consumption, and increase the complexity of the DNNs serviceable to wearable platforms.
}





% %===================================================================
% \subsubsection{Exploration of New Machine Learning Method}

% With the rapid progression of Machine Learning, researchers invest efforts to apply new models for improving performance and extending application scenarios. 
% \textcolor{red}{I added RL papers here}



% %===================================================================
% \subsection{Topics in HAR}
% \subsubsection{Sensor Fusion}
% Sensor fusion is a popular and significant topic in human activity recognition. Existing fusion paradigms are categorized into 3 classes including early fusion, middle fusion, and late fusion. 
% % 
% Early fusion is often data-level fusion, which combines multiple data resources from heterogeneous sensors and homogeneous sensors.
% % 
% Late fusion decision level.
% % 
% Middle fusion includes feature levels and ...



%===================================================================
% \subsubsection{On-device Deployment}








%===================================================================

% ===================================================================
% \subsection{Interpretability of DL Algorithms}




==> 7-future.tex <==
% \section{Future Direction} \label{sec:future}

% What's the next step after sensing and recognizing?

% Healthcare:

% Intervention: smart, personalized, self-evolving, lifelong learning intelligent agent.




==> 8-conclusion.tex <==
\section{Conclusion} \label{sec:conclusions}

% CNN stems from CV. RNN/LSTM stems from NLP. Can we expect an algorithm that originates from sensors so that fully suits the characteristics of sensory data?

% a fairly huge amount of labeled data is desired by deep learning algorithm to achieve better performance

Human activity recognition in wearables has provided us with many conveniences and avenues to monitor and improve our life quality. AI and ML have played a vital role in enabling HAR in wearables. 
In recent years, DL has pushed the boundary of wearables-based HAR, bringing activity recognition performance to an all-time high. 
% 
\change{In this paper, we provided our answers to the three research questions we proposed in Section II. We firstly gave an overall picture of the real-life applications, mainstream sensors, and popular public datasets of HAR. Then we gave a review of the advances of the deep learning approaches used in the field of wearable HAR and provided guideline and insight about how to choose an appropriate DL approach after comparing the advantages and disadvantages of them. At last, we discussed the current road blockers in three aspects: data-wise, label-wise, and model-wise, for each of which we provide potential opportunities.
We further identify the open challenges and finally provide suggestions for future avenues of research in this field. 
% 
By categorizing and summarizing existing works that apply DL approaches to wearable sensors based HAR, we aim to provide new engineers and researchers entering this field an overall picture of the existing research work and remaining challenges. We would also like to benefit experienced researchers by analyzing and discussing about the developing trends, major barriers, cutting-edge frontiers, and potential future directions.
% By \changezs{\st{systematically}} categorizing and summarizing existing works that apply DL approaches to wearable sensors based HAR, we aim to provide new engineers and researchers entering this field an overall picture of the existing research work and remaining challenges. We would also like to benefit experienced researchers by analyzing and discussing about the developing trends, major barriers, cutting-edge frontiers, and potential future directions.
}

==> wyfsmsdjwmmpwddskgkrzmpfhdscywyz/camera_ready.tex <==
\section{Introduction} 
\label{sec:intro}


Since the first Linux-based smartwatch was presented in 2000 at the IEEE International Solid-State Circuits Conference (ISSCC) by Steve Mann, who was later hailed as the ``father of wearable computing”, the 21st century has witnessed a rapid growth of wearables. For example, as of January 2020, 21\% of adults in the United States, most of whom are not opposed to sharing data with medical researchers, own a smartwatch~\cite{techcrunch2020}. 
 
 
In addition to being fashion accessories, wearables provide unprecedented opportunities for monitoring human physiological signals and facilitating natural and seamless interaction between humans and machines. Wearables integrate low-power sensors that allow them to sense movement and other physiological signals such as heart rate, temperature, blood pressure, and electrodermal activity. The rapid proliferation of wearable technologies and advancements in sensing analytics have spurred the growth of human activity recognition (HAR). 
%Human activity recognition (HAR) has become more robust and practical than ever before due to the proliferation of wearable technologies (enabling a plethora of data to be collected to train models) and rapid advancements in 
% artificial intelligence.
%sensing analytic methods.
As a general understanding of the HAR shown in \mbox{Figure \ref{figg1}}, HAR has drastically improved the quality of service in a broad range of applications spanning healthcare, entertainment, gaming, industry, and lifestyle, among others. 
% \textcolor{red}{For example, step counts during inpatient recovery after cancer surgery was shown to be an accurate predictor of 30- and 60-day hospital readmission~\cite{Low2017}}. 
Market analysts from Meticulous Research\textregistered~\cite{wearable_forecast} forecast that the global wearable devices market will grow at a compound annual growth rate of 11.3\% from 2019, reaching \$62.82 billion by 2025, with companies like Fitbit\textregistered, Garmin\textregistered, and Huawei Technologies\textregistered ~investing more capital into the area.


In the past decade, deep learning (DL) has revolutionized traditional machine learning (ML) and brought about improved performance in many fields, including image recognition, object detection, speech recognition, and natural language processing.
DL has improved the performance and robustness of HAR, speeding its adoption and application to a wide range of wearable sensor-based applications.
% 
%\zs{The reason behind the overwhelming performance of DL is two-folded -- its automatic feature extraction capability and the capability of modeling complex distribution. Traditional machine learning algorithms usually call for manual feature engineering which unavoidably requires expert domain knowledge and large amount of human efforts. When using a deep neural network, the representative features can be learnt automatically from raw data in a hierarchical manner, thus eliminating the challenging stage of feature engineering. Besides, deep neural networks contain a large number of parameters, which allows learning from large-scale datasets in order to model more complex distributions than traditional ML approaches and shallow neural networks. Due to the extraordinary expressive power and capability of utilizing large datasets, we have witnessed an exponential increase in DL-based HAR applications.}
There are two key reasons why DL is effective for many applications. First, DL methods are able to directly learn robust features from raw data for specific applications, whereas features generally need to be manually extracted or engineered in traditional ML approaches, which usually requires expert domain knowledge and a large amount of human effort. Deep neural networks can efficiently learn representative features from raw signals with little domain knowledge. Second, deep neural networks have been shown to be universal function approximators, capable of approximating almost any function given a large enough network and sufficient observations~\cite{cybenko1989approximation, scafer2006approximator, zhou2020universality}. Due to this expressive power, DL has seen \minorrevision{a substantial} growth in HAR-based applications.
% \minorrevision{as presented in other papers such as~\cite{wang2019deep, nweke2018deep}}.


% Deep models introduce layered architectures for data representation~\cite{deng2014tutorial}. 

Despite promising results in DL, there are still many challenges and problems to overcome, leaving room for more research opportunities. We present a review on deep learning in HAR with wearable sensors and elaborate on ongoing challenges, obstacles, and future directions in this field.



\begin{figure}[h!]
\centering %% If there is a figure in wide page, please release command \centering
\begin{tabular}{ccc}
\includegraphics[width=0.32\linewidth]{final_images/wearables_shares_on_purpose.png}
&\includegraphics[width=0.32\linewidth]{final_images/sensors2.png}
&\includegraphics[width=0.28\linewidth]{final_images/wearables_shares_on_body_part.png}\\
({\bf a})&({\bf b})&({\bf c})\\
\end{tabular}


    \caption{Wearable devices and their application. (\textbf{a}) Distribution of wearable applications %MDPI: Please check if the copyright permission is needed for this Figures 1,5-9. If so, please provide it.
 \cite{wearable_database}. (\textbf{b})~Typical wearable devices. (\textbf{c}) Distribution of wearable devices placed on common body areas~\cite{wearable_database}.}\label{figg1}
\end{figure}



% passive sensors are defined as sensors receiving and processing signals coming for the environment.
% \textcolor{red}{Technical challenge:}
%
% From the perspective of sensor adaptability for HAR, it is common that the widely accepted wearable sensors are not able to provide valid information for inferring human activities, since their captured data can have little informative modality. (Very confusing sentence "sensor adaptability" , "informative modality". Perhaps rephrase)

% The inherent reason of their being more accepted by users \textcolor{red}{(what is the inherent reason of these sensors being widely used, despite their deficiencies?)} decides their lower capability toward the goal to infer or predict human activity. 

% That’s also embodied by the fact that in HAR studies, the ground truth is often obtained by manually observing and labeling the video recording, which represents the vision modality. However, while cyber security experts may disagree, most humans can hardly distinguish the exact activity visually from the inertial sensor data. In this case, interpreting HAR from measurements of the inertial sensor is an inherently difficult problem, which can be only accomplished by specifically targeting certain symbolic icons of human behaviors. 

% If we compare it with image recognition field, we can find that, when compared with the complexity of tasks and astonishingly high performance that image/video recognition has achieved, the performance of high-level complex human activity recognition from wearable sensors other than camera is quite preliminary and far from ready to be deployed in real life. 
 




% \textbf{Topic: Multi-modality}

% According to ensemble theory, multiple informatively weak sensors can form a strong perception method. This lays the foundation of this study combining multiple modalities for human activity recognition. 


% \begin{figure}
% \centering
%   \includegraphics[width=0.38 \columnwidth]{img/modality_rank.jpg}
%   \caption{modality rank}~\label{fig:modality}
% \end{figure}


Specifically, we focus on the recognition of physical activities, including locomotion, activities of daily living (ADL), exercise, and factory work. While DL has shown a lot of promise in other applications, such as ambient scene analysis, emotion recognition, or subject identification, we focus on HAR. Throughout this work, we present brief and high-level summaries of major DL methods that have significantly impacted wearable HAR. For more details about specific algorithms or basic DL, we refer the reader to original papers, textbooks, and tutorials~\cite{Goodfellow-et-al-2016, Sutton2018}.
\change{
Our contributions are summarized as followings.}

\begin{enumerate}[label=(\roman*),labelsep=7pt]

\item \change{Firstly, we give an overview of the background of the human activity recognition research field, including the traditional and novel applications where the research community is focusing, the sensors that are utilized in these applications, as well as widely-used publicly available datasets.}
% 
\item \change{Then, after briefly introducing the popular mainstream deep learning algorithms, we give a review of the relevant papers over the years using deep learning in human activity recognition using wearables. We categorize the papers in our scope according to the algorithm (autoencoder, CNN, RNN, etc.). In addition, we compare different DL algorithms in terms of the accuracy of the public dataset, pros and cons, deployment, and high-level model selection criteria.} 
% 
\item \change{We provide a comprehensive \changeanother{systematic} review on the current issues, challenges, and opportunities in the HAR domain and the latest advancements towards solutions. At last, honorably and humbly, we make our best to shed light on the possible future directions with the hope to benefit students and young researchers in this field.
}
 
\end{enumerate}

% \yx{need update in the end} 


\section{Methodology} 
\label{sec:method}


\subsection{Research Question} 
\label{sec:question}

\changezs{In this work, we propose several major research questions, including $\mathsf{Q1:}$ What the real-world applications of HAR, mainstream sensors, and major public datasets are in this field, $\mathsf{Q2:}$ What deep learning approaches are employed in the field of HAR and what pros and cons each of them have, and $\mathsf{Q3:}$ What challenges we are facing in this field and what opportunities and potential solutions we may have. In this work, we review the state-of-the-art work in this field and present our answers to these questions.}


This article is organized as follows:
\changezs{
% We first propose the research question and define our research scope in Section~\ref{sec:method}. Then 
We compare this work with related existing review work in this field in Section~\ref{sec:related}.} Section~\ref{sec:applications} introduces common applications for HAR. Section~\ref{sec:sensor} summarizes the types of sensors commonly used in HAR. Section~\ref{sec:dataset} summarizes major datasets that are commonly used to build HAR applications. Section~\ref{sec:deeplearning} introduces the major works in DL that contribute to HAR. Section~\ref{sec:challenges} discusses major challenges, trends, and opportunities for future work. We provide concluding remarks in Section~\ref{sec:conclusions}.




\subsection{Research Scope} 
\label{sec:scope}



% \section{Scope of This Paper} \label{sec:scope}

%
% \begin{figure}
% \centering
%   \includegraphics[width=.6\columnwidth]{img/consort.pdf}
%   \caption{Consort diagram.}~\label{fig:signal}
% \end{figure}

% \change{While this work is not aiming for a systematic survey of existing research work, we would still like to introduce our research scoping method in this section to provide an overview of this review work.}
%Our inclusion criteria are:
\changeanother{In order to provide a comprehensive overview of the whole HAR field, we conducted a systematic review for human activity recognition. To ensure that our work satisfies the requirements of a high-quality systemic review, we conducted the 27-item PRISMA review process~\cite{prisma} and ensured that our work satisfied each requirement. }
We searched in Google Scholar with meta-keywords %MDPI: footnotes are not allowed in the journal, please consider this change.
 ({\changefinal{We began compiling papers for this review in November 2020. As we were preparing this review, we compiled a second round of papers in November 2021 to incorporate the latest works published in 2021}}). (A) ``Human activity recognition'', ``motion recognition'', ``locomotion recognition'', ``hand gesture recognition'', ``wearable'', (B) ``deep learning'', ``autoencoder'' (alternatively ``auto-encoder''), ``deep belief network'', ``convolutional neural network'' (alternatively ``convolution neural network''), ``recurrent neural network'', ``LSTM'', ``recurrent neural network'', ``generative adversarial network'' (alternatively ``GAN''), ``reinforcement learning'', ``attention'', ``deep semi-supervised learning'', and ``graph neural network''. We used an AND rule to get combinations of the above meta-keywords (A) and (B). For each combination, we obtained top 200 search results ranked by relevance. We didn't consider any patent or citation-only search result (no content available online).

% \item Since the result from the search engines does not contain latest published works due to relatively low exposure and citation, we focus on the latest publications in the ubiquitous computing area including IMWUT, CHI Proceedings, SenSys Proceedings, MDPI Sensors, MDPI Informatics, and IEEE Sensors in order to follow the latest trend. 
% \end{enumerate}

% \change{We include works from 1) and 2). In the challenge and opportunity section, to cover the exploratory works focusing on the challenges of the wearable-based HAR, we also consider the works approaching challenging topics including data quality, data label acquisition, model generalizability, etc, with machine learning or deep learning.}

% \textcolor{red}{(Writing needs to be improved) } 
% \textcolor{orange}{already changed the word, please check whether this is ok}
\change{There are several exclusion criteria to build the database of the paper we reviewed.
% \begin{enumerate}[label=(\roman*)]
% \item 
First of all, we omitted image or video-based HAR works, such as~\cite{kiran2021fusion}, since there is a huge body of work in the computer vision community and the method is significantly different from sensor-based HAR. 
% We don’t include image or video based HAR works, such as~\cite{kiran2021fusion}, since there is a rather huge body of work in the computer vision community and the method is significantly different from sensor-based HAR. 
% \item 
Secondly, we removed the papers using environmental sensors or systems assisted by environmental sensors such as WiFi- and RFID-based HAR. 
% We remove the papers using environmental sensors or using systems assisted by environmental sensors such as WiFi- and RFID- based HAR. 
% \item 
Thirdly, we removed the papers with minor algorithmic advancements based on prior works. We aim to present the technical progress and algorithmic achievements in HAR, so we avoid presenting works that do not stress the novelty of methods.
In the end, as the field of wearable-based HAR is becoming excessively popular and numerous papers are coming out, it is not a surprise to find that many papers share rather similar approaches, and it is almost impossible and less meaningful to cover all of them. 
\changeanother{Figure~\ref{fig:consort} shows the consort diagram that outlines step-by-step how we filtered out papers to arrive at the final 176 papers we included in this review. We obtained 8400 papers in the first step by searching keywords mentioned above on Google Scholar. Next, we removed papers that did not align with the topics in this review (i.e., works that do not utilize deep learning in wearable systems), leaving us with 870 papers. In this step, we removed 2194 papers that utilized vision, 2031 papers that did not use deep learning, and 2173 papers that did not perform human activity recognition. Then, we removed 52 review papers, 109 papers that did not propose novel systems or algorithms, and five papers that were not in English, leaving us with 704 papers. Finally, we selected the top 25\% most relevant papers to review, leaving us with 176 papers that we reviewed for this work. We used the relevancy score provided through Google Scholar to select the papers to include in this systemic review.}
%
%
%
%
Therefore, we select, categorize, and summarize representative works to present in this review paper. We adhere to the goal of our work throughout the whole paper, that is, to give an overall introduction to new researchers entering this field and present cutting-edge research challenges and opportunities.}



\begin{figure}[h!]\centering
  \includegraphics[width= 0.7\linewidth]{img/consort_diagram.pdf}
  \caption{\change{Consort diagram outlining how we selected the final papers we included in this work.}}
  \label{fig:consort}
\end{figure}








\changefinal{However, we admit that the review process conducted in this work has some limitations. 
% First of all, we classified the deep learning algorithms into six categories. However, many more traditional approaches can also achieve good performance. 
% 
Due to the overwhelming amount of papers in this field in recent years, it is almost impossible to include all the published papers in the field of deep learning-based wearable human activity recognition in a single review paper. The selection of the representative works to present in this paper is unavoidably subject to the risk of bias. Besides, we may miss the very first paper initiating or adopting a certain method. At last, due to the nature of human-related research and machine learning research, many possibilities could cause heterogeneity among study results, including the heterogeneity in devices, heterogeneity from the demography of participants, and even heterogeneity from the algorithm implementation details.
}

% 
% 
% \begin{figure}[tb]
% 
% 
%   \includegraphics[width= 0.65\linewidth]{img/consort.pdf}
%   \caption{\changefinal{Consort diagram.}}
%   \label{fig:taxonomy}
% \end{figure}



% We remove the papers with little algorithmic advancements based on prior works. Our aim is to present the technical progress and algorithmic achievements in HAR, so we try to avoid presenting works which do not stress on the novelty of methods.}

% \end{enumerate}



\subsection{Taxonomy of Human Activity Recognition} 
\label{sec:scope}

\change{
In order to obtain a straightforward understanding of the hierarchies under the tree of HAR, we illustrate the taxonomy of HAR as shown in Figure~\ref{fig:taxonomy}. We categorized existing HAR works into four dimensions: Sensor, application, DL approach, and challenge. There are basically two kinds of sensors: Physical sensors and physiological sensors. Physical sensors include Inertial Measurement Unit (IMU), piezoelectric sensor, GPS, wearable camera, etc. Some exemplary physiological sensors are electromyography (EMG) and photoplethysmography (PPG), just to name a few. 
In terms of the applications of HAR systems, we categorized them into healthcare, fitness\&
lifestyle, and Human Computer Interaction (HCI). Regarding the DL algorithm, we introduce six approaches, including autoencoder (AE), Deep Belief Network (DBN), Convolutional Neural Network, Recurrent Neural Network (including Long Short-Term Memory (LSTM) and Gated Recurrent Units (GRUs)), Generative Adversarial Network (GAN), and Deep Reinforcement Learning (DRL). In the end, we discuss the challenges our research community is facing and the state-of-the-art works are coping with, also shown in Figure~\ref{fig:taxonomy}.
}
% 

% \begin{figure*}[tb]
\begin{figure}[h!]

\centering %% If there is a figure in wide page, please release command \centering
  \includegraphics[width= 0.95\linewidth]{img/HAR_taxonomy.pdf}

  \caption{\change{Taxonomy of Deep Learning-based Human Activity Recognition with Wearables.}}
  \label{fig:taxonomy}
\end{figure}
% \end{figure*}



% \begin{figure*}
% \centering
%   \includegraphics[width=\columnwidth]{img/HAR_taxonomy.pdf}
%   \caption{Taxonomy of Human Activity Recognition.}~\label{fig:taxonomy}
% \end{figure*}



% \change{Our inclusion criteria are:
% % \begin{enumerate}[label=(\roman*)]
% % \item 
% We search in Google Scholar with meta-keywords A) “Human activity recognition”, ”motion recognition”, ”locomotion recognition”, ``hand gesture recognition'', “wearable” B) “Deep learning”, “autoencoder” (“auto-encoder”), "deep belief network", “convolutional neural network” (“convolution neural network”), “recurrent neural network”, "LSTM", “recurrent neural network”, "generative adversarial network" ("GAN"), "reinforcement learning", "attention", "deep semi-supervised learning", and "graph neural network". We use an AND rule to get combinations of the above meta-keywords A) and B). For each combination, we obtain top 200 search results ranked by relevance. We cancelled out the checkbox for "including patents" and "including citations" to exclude patents and citation-only results.}

% % \item Since the result from the search engines does not contain latest published works due to relatively low exposure and citation, we focus on the latest publications in the ubiquitous computing area including IMWUT, CHI Proceedings, SenSys Proceedings, MDPI Sensors, MDPI Informatics, and IEEE Sensors in order to follow the latest trend. 
% % \end{enumerate}

% \change{The review includes works from 1) and 2). In the challenge and opportunity section, to cover the exploratory works focusing on the challenges of the wearable-based HAR, we also consider the works approaching challenging topics including data quality, data label acquisition, model generalizability, etc, with machine learning or deep learning.}

% \change{Our exclusion criteria are:
% % \begin{enumerate}[label=(\roman*)]
% % \item 
% We don’t include image or video based HAR works, since there’s a rather huge body of work in the computer vision community and the method is significantly different from sensor-based HAR. 
% % \item 
% We remove the papers using environmental sensors or using systems assisted by environmental sensors such as WiFi- and RFID- based HAR. 
% % \item 
% We remove the papers with little algorithmic advancements based on prior works. Our aim is to present the technical progress and algorithmic achievements in HAR, so we try to avoid presenting works which do not stress on the novelty of methods.}

% \end{enumerate}

\section{Related Work} 
\label{sec:related}

\change{
There are some existing review papers in the literature for deep learning approaches for sensor-based human activity recognition~\cite{wang2019deep,nweke2018deep,chen2021deep,ramanujam2021human}.}
% 
\change{
Nweke \etal accentuated the advancements in deep learning models by proposing a taxonomy of generative, discriminative, and hybrid methods along with further explorations for the advantages and limitations up to year 2018~\cite{nweke2018deep}. 
% 
Similarly, Wang \etal conducted a thorough analysis on different sensor-based modalities, deep learning models, and their respective applications up to the year 2017~\cite{wang2019deep}. 
% 
However, in recent years, due to huge advancements in the availability and computational power of computing resources and cutting-edge deep learning techniques, the applied deep learning area has been revolutionized and reached all-time-high performance in the field of sensor-based human activity recognition. Therefore, we aim to present the most recent advances and most exciting achievements in the community in a timely manner to our readers.}


\change{In another work, Chen \etal provided the community a comprehensive review which has done an in-depth analysis of the challenges/opportunities for deep learning in sensor-based HAR and proposed a new taxonomy for the challenges ahead of the activity recognition systems~\cite{chen2021deep}. 
% 
In contrast, we view our work as more of a gentle introduction of this field to students and novices in the way that our literature review provides the community with a detailed analysis on most recent state-of-the-art deep learning architectures (i.e., CNN, RNN, GAN, Deep Reinforcement Learning, and hybrid models) and their respective pros and cons on HAR benchmark datasets. At the same time, we distill our knowledge and experience from our past works in this field and present the challenges and opportunities from a different viewpoint.
% 
Another recent work was presented by Ramanujam \etal, in which they categorized the deep learning architectures in CNN, LSTM, and hybrid methods and conducted an in-depth analysis on the benchmark datasets~\cite{ramanujam2021human}. 
% 
Compared with their work, our paper pays more attention to the most recent cutting-edge deep learning methods applied on HAR on-body sensory data, such as GAN and DRL. We also provide both new learners and experienced researchers with a profound resource in terms of model comparison, model selection and model deployment.
% 
% as a resource assisting with model selection/deployment with most recent privacy-aware measures, e.g., blockchain. 
% 
% 
% However, due to the ubiquity of advanced low power sensors in wearable devices in recent years, this review paper failed to bring up the challenge of unlabeled data annotation, which is the bottleneck to DL systems in this field due to the reason that DL approaches are reliant on large amounts of sensory data to perform acceptably in HAR platforms.
In a nutshell, our review has thoroughly analysed most up-to-date deep learning architectures applied on various wearable sensors, elaborated on their respective applications, and compared performances on public datasets. What's more, we attempt to cover the most recent advances in resolving the challenges and difficulties and shed light on possible research opportunities. 
}

% \textcolor{red}{(Farzad, also this paper: Deep learning for sensor-based activity recognition: A survey, and this: A Survey of Human Activity Recognition in Smart Homes Based on IoT Sensors Algorithms: Taxonomies, Challenges, and Opportunities with Deep Learning, and Deep Learning for Sensor-based Human Activity Recognition: Overview, Challenges, and Opportunities)
% } done

% \textcolor{red}{is this covered? Human Activity Recognition With Smartphone and Wearable Sensors Using Deep Learning Techniques: A Review https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9389739}
% done
% \vspace{10pt}

\section{Human Activity Recognition Overview}

\subsection{Applications} \label{sec:applications}
% \yx{edited. Need proofread}
% In this section, we introduce and summarize the major areas and applications that HAR has impacted. We first give a brief introduction, and then illustrate each of the areas with concrete applications and examples that HAR has improved or enabled.
%Since deep learning techniques are quickly unlocking more application scenarios that were previously attempted by traditional machine learning methods, we'll not only include the existing work using deep learning in this section, but also discuss those pivotal applications using the traditional machine learning and data mining techniques in general. (A bit wordy and unnecessary. consider removing)
%

In this section, we illustrate the major areas and applications of wearable devices in HAR. Figure~\ref{figg1}a, taken from the wearable technology database~\cite{wearable_database}, breaks down the distribution of application types of 582 commercial wearables registered since 2015~\cite{wearable_database}. The database suggests that wearables are increasing in popularity and will impact people's lives in several ways, particularly in applications ranging from fitness and lifestyle to medical and human-computer interaction.






\subsubsection{Wearables in Fitness and Lifestyle}
% \subsubsection{Wearables in Fitness and Wellness}
% \subsection{Daily Life Logging}



% \textbf{Physical Activity Recognition:}
% Physical activities include, but are not limited to, sitting, walking, laying down, going upstairs or downstairs, jogging, running~\cite{Physical_activity_recognition}. The duration and intensity of an individual's physical activities throughout the day can reveal and, in turn, reshape daily habits and health conditions~\cite{physical_activity_health}. For example, regular physical activities can decrease the risk of many chronic diseases like obesity, diabetes, cardiovascular, and improve mental health~\cite{mobility_chronicdisease}. 
% Moreover, individuals' modes of transportation, such as walking, bicycling, or driving, are also of great interest to physicians, healthcare providers, and users themselves. Being aware of daily locomotion and transportation patterns can provide physicians with the necessary information to better understand patients' conditions, while also encouraging users to engage in more exercise and lead to self-regulatory behavioral change~\cite{Fitness_Behavior_Change}. Due to the above reasons, physical activity recognition is among the most prolific HAR applications~\cite{cnnhar2014, cnn2015smc, cnn2015mm, cnn2016expert, cnn2017bigcomp, benchmarkingSHL, SHLIndRNN, TMD2018, Attention_CNN_weaklylabel}.

% Based on physical activity recognition, energy expenditure can be estimated, which represents the amount of energy people burn to support metabolism and daily activities~\cite{Zhu2015Using}. Energy expenditure estimation can be estimated and presented to users in smartphones and smartwatches, or dedicated products such as Fitbit~\cite{fitbit}.



% \yx{edited. Need proofread}
Physical activity involves activities such as sitting, walking, laying down, going up or downstairs, jogging, and running~\cite{Physical_activity_recognition}. 
Regular physical activity is increasingly being linked to a reduction in risk for many chronic diseases, such as obesity, diabetes, and cardiovascular disease, and has been shown to improve mental health~\cite{mobility_chronicdisease}. 
The data recorded by wearable devices during these activities include plenty of information, such as duration and intensity of activity, which further reveals an individual's daily habits and health conditions~\cite{physical_activity_health}. 
For example, dedicated products such as Fitbit~\cite{fitbit} can estimate and record energy expenditure on smart devices, which can further serve as an important step in tracking personal activity and preventing chronic diseases~\cite{Zhu2015Using}. Moreover, there has been evidence of the association between modes of transport (motor vehicle, walking, cycling, and public transport) and obesity-related outcomes~\cite{transport_medical}.
Being aware of daily locomotion and transportation patterns can provide physicians with the necessary information to better understand patients' conditions and also encourage users to engage in more exercise to promote behavior change~\cite{Fitness_Behavior_Change}. Therefore, the use of wearables in fitness and lifestyle has the potential to significantly advance one of the most prolific aspects of HAR \mbox{applications~\cite{cnnhar2014, cnn2015smc, cnn2015mm, cnn2016expert, cnn2017bigcomp, benchmarkingSHL, SHLIndRNN, TMD2018, Attention_CNN_weaklylabel}.}

Energy (or calorie) expenditure (EE) estimation has grown to be an important reason why people care to track their personal activity. Self-reflection and self-regulation of one's own behavior and the habit has been important factor in designing interventions that prevent chronic diseases such as obesity, diabetes, and cardiovascular diseases. %Accurate and real-time EE estimation using wearable sensors is a challenge primarily due to....

\subsubsection{Wearables in Healthcare and Rehabilitation}

HAR has greatly impacted the ability to diagnose and capture pertinent information in healthcare and rehabilitation domains. 
By tracking, storing, and sharing patient data with medical institutions, wearables have become instrumental for physicians in patient health assessment and monitoring. 
% 
Specifically, several works have introduced systems and methods for monitoring and assessing  Parkinson disease (PD) symptoms~\cite{parkinson2015, parkinson2016, parkinson2017, parkinson2018, parkinson2018_2, parkinson_augmentation}. 
% 
\change{Pulmonary disease, such as Chronic Obstructive Pulmonary Disease (COPD), asthma, and COVID-19, is one of leading causes of morbidity and mortality. Some recent works use wearables to detect cough activity, a major symptom of pulmonary diseases~\cite{Listen2Cough, mcc,CoughBuddy2021Nemati,zhang2021coughtrigger}}.
% 
Other works have introduced methods for monitoring stroke in infants using wearable accelerometers~\cite{infant_stroke} and methods for assessing depressive symptoms utilizing wrist-worn sensors~\cite{depression}.
% 
In addition,  detecting muscular activities and hand motions using electromyography (EMG) sensors has been widely applied to enable improved prostheses control for people with missing or damaged limbs~\cite{EMG_review, EMG_armband, EMG_prosthese, EMG_prosthese2}.

% \textcolor{red}{Restless legs syndrome (RLS)}

% The cardinal motor symptoms of PD are bradykinesia, rigidity, tremor, and postural instability.

% tremor~\cite{pakinson2018_2}


\subsubsection{Wearables in Human Computer Interaction (HCI)}

% \yx{edited. Need proofread}
Modern wearable technology in HCI has provided us with flexible and convenient methods to control and communicate with electronics, computers, and robots. 
For example, a wrist-worn wearable outfitted with an inertial measurement unit (IMU) can easily detect the wrist shaking~\cite{seg_cnn, dynamichandgesturerecognition, fingerping} to control smart devices to skip a song by shaking the hand, instead of bringing up the screen, locating, and pushing a button. 
%
Furthermore, wearable devices have played an essential role in many HCI applications in entertainment systems and immersive technology.
One example field is augmented reality (AR) and virtual reality (VR), which has changed the way we interact and view the world. Thanks to accurate activity, gesture, and motion detection from wearables, these applications could induce feelings of cold or hot weather by providing an immersive experience by varying the virtual environment and could enable more realistic interaction between the human and virtual objects~\cite{EMG_review, EMG_armband}. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% re organized by yaxuan.  Here is the old version
% Augmented reality (AR) and virtual reality (VR) are two emerging fields that will change the way we interact and view the world around us. Many of the services provided by AR and VR are made possible only through HAR. For instance, a major method of interacting with AR and VR systems will be through arm or body gestures. Robust HAR to recognize these gestures will be crucial for effective and practical AR and VR systems. Several works and products have been introduced that can detect muscular activities and hand motions using electromyography (EMG) sensors embedded in an armband~\cite{EMG_review, EMG_armband}. Works such as these have impacts beyond just AR and VR, but can enable improved prostheses control for people with missing or damaged limbs~\cite{EMG_prosthese, EMG_prosthese2}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
% What's worth mentioning is that these application domains are not absolutely separate. There could be overlap between them. For example, energy expenditure estimation contains the locomotion recognition as the first step. % Human computer interaction and 
%

% \textcolor{red}{(I think it doesn't hurt to include this section, but it is somewhat out of scope for the topic of "Human Activity Recognition)}
% Identity authentication is the way to secure access to the physical or digital resources through personal biological characteristics. Aside from traditional biometrics such as fingerprint, iris, voice, and face, etc., motion sensor based solutions require no active interaction or interruption. The currently proposed solutions include breathing-based authentication, PPG-based~\cite{DBN3} authentication, gait-based authentication, and motion pattern-based authentication~\cite{motionid2016}. In summary, sensor-based authentication has been under continuous development since it embodies the advantage of allowing remote authentication~\cite{shoes}.
%

%The wearable industry has been surging since recent years. The widespread deployment of wearables is deeply influencing and transforming the healthcare industry, the medical industry, and the entertainment industry, as well as reshaping the human lifestyle. 
% ~\textcolor{red}{(Haik: That is all true! Another option is to cover the adherence and even privacy issues in wearable sensors. I'm sure there are many works along these lines)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Background} \label{sec:background}

% [A figure showing the number of deep learning CV papers v.s. deep learning wearable papers (intersection as deep learning ego-centric papers) v.s. DL NLP papers V.S. speech recognition] 
 
 
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Wearable Sensors}
\label{sec:sensor}
Wearable sensors are the foundation of HAR systems. As shown in Figure~\ref{figg1}b, there are a large number of off-the-shelf smart devices or prototypes under development today, including smartphones, smartwatches, smart glasses, smart rings~\cite{ring}, smart gloves~\cite{nature_gloves}, smart armbands~\cite{armband}, smart necklaces~\cite{necklace2015, necksense, NeckFace2021Chen}, smart shoes~\cite{shoes}, and E-tattoos~\cite{e-tattoo}. These wearable devices cover the human body from head to toe with a general distribution of devices shown in Figure~\ref{figg1}c, as reported by~\cite{wearable_database}.
% remove smart headsets, wearable cameras~\cite{sensecam},
The advance of micro-electro-mechanical system (MEMS) technology (microscopic devices, comprising a central unit such as a microprocessor and multiple components that interact with the surroundings such as microsensors) has allowed wearables to be miniaturized and lightweight to reduce the burden on adherence to the use of wearables and Internet of Things (IoT) technologies. In this section, we introduce and discuss some of the most prevalent MEMS sensors commonly used in wearables for HAR.
\change{The summary of wearable sensors is represented as a part of Figure \ref{fig:taxonomy}.}






%They usually consist of a central unit that processes data (an integrated circuit chip such as microprocessor) and several components that interact with the surroundings (such as microsensors)
%Their data collection reliability, sensor robustness, device usage feasibility, function configuration, as well as the comfort level of wearables jointly determine the effectiveness of the whole system. 

%Sensors built from Micro-Electro-Mechanical Systems (MEMS) are the pillars of support for the IoT era. Consider that Bosch, one of the world's leading MEMS sensor providers, has produced over 9.5 billion MEMS sensors since 1995~\cite{Bosch}. Among various MEMS sensors, no matter wearable or environmental, the Inertial Measurement Unit (IMU) is among the most fundamental and popular sensors on the stage of IoT. Especially in the area of wearable HAR, IMU is the leading widely-adopted sensor with the most popularity.

\subsubsection{Inertial Measurement Unit (IMU)}
% \yx{passed. Need proofread}
Inertial measurement unit (IMU) is an integrated sensor package comprising of accelerometer, gyroscope, and sometimes magnetometer. Specifically, an accelerometer detects linear motion and gravitational forces by measuring the acceleration in 3 axes (x, y, and z), while a gyroscope measures rotation rate (roll, yaw, and pitch). The magnetometer is used to detect and measure the earth's magnetic fields. Since a magnetometer is often used to obtain the posture and orientation in accordance with the geomagnetic field, which is typically outside the scope of HAR, the magnetometer is not always included in data analysis for HAR.  
% 
By contrast, accelerometers and gyroscopes are commonly used in many HAR applications. We refer to an IMU package comprising a 3-axis accelerometer and a 3-axis gyroscope as a 6-axis IMU. This component is often referred to as a 9-axis IMU if a 3-axis magnetometer is also integrated. Owing to mass manufacturing and the widespread use of smartphones and wearable devices in our daily lives, IMU data are becoming more ubiquitous and more readily available to collect. % through APIs of wearable devices such as smartphones, smartwatches, Google Glasses, etc. 
In many HAR applications, researchers carefully choose the sampling rate of the IMU sensors depending on the activity of interest, often choosing to sample between 10 and several hundred Hz. 
In~\cite{SampleRate}, Chung \etal  tested a range of sampling rates and gave the best one in his application. 
Besides, it's been shown that higher sampling rates allow the system to capture signals with higher precision and frequencies, leading to more accurate models at the cost of higher energy and resource consumption. 
For example, the projects presented in~\cite{ViBand, Laput2} utilize sampling rates above the typical rate. These works sample at 4 kHz to sense the vibrations generated from the interaction between a hand and a physical object. 
% There is generally no consensus on the best choice of sampling rates for different sensors. 


%which is referred to as bio-acoustic signals.
% 
% \textcolor{red}{In~\cite{cnn2015smc}, a single accelerometer is used to collect data from 3 different body parts: cloth pocket, trouser pocket and waist. Self-collected data on 100 subjects including 8 activities such as falling, running, jumping, walking, walking quickly, step walking, walking upstairs, and walking downstairs.}





\subsubsection{Electrocardiography (ECG) and Photoplethysmography (PPG)}

Electrocardiography (ECG) and photoplethysmography (PPG) are the most commonly used sensing modalities for heart rate monitoring. ECG, also called EKG, detects the heart's electrical activity through electrodes attached to the body. The standard 12-lead ECG attaches ten non-intrusive electrodes to form 12 leads on the limbs and chest. ECG is primarily employed to detect and diagnose cardiovascular disease and abnormal cardiac rhythms. PPG relies on using a low-intensity infrared (IR) light sensor to measure blood flow caused by the expansion and contraction of heart chambers and blood vessels. Changes in blood flow are detected by the PPG sensor as changes in the intensity of light; filters are then applied to the signal to obtain an estimate of heart rate. 
Since ECG directly measures the electrical signals that control heart activity, it typically provides more accurate measurements for heart rate and often serves as a baseline for evaluating PPG sensors.



% \begin{figure}[tb]
% \centering
%     
%   \includegraphics[width=\linewidth]{img/taxonomy_sensor.png}
%   \caption{\change{Taxonomy of wearable sensors}}
%   \label{fig:tax_sensor}
% \end{figure}


\subsubsection{Electromyography (EMG)}
Electromyography (EMG) measures the electrical activity produced by muscle movement and contractions. EMG was first introduced in clinical tests to assess and diagnose the functionality of muscles and motor neurons. There are two types of EMG sensors: Surface EMG (sEMG) and intramuscular EMG (iEMG). sEMG uses an array of electrodes placed on the skin to measure the electrical signals generated by muscles through the surface of the skin~\cite{wiki:emg}. 
There are a number of wearable applications that detect and assess daily activities using sEMG~\cite{EMG_armband, EMG_handmotion}. 
In~\cite{cnn12}, researchers developed a neural network that distinguishes ten different hand motions using sEMG to advance the effectiveness of prosthetic hands.
iEMG places electrodes directly into the muscle beneath the skin. Because of its invasive nature, non-invasive wearable HAR systems do not typically include iEMG.


\subsubsection{Mechanomyography (MMG)}
Mechanomyography (MMG) uses a microphone or accelerometer to measure low-frequency muscle contractions and vibrations, as opposed to EMG, which uses electrodes. For example, 4-channel MMG signals from the thigh can be used to detect knee motion patterns~\cite{cnn11}. Detecting these knee motions is helpful for the development of power-assisted wearables for powered lower limb prostheses. The authors create a convolutional neural network and support vector machine (CNN-SVM) architecture comprising a seven-layer CNN to learn dominant features for specific knee movements. The authors then replace the fully connected layers with an SVM classifier trained with the extracted feature vectors to improve knee motion pattern recognition.
Moreover, Meagher \etal~\cite{meagher2020new} proposed developing an MMG device as a wearable sensor to detect mechanical muscle activity for rehabilitation after stroke.


% 
% 2016 A convolutional neural network for robotic arm guidance using sEMG based frequency-features
% 2016 Multiday EMG-Based Classification of Hand Motions with Deep Learning Techniques
% 2017 Transfer Learning for sEMG Hand Gestures Recognition Using Convolutional Neural Networks: TL_CNN2
% 2018 Deep Learning for Electromyographic Hand Gesture Signal Classification Using Transfer Learning
% 2018 Worker Activity Recognition in Smart Manufacturing Using IMU and sEMG Signals with Convolutional Neural Networks:
% 2018 EMG Pattern Recognition in the Era of Big Data and Deep Learning: EMG_review
% 2019 An sEMG-Based Human–Robot Interface for Robotic Hands Using Machine Learning and Synergies: EMG_armband (non-deep learning)





 % \textcolor{red}{(Haik: I believe that EEG, EMG, ECG in particular are all very related concepts that could be separated from the discussion and discussed independently)} for recording the electrical stimulus produced by skeletal muscles, 
Other wearable sensors used in HAR include (but are not limited to) \change{piezoelectric sensor~\cite{khalifa2017harke, cha2018flexible} for converting changes in pressure, acceleration, temperature, strain, or force to electrical charge, barometric pressure sensor~\cite{masse2015improving} for atmospheric pressure, temperature measurement~\cite{barna2019study},} electroencephalography (EEG) for measuring brain activity~\cite{salehzadeh2020human}, respiration sensors for breathing monitoring~\cite{ramos2016using}, ultraviolet (UV) sensors~\cite{filippoupolitis2016activity} for sun exposure assessment, GPS for location sensing, \change{microphones for audio recording~\cite{jin2021sonicasl, ntalampiras2018transfer, CoughBuddy2021Nemati}}, and wearable cameras for image or video recording~\cite{NeckFace2021Chen}. 
% Specifically, images and videos are often recorded by wearable cameras, which are often referred to as egocentric cameras. 
% 
It is also important to note that the wearable camera market has drastically grown with cameras such as GoPro becoming mainstream~\cite{GoPro1, GoPro2, alharbi2018can, alharbi2019mask} over the last few years. However, due to privacy concerns posed by participants related to video recording, utilizing wearable cameras for longitudinal activity recognition is not as prevalent as other sensors. Additionally, HAR with image/video processing has been extensively studied in the computer vision community~\cite{voulodimos2018deep, xu2020computer}, and the methodologies commonly used differ significantly from techniques used for IMUs, EEG, PPG, etc. For these reasons, despite their significance in applications of deep learning methods, this work does not cover image and video sensing for HAR. 


% measure changes in pressure, acceleration, temperature, strain, or force by converting them to an electrical charge

% \begin{figure}[!h]
% \centering
%   \includegraphics[width=\columnwidth]{img/sensors.pdf}
%   \caption{Typical devices and application domains of wearables. \textcolor{red}{Where is this referenced in text?}}~\label{fig:signal}
% \end{figure}


% \begin{figure}[!h]
% \centering
%   \includegraphics[width=0.63\columnwidth]{final_images/wearables_shares_on_body_part.png}
%   \caption{Distribution of wearable devices placed on common body areas~\cite{wearable_database}.  \textcolor{red}{Where is this referenced in text?}}
%   \label{fig:wearables_shares_on_body_part}
% \end{figure}


% \subsection{Problem Definition}
% %
% %
% Conventionally, we convert the detection task to a classification problem by pre-defining classes of interest and the NULL class. With a sliding window manner and classification approach,
% %

% The way that it's transformed to a classification problem
% is similar to the object detection problem in computer vision area and keyword spotting problem in speech recognition area.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Major Datasets} \label{sec:dataset}
%
%

%
%

We list the major datasets employed to train and evaluate various ML and DL techniques in Table~\ref{tab:datasets}, ranked based on the number of citations they received per year according to Google Scholar. 
% All of the three-star datasets have been cited more than 200 times, indicating a particularly vibrant and concentrated research focus in the field of HAR. 
As described in the earlier sections, most datasets are collected via IMU, GPS, or ECG. While most datasets are used to recognize physical activity or daily activities~\cite{Opportunity, USC-HAD, UCI-HAR, DSA, TROIKA, SHO, WISDM, WHARF, HASC, SARD, Stisen, mHealth1, mHealth2, UTD-MHAD1/2, ExtraSensory, SHAR, Actitracker, PAMAP2, Ubicomp_08}, there are also a few datasets dedicated to hand gestures~\cite{ActRecTut, FIC}, breathing patterns~\cite{BreathPrint}, and car assembly line activities~\cite{Skoda}, as well as those that monitor gait for patients with PD~\cite{Daphnet}.
%

\begin{table}[h!]
\centering
\small
    \caption{Major Public Datasets for Wearable-based HAR.}
    \renewcommand\tabcolsep{5.9pt} 


\centering %% If there is a figure in wide page, please release command \centering
\begin{tabular}{lcccccc}
\toprule
\textbf{Dataset} & \textbf{Application} & \textbf{Sensor} &\textbf{ \# Classes} & \textbf{Spl. Rate} & \textbf{Citations/yr }\\
\midrule
WISDM~\cite{WISDM} & Locomotion & 3D Acc. & 6 & 20 Hz &  217 \\
ActRecTut~\cite{ActRecTut} & Hand gestures & 9D IMU & 12 & 32 Hz & 153 \\
UCR(UEA)-TSC~\cite{UCRArchive, UEA} & 9 datasets (e.g., uWave~\cite{uWave}) & Vary & Vary & Vary & 107 \\ %UCR(UEA)-TSC Archive 
UCI-HAR~\cite{UCI-HAR} & Locomotion & Smartphone 9D IMU  & 6 & 50 Hz & 78 \\
Ubicomp 08 ~\cite{Ubicomp_08} & Home activities &  Proximity sensors & 8 & N/A & 69 \\
% TROIKA~\cite{TROIKA} & Heart rate monitoring & PPG, ECG, 3D Acc. &  6 & 125 Hz & 55  \\
SHO~\cite{SHO} & Locomotion & Smartphone 9D IMU & 7 & 50 Hz & 52 \\
UTD-MHAD1/2~\cite{UTD-MHAD1/2} & Locomotion \& activities & 3D Acc. \& 3D Gyro. & 27 & 50 Hz & 39 \\
HHAR~\cite{Stisen} & Locomotion & 3D Acc. & 6 & 50--200 Hz & 37 \\
Daily \& Sports Activities~\cite{DSA} & Locomotion & 9D IMU & 19 & 25 Hz & 37  \\
MHEALTH~\cite{mHealth1, mHealth2} & Locomotion \& gesture & 9D IMU \& ECG & 12 & 50 Hz & 33 \\
Opportunity~\cite{Opportunity} & Locomotion \& gesture  & 9D IMU & 16 & 50 Hz & 32 \\
PAMAP2~\cite{PAMAP2} & Locomotion \& activities & 9D IMU \& HR monitor & 18 & 100 Hz & 32 \\
Daphnet~\cite{Daphnet} & Freezing of gait & 3D Acc. & 2 & 64 Hz & 30 \\
SHL~\cite{SHL} & Locomotion \& transportation & 9D IMU & 8 & 100 Hz & 23 \\
SARD~\cite{SARD} & Locomotion & 9D IMU \& GPS & 6 & 50 Hz & 22 \\
Skoda Checkpoint~\cite{Skoda} & Assembly-line activities & 3D Acc. & 11 & 98 Hz & 21 \\
UniMiB SHAR~\cite{SHAR} & Locomotion \& gesture & 9D IMU & 12 & N/A & 20 \\
USC-HAD~\cite{USC-HAD} & Locomotion & 3D ACC. \& 3D Gyro. &  12 & 100 Hz & 20 \\
ExtraSensory~\cite{ExtraSensory} & Locomotion \& activities & 9D IMU \& GPS & 10 & 25--40 Hz & 13 \\
HASC~\cite{HASC} & Locomotion & Smartphone 9D IMU & 6 & 100 Hz & 11 \\
% BreathPrint~\cite{BreathPrint} & Breathing activities & Smartphone audio & 3 & 8 kHz & 9 \\
Actitracker~\cite{Actitracker} & Locomotion & 9D IMU \& GPS & 5 & N/A & 6 \\
FIC~\cite{FIC} & Feeding gestures  & 3D Acc. & 6 & 20 Hz & 5 \\
WHARF~\cite{WHARF} & Locomotion & Smartphone 9D IMU & 16 & 50 Hz & 4 \\
\bottomrule
\end{tabular}


\label{tab:datasets}
\end{table}

% %
% %\end{paracol}
% \begin{figure}
% \centering
% 
%   \includegraphics[width=\linewidth]{img/HAR_location.pdf}
%   \caption{Placement of inertia sensors in different datasets: (a) WISDOM; (b) ActRecTut; (c) UCI-HAR; (d) SHO; (e) PAMAP2; and (f) Opportunity.}~\label{fig:location}
% \end{figure}
% %\begin{paracol}{2}
% %\linenumbers
% %\switchcolumn


Most of the datasets listed above are publicly available. The University of California Riverside-Time Series Classification (UCR-TSC) archive is a collection of datasets collected from various sensing modalities~\cite{UCR}. The UCR-TSC archive was first released and included 16 datasets, growing to 85 datasets by 2015 and 128 by October 2018. Recently, researchers from the University of East Anglia have collaborated with UCR to generate a new collection of datasets, which includes nine categories of HAR: {{BasicMotions}
}, {Cricket}, {Epilepsy}, {ERing}, {Handwriting}, {Libras}, {NATOPS}, {RacketSports}, and {UWaveGestureLibrary}~\cite{UEA}.
One of the most commonly used datasets is the OPPORTUNITY dataset~\cite{Opportunity}. This dataset contains data collected from 12 subjects using 15 wireless and wired networked sensor systems, with 72 sensors and ten modalities attached to the body or the environment. 
Existing HAR papers mainly focus on data from on-body sensors, including 7 IMUs and 12 additional 3D accelerometers for classifying 18 kinds of activities. Researchers have proposed various algorithms to extract features from sensor signals and to perform activity classification using machine-learned models like K Nearest Neighbor (KNN) and SVM~\cite{knn_har1, knn_har2, SVM_har1, cnn5, cnnhar2014, cnn17, cnn57, cnn61, cnn84, cnn115}.
% \textcolor{red}{[X, X, X, X, 5, 9, 17, 57, 61, 84, 115]}.
Another widely-used dataset is PAMAP2~\cite{PAMAP2}, which is collected from 9 subjects performing 18 different activities, ranging from jumping to house cleaning, with 3 IMUs (100-Hz sampling rate) and a heart rate monitor (9 Hz) attached to each subject. Other datasets such as Skoda~\cite{Skoda} and WISDM~\cite{WISDM} are also commonly used to train and evaluate HAR algorithms. In Figure~\ref{fig:location}, we present the placement of inertial sensors in 9 common datasets.

\vspace{-6pt}
% \end{paracol}
\begin{figure}[h!]
\centering %% If there is a figure in wide page, please release command \centering
  \includegraphics[width= \linewidth]{img/HAR_diagram.pdf}
  \caption{Placement %MDPI: 1. there is no a-f in the figure. 2. This figure is not mentioned in the main text, please mention the figure before where it is first presented in the text, and make sure the figures are mentioned in numerical order.
 of inertial sensors in different datasets: WISDOM; ActRecTut; UCI-HAR; SHO; PAMAP2; and Opportunity.}
  \label{fig:location}
\end{figure}
% \begin{paracol}{2}
% \linenumbers
% \switchcolumn

\section{Deep Learning Approaches}
\label{sec:deeplearning}

In recent years, DL approaches have outperformed traditional ML approaches in a wide range of HAR tasks. There are three key factors behind deep learning's success: Increasingly available data, hardware acceleration, and algorithmic advancements. The growth of datasets publicly shared through the web has allowed developers and researchers to quickly develop robust and complex models. The development of GPUs and FPGAs have drastically shortened the training time of complex and large models. Finally, improvements in optimization and training techniques have also improved training speed. In this section, we will describe and summarize HAR works from six types of deep learning approaches. 
\change{
We also present an overview of deep learning approaches in Figure \ref{fig:taxonomy}.}


% \begin{figure}[t]
% \centering
% 
%   \includegraphics[width=\linewidth]{img/taxonomy_ml_approaches.png}
%   \caption{\change{Taxonomy of deep learning approaches. }}
%   \label{fig:tax_ml}
% \end{figure}


%\textcolor{purple}{In recent years, DL approaches outperform traditional ML approaches in a wide range of HAR tasks. There are three key factors behind the arisal of deep learning: increasingly available data, hardware acceleration, and algorithmic advancements. Data-wise, the web-scaled data explosion provides the opportunity to train a large model with an exponential number of parameters. From hardware aspect, the prevalent usage of GPUs and FPGAs in training deep neural networks has dramatically shorten the training time from a formidable amount of time to a reasonable level. Besides, the development of deep neural models, the advancement of optimization techniques, and a bag of training tricks have collectively underpinned the boom of deep learning. In this section, we will describe 6 types of mainstream deep learning approaches that are applied in HAR tasks.}


\subsection{Autoencoder}




The autoencoder, originally called ``autoassociative learning module'', was first proposed in the 1980s as an unsupervised pre-training method for artificial neural networks (ANN)~\cite{AE0}.
Autoencoders have been widely adopted as an unsupervised method for learning features. As such, the outputs of autoencoders are often used as inputs to other networks and algorithms to improve performance~\cite{AE420, AE437, AE440, AE460, AE463}. An autoencoder is generally composed of an encoder module and a decoder module. The encoding module encodes the input signals into a latent space, while the decoder module transforms signals from the latent space back into the original domain. As shown in Figure \ref{fig:fig_ae}, the encoder and decoder module is usually several dense layers (i.e., fully connected layers) of the form 

$$
\begin{array}{l}
f_{\theta}(\mathbf{x}): \mathbf{z}=\sigma\left(W_{e} \mathbf{x} + b_{e}\right) \\
g_{\theta^{\prime}}(\mathbf{z}): \mathbf{x}^{\prime}=\sigma\left(W_{d} \mathbf{z} + b_{d}\right)
\end{array}
$$
where $\theta=\left\{W_{e}, b_{e}\right\}$, $\theta^{\prime}=\left\{W_{d}, b_{d}\right\}$ are the learnable parameters of the encoder and decoder. $\sigma$ is the non-linear activation function, such as Sigmoid, tanh, or rectified linear unit (ReLU). $W_{e}$ and $W_{d}$ refer to the weights of the layer, while $b_e$ and $b_d$ are the bias vectors. By minimizing a loss function applied on $\mathbf{x}$ and $\mathbf{x}^{\prime}$, autoencoders aim at generating the final output by imitating the input. Autoencoders are efficient tools for finding optimal codes, $\mathbf{z}$, and performing dimensionality reduction. An autoencoder's strength in dimensionality reduction has been applied to HAR in wearables~\cite{AE1, AE2, AE3, parkinson2018, AE437, AE6, AE7, AE8, AE423} and functions as a powerful tool for denoising and information retrieval.
\vspace{-9pt}
\begin{figure}[h!]
\centering
  \includegraphics[width=0.7\linewidth]{img/fig_ae}
  \caption{Illustration of an autoencoder network~\cite{autoencoder_graph}.}
  \label{fig:fig_ae}
\end{figure}


As such, autoencoders are most commonly used for feature extraction and dimensionality reduction~\cite{AE1, AE2, AE419, AE420, AE422, AE426, AE427, AE432, AE436, AE440, AE445, AE452, AE460, AE463, AE464}. Autoencoders are generally used individually or in a stacked architecture with multiple autoencoders.
{Mean squared error} or {mean squared error plus KL divergence} loss functions are typically used to train autoencoders. Li \etal presents an autoencoder architecture where a sparse autoencoder and a denoising autoencoder are used to explore useful feature representations from accelerometer and gyroscope sensor data, and then they perform classification using support vector machines~\cite{AE1}. Experiments are performed on a public HAR dataset~\cite{UCI-HAR} from the UCI repository, and the classification accuracy is compared with that of Fast Fourier Transform (FFT) in the frequency domain and Principal Component Analysis (PCA). The result reveals that the stacked autoencoder has the highest accuracy of 92.16\% and provides a 7\% advantage over traditional methods with hand-crafted features. Jun and Choi~\cite{AE481} studied the classification of newborn and infant activities into four classes: Sleeping, moving in agony, moving in normal condition, and movement by an external force. Using the data from an accelerometer attached to the body and a three-layer autoencoder combined with k-means clustering, they achieve 96\% weighted accuracy in an unsupervised way. 
Additionally, autoencoders have been explored for feature extraction in domain transfer learning~\cite{AE439}, detecting unseen data~\cite{AE434}, and recognizing null classes~\cite{AE435}. \change{For example, \citet{prabono2021atypical} propose a two-phase autoencoder-based approach of domain adaptation for human activity recognition. In addition, \citet{garcia2021ensemble} proposed an effective multi-class algorithm that consists of an ensemble of autoencoders where each autoencoder is associated with a separate class. This modular structure of classifiers makes models more flexible when adding new classes, which only calls for adding new autoencoders instead of re-training the model.}


Furthermore, autoencoders are commonly used to sanitize and denoise raw sensor data~\cite{AE3, AE8, AE467}, a known problem with wearable signals that impacts our ability to learn patterns in the data.
Mohammed and Tashev in~\cite{AE3} investigated the use of sensors integrated into common pieces of clothing for HAR.
However, they found that sensors attached to loose clothing are prone to contain large amounts of motion artifacts, leading to low mean signal-to-noise ratios (SNR). % as low as \zs{(commonly SNR in range of ...?)}. \yx{I didn't found "commonly range" in their paper. I think they conducted experiments and found that mean is -12 in their setup.} \zs{got it.}
To remove motion artifacts, the authors propose a deconvolutional sequence-to-sequence autoencoder (DSTSAE). The weights for this network are trained with a weighted form of a standard VAE loss function. Experiments show that the DSTSAE outperforms traditional Kalman Filters and improves the SNR from $-$12 dB to  +18.2 dB, with the F1-score of recognizing gestures improved by 14.4\% and locomotion activities by 55.3\%. 
Gao \etal explores the use of stacking autoencoders to denoise raw sensor data to improve HAR using the UCI dataset~\cite{UCI-HAR}~\cite{AE8}. Then, LightGBM (LBG) is used to classify activities using the denoised signals.

Autoencoders are also commonly used to detect abnormal muscle movements, such as Parkinson's Disease and Autism Spectrum Disorder (ASD).
% 
Rad \etal in~\cite{parkinson2018} utilizes an autoencoder to denoise and extract optimized features of different movements and use a one-class SVM to detect movement anomalies. To reduce the overfitting of the autoencoder, the authors inject artificial noise to simulate different types of perturbations into the training data. Sigcha \etal in~\cite{AE478} uses a denoising autoencoder to detect freezing of gait (FOG) in Parkinson's disease patients. The autoencoder is only trained using data labelled as a normal movement. During the testing phase, samples with significant statistical differences from training data are classified as abnormal FOG events.

As autoencoders map data into a nonlinear and low-dimensional latent space, they are well-suited for applications requiring privacy preservation. Malekzadeh \etal developed a novel replacement autoencoder that removes prominent features of sensitive activities, such as drinking, smoking, or using the restroom~\cite{AE437}. Specifically, the replacement autoencoder is trained to produce a non-sensitive output from a sensitive input via stochastic replacement while keeping characteristics of other less sensitive activities unchanged. Extensive experiments are performed on Opportunity~\cite{Opportunity}, Skoda~\cite{Skoda}, and \mbox{Hand-Gesture~\cite{ActRecTut}} datasets. The result shows that the proposed replacement autoencoder can retain the recognition accuracy of non-sensitive tasks using state-of-the-art techniques while simultaneously reducing detection capability for sensitive tasks. 

Mohammad \etal introduces a framework called Guardian-Estimator-Neutralizer (GEN) that attempts to recognize activities while preserving gender privacy~\cite{AE6}. 
The rationale behind GEN is to transform the data into a set of features containing only non-sensitive features. 
The Guardian, which is constructed by a deep denoising autoencoder, transforms the data into representation in an inference-specific space. 
% The Guardian part of the architecture is a deep denoising autoencoder that provides an inference-specific transformation. 
The Estimator comprises a multitask convolutional neural network that guides the Guardian by estimating sensitive and non-sensitive information in the transformed data. Due to privacy concerns, it attempts to recognize an activity without disclosing a participant's gender. 
The Neutralizer is an optimizer that helps the Guardian converge to a near-optimal transformation function. 
Both the publicly available MobiAct~\cite{MobiAct} and a new dataset, MotionSense, are used to evaluate the proposed framework's efficacy. 
Experimental results demonstrate that the proposed framework can maintain the usefulness of the transformed data for activity recognition while reducing the gender classification accuracy to 50\% (random guessing) from more than 90\% when using raw sensor data. 
Similarly, the same authors have proposed another anonymizing autoencoder in~\cite{AE7} for classifying different activities while reducing user identification accuracy. Unlike most works, where the output to the encoder is used as features for classification, this work utilizes both the encoder and decoder outputs. Experiments performed on a self-collected dataset from the accelerometer and gyroscope showcased excellent activity recognition performance (above 92\%) while keeping user identification accuracy below 7\%.





\subsection{Deep Belief Network (DBN)}
%
%
A DBN, as illustrated in Figure \ref{fig:fig_dbn}, is formed by stacking multiple simple unsupervised networks, where the hidden layer of the preceding network serves as the visible layer for the next. The representation of each sub-network is generally the restricted Boltzmann machine (RBM), an undirected generative energy-based model with a ``visible'' input layer, a hidden layer, and intra-layer connections in between. The DBN typically has connections between the layers but not between units within each layer. This structure leads to a fast and layer-wise unsupervised training procedure, where contrastive divergence (a training technique to approximate the relationship between a network's weights and its error) is applied to every pair of layers in the DBN architecture sequentially, starting from the ``lowest'' pair.
%
\vspace{-12pt}
\begin{figure}[h!]
\centering
  \includegraphics[width= 0.9\linewidth]{img/fig_dbn.png}
  \caption{The greedy layer-wise training of DBNs. The first level is trained on triaxial acceleration data. Then, more RBMs are repeatedly stacked to form a deep activity recognition model~\cite{DBN4}.
  }
  \label{fig:fig_dbn}
\end{figure}



The observation that DBNs can be trained greedily led to one of the first effective deep learning algorithms~\cite{DBN0}. There are many attractive implementations and uses of DBNs in real-life applications such as drug discovery~\cite{DBN8}, natural language understanding~\cite{DBN9}, fault diagnosis~\cite{DBN10}, etc. There are also many attempts to perform HAR with DBNs. In early exploratory work back in 2011~\cite{DBN1}, a five-layer DBN is trained with the input acceleration data collected from mobile phones.
% , and the HAR recognition time is less than 0.15 ms for an data frame time of 1 s
The accuracy improvement ranges from 1\% to 32\% when compared to traditional ML methods with manually extracted features. %compared with 8 traditional ML methods
%
 
In later works, DBN is applied to publicly available datasets~\cite{DBN2, DBN4, DBN7,mahmoodzadeh2021human}. In~\cite{DBN2}, two five-layer DBNs with different structures are applied to the Opportunity dataset~\cite{Opportunity}, USC-HAD dataset~\cite{USC-HAD}, and DSA dataset~\cite{DSA}, and the results demonstrate improved accuracy for HAR over traditional ML methods for all the three datasets. Specifically, the accuracy for the Opportunity, USC-HAD, and DSA datasets are 82.3\% (1.6\% improvement over traditional methods), 99.2\% (13.9\% improvement), and 99.1\% (15.9\% improvement), respectively. 
% (REMOVE Heart Rate Monitoring from our scope)
% In~\cite{DBN3}, the effectiveness of DBN is validated with the TROIKA dataset~\cite{TROIKA} via a two-stage technique: 1) clustering individuals into different groups using partition around medoids (PAM); 2) performing biometric identification (gender, weight, current movement, etc.) using DBN with unsupervised training. The validation accuracy with TROIKA is as high as 96.1\%. 
In addition, Alsheikh et al.~\cite{DBN4} tested the activity recognition performance of DBNs using different parameter settings. Instead of using the raw acceleration data similar to~\cite{DBN1}, they used spectrogram signals of the triaxial accelerometer data to train the deep activity recognition models. They found that deep models with more layers outperform the shallow models, and the topology of layers having more neurons than the input layer is shown to be more advantageous, which indicates overcompete representation is essential for learning deep models. The accuracy of the tuned DBN was 98.23\%, 91.5\%, and 89.38\% on the WISDM~\cite{WISDM}, Daphnet~\cite{Daphnet}, and Skoda~\cite{Skoda} benchmark datasets, respectively. In~\cite{DBN7}, a RBM is used to improve upon other methods of sensor fusion, as neural networks can identify non-intuitive predictive features largely from cross-sensor correlations and thus offer a more accurate estimation. The recognition accuracy with this architecture on the Skoda dataset reached 81\%, which is around 6\% higher than the traditional classification method with the best performance (Random Forest).
%

In addition to taking advantage of public datasets, there are also researchers employing DBNs on human activity or health-related recognition with self-collected datasets~\cite{parkinson2015, DBN5}. In~\cite{parkinson2015}, DBNs are employed in Parkinson's disease diagnosis to explore if they can cope with the unreliable labelling that results from naturalistic recording environments. The data was collected with two tri-axial accelerometers, with one worn on each wrist of the participant. The DBNs built are two-layer RBMs, with the first layer as a Guassian-binary RBM (containing gaussian visible units) and the second layer as binary-binary (containing only binary units) (please refer to~\cite{hinton2012practical} for details). In~\cite{DBN5}, an unsupervised five-layer DBM-DNN is applied for the automatic detection of eating episodes via commercial bluetooth headsets collecting raw audio signals, and demonstrate classification improvement even in the presence of ambient noise. The accuracy of the proposed DBM-DNN approach is 94\%, which is significantly better than SVM with a 75.6\% accuracy. 
% There are also research seeking to accurately determine the heart rate with DBN during intensive motion~\cite{DBN6}, which is accomplished by classifying PPG signals obtained from smartphones or wearable devices combined with motion-related signals obtained from accelerometers.





\subsection{Convolutional Neural Network (CNN)}

% \begin{table*}[t]
% \centering 
% \caption{Comparing the literature on in-wild eating detection to this work.}
% \begin{small}
% \begin{tabular*}{\textwidth}{p{0.5cm}p{4.5cm}p{0.5cm}p{4.8cm}cc c}
% \toprule
%     {Study} & {Architecture} & \mc{\stackon{kernel}{Conv.}} & {Activity of interest} & \mc{\stackon{classes}{Num. of}} &  {Sensors} & {Dataset} \\
%     \midrule
%     {[89]} & C-P-C-P-C-P-S & 12*2 & daily activities including brush teeth, comb hair, get up from bed, etc & 12 & S1, S2, S3 & WHARF \\
    
%     {[1]} &  &  & locomotion activities including falling, running, jumping, etc &  & S1 & self \\
% % 2014  & Fontana et al.~\cite{fontana2014automatic} & S1, S4, S6	 & Ear, wrist, chest & 12 & 24.0 &  \xmark & \cmark & \cmark\\
% % 2015& {Thomaz et al.~\cite{Thomaz2015}}&S1&Wrist&7 + 1&5.7/13.6&\xmark&\xmark&\xmark\\
% \bottomrule
% \end{tabular*}
% \end{small}
% \begin{captiontext}
% \begin{small}
% C - convolutional layer, P - max pooling layer, FC - fully connected layer, S - softmax\\
%  S1 - accelerometer, S2 - gyroscope, S3 - magnetometer, S4 - piezo, S5 - proximity, S6 - radio frequency, S7 - microphone, S8 - electromyography, S9 - light, S10 - camera
% \end{small}
% \end{captiontext}
% \label{tbl:eating_detect_table}
% \end{table*}



% \newgeometry{margin=.2cm} % modify this if you need even more space
% \begin{landscape}

% S1 - accelerometer, S2 - gyroscope, S3 - magnetometer, S4 - piezo, S5 - proximity, S6 - radio frequency, S7 - microphone, S8 - electromyography, S9 - light, S10 - camera



% \textcolor{red}{Haik: I think we should decide once again who the target audience is for this paper. Because readers unfamiliar with the material will not be able to follow your explanation: its a very complex topic to condense into three paragraphs. And those which do know, probably don't need it. So either a much more thorough explanation is needed for those with no background, or a simple sentence (with citations) will be enough, and your paper should be emphasizing the applications instead}
A CNN comprises convolutional layers that make use of the convolution operation, pooling layers, fully connected layers, and an output layer (usually Softmax layer). The convolution operation with a shared kernel enables the learning process of space invariant features. Because each filter in a convolutional layer has a defined receptive field, CNN is good at capturing local dependency, compared with a fully-connected neural network. Though each kernel in a layer covers a limited size of input neurons, by stacking multiple layers, the neurons of higher layers will cover a larger more global receptive field. The pyramid structure of CNN contributes to its capability of gathering low-level local features into high-level semantic meanings. This allows CNN to learn excellent features as shown in~\cite{cnn91}, which compares the features extracted from CNN to hand-crafted time and frequency domain features (Fast Fourier Transform and Discrete Cosine Transform).

% The mechanism of CNN resembles the biological processes of the animal visual cortex~\cite{cnn_origin}. 
% Featured by incorporating convolutional operation, CNN is composed of convolutional layers, pooling layers, fully connected layers, and a softmax layer. 
% The convolutional operation, with a shared kernel, enables the learning process of space invariant features. 
% 
% Compared with a fully-connected neural network, CNN is good at capturing local dependency since each filter in one convolutional layer has a defined receptive field. Though each kernel in a layer covers a limited size of input neurons, by stacking multiple layers, the neurons of higher layers turn to cover a large area of the reception field. 
% and with convolutional layers stacked together, the overall receptive field can be derived. 


CNN incorporates a pooling layer that follows each convolutional layer in most cases. A pooling layer compresses the representation it is learning and strengthens the model against noise by dropping a portion of the output to a convolutional layer. Generally, a few fully connected layers follow after a stack of convolutional and pooling layers that reduce feature dimensionality before being fed into the output layer. A softmax classifier is usually selected as the final output layer. However, as an exception, some studies explored the use of traditional classifiers as the output layer in a CNN~\cite{cnn11,cnn115}. 

% 
% \textcolor{red}{[91] compared hand-craft time domain and frequency domain features, Fast Fourier Transform, Discrete Cosine Transform and CNN features. They extract features from accelerometer data collected from wrist and thigh.} 


% In this part, we will exhibit different types of CNNs used for HAR and guide the introduction of existing works with a handful of research questions during this survey work. We pay special attention to questions of these aspects: 1). What format are the input data used in? 2). How many layers are used? What is the loss function? 3). What datasets are used in these work? Identify the application and categorize them.


% \begin{itemize}
%     \item $\mathsf{Q1:}$ \textbf{Input data}
% \end{itemize}

Most CNNs use univariate or multivariate sensor data as input. Besides raw or filtered sensor data, the magnitude of 3-axis acceleration is often used as input, as shown in~\cite{cnn2017bigcomp}. Researchers have tried encoding time-series data into 2D images as input into the CNN. In~\cite{cnn35}, the Short-time Fourier transform (STFT) for time-series sensor data is calculated, and its power spectrum is used as the input to a CNN. Since time series data is generally one-dimensional, most CNNs adopt 1D-CNN kernels. Works that use frequency-domain inputs (e.g., spectrogram), which have an additional frequency dimension, will generally use 2D-CNN kernels~\cite{cnn69}. The choice of 1D-CNN kernel size normally falls in the range of 1~$\times$~3 to 1~$\times$~5 (with exceptions in~\cite{cnnhar2014,cnn11,cnn12} where kernels of size 1~$\times$~8, 2~$\times$~101, and 1~$\times$~20 \mbox{are adopted). }

% 1*8: [46] An Improved Performance of Deep Learning Based on Convolution Neural Network to Classify
% 2*101: cnn-svm - [47]
% 1*20: CNN-HAR-MS - [119]

% Researchers also tried encoding time-series data into 2D images and then taking 2D images as input. % apply 2D CNN to classify human activities [105]. %They use HHAR and MHEALTH dataset. 
% In~\cite{cnn35}, since human activities differ largely among individuals, they adapt their model to each individual with a small amount of his/her data. 
% Short-time Fourier transform (STFT) for time-series sensor data is calculated in pre-processing and its power spectrum is used as an input to a CNN. 
% It inserts several hidden unit layers in the network and customized the weights using a small amount of user-dependent data. Recognition performance was improved by 3\%. 

% Novel weight sharing method in convolutional operation was also proposed. In the CNN model of [13], partial and full weight sharing, which was called CNN-pff, was used in first convolutional layer and \textbf{full weight sharing} in the second convolutional layer. The novel weight sharing method outperforms normal 1D-CNN and 2D-CNN on dataset Mhealth, which contains 3 accelerometers (chest, right wrist, left ankle) and 2 gyroscopes (right wrist, left ankle). 
% In [9], They proposed \textbf{CNN partial weight sharing} and showed it outperforms traditional CNN and traditional ML methods.

%
% In [84], they use a set of lower-dimensional filters as Lego bricks to be stacked for conventional filters, which can greatly reduce memory and computation cost over CNN, while achieving higher accuracy. 

% A public dataset (R. N. Khushaba, M. Takruri, S. Kodagoda, and G. Dissanayake, "Toward Improved Control of Prosthetic Fingers Using Surface Electromyogram (EMG) Signals", Expert Systems with Applications, vol 39, no. 12, pp.~10731–10738, 2012.) % 8-layer architecture with 4 conv layers used


% \begin{itemize}
%     \item $\mathsf{Q2:}$ \textbf{Network structure}
% \end{itemize}

To discover the relationship between the number of layers, the kernel size, and the complexity level of the tasks, we picked and summarized several typical studies in \mbox{Table \ref{tab:CNN}.}
%
A majority of the CNNs consist of five to nine layers~\cite{cnn2015smc,cnn2, cnn5, cnn11, cnn12, cnn17, cnn31,huang2021shallow,gao2021deep}, usually including two to three convolutional layers, two to three max-pooling layers, followed by one to two fully connected layers before feeding the feature representation into the output layer (softmax layer in most cases). \changezs{\citet{dong2019harnet} demonstrated performance improvements by leveraging both handcrafted time and frequency domain features along with features generated from a CNN, called HAR-Net, to classify six locomotion activities using accelerometer and gyroscope signals from a smartphone.} \citet{cnn66} used a shallow three-layer CNN network including a convolutional layer, a fully connected layer, and a softmax layer to perform on-device activity recognition on a resource-limited platform and shown its effectiveness and efficiency on public datasets. \citet{cnnhar2014} and \citet{cnn2017bigcomp} also used a small number of layers (four layers). 
% 
The choice of the loss function is an important decision in training CNNs. In classification tasks, cross-entropy is most commonly used, while in regression tasks, mean squared error is most commonly used. %~\cite{cnn11}\textcolor{red}{[X]}.
\change{Most CNN models process input data by extracting and learning channel-wise features separately while \citet{huang2021shallow} first propose a shallow CNN that considers cross-channel communication.
The channels in the same layer interact with each other to obtain discriminative features of sensor data.
}
% 
% 
% 
% In~\cite{cnnhar2014}, the authors built a 4-layer model with 1 convolutional layer, 1 pooling layer and 2 fully connected layers on three public datasets: Skoda, Opportunity, Actitracker. They proposed \textbf{CNN partial weight sharing} and showed it outperforms traditional CNN and traditional ML methods. Experiments also showed the influence of different pooling sizes, dropout, weight decay and momentum in optimization.


% \begin{minipage}
% \begin{adjustbox}{angle=90}
\begin{table}[h!]
\centering
\renewcommand\tabcolsep{4.5pt} 
\caption{\changezs{Summary of typical studies that use layer-by-layer CNN structure in HAR and their configurations. \change{We aim to present the relationship of CNN kernels, layers, and targeted problems (application and sensors)}.} Key: C---convolutional layer; P---max-pooling layer; FC---fully connected layer; S---softmax; S1---accelerometer; S2---gyroscope; S3---magnetometer; S4---EMG; S5---ECG}



\centering %% If there is a figure in wide page, please release command \centering
\begin{tabular}{ccccccc}
\toprule
\textbf{Study}    & \textbf{Architecture} & \textbf{Kernel Conv. }  & \textbf{Application}       &\textbf{ \# Classes} & \textbf{Sensors}  & \textbf{Dataset} \\ \midrule
{\cite{cnn2017bigcomp}} & C-P-FC-S    & \begin{tabular}[c]{@{}c@{}}1~$\times$~3, 1~$\times$~4,\\ 1~$\times$~5\end{tabular}  & locomotion activities     & 3 & S1   & Self     \\ \midrule
{\cite{gholamrezaii2021time}} & \change{C-P-C-P-S}  & \change{4~$\times$~4} & \change{locomotion activities}  & \change{6, 12}   & \change{S1} & \change{UCI, mHealth}   \\ \midrule
{\cite{cnnhar2014}}  & C-P-FC-FC-S & 1~$\times$~20 & \begin{tabular}[c]{@{}c@{}}daily activities,\\ locomotion activities\end{tabular}                                                   & -                          & -& \begin{tabular}[c]{@{}c@{}c@{}}Skoda, \\ Opportunity, \\ Actitracker\end{tabular}           \\ \midrule
{\cite{xu2021human}} & \change{C-P-C-P-FC-S}  & \change{5~$\times$~5} & \change{locomotion activities}  & \change{6}   & \change{S1} & \change{WISDM}   \\ \midrule
{\change{\cite{uddin2018activity}}} & \change{C-P-C-P-C-FC}   &  \change{$1\times5, 1\times9$} & \change{locomotion activities}  & \change{12}   & \change{S5} & \change{mHealth}   \\ \midrule
{\cite{cnn13}} & C-P-C-P-FC-FC-S & -               & \begin{tabular}[c]{@{}c@{}}daily activities,\\ locomotion activities\end{tabular}                    & 12      & \begin{tabular}[c]{@{}c@{}}S1, S2, S3 \\ ECG\end{tabular} & mHealth          \\ \midrule
{\cite{cnn89}} & C-P-C-P-C-P-S & 12~$\times$~2            & \begin{tabular}[c]{@{}c@{}}daily activities including \\ brush teeth, comb hair, \\ get up from bed, etc\end{tabular}               & 12                                                               & S1, S2, S3                                                                   & WHARF                                                                                \\ \midrule
{\cite{cnn2015smc}}  & C-P-C-P-C-P-S                                                                                         &   12~$\times$~2      & locomotion activities   & 8 & S1    & Self  \\ \midrule
{\cite{cnn5}}  & \begin{tabular}[c]{@{}c@{}}C-P-C-P-U-FC-S, \\ U: unification layer\end{tabular}                       & 1~$\times$~3, 1~$\times$~5        & \begin{tabular}[c]{@{}c@{}}daily activities,\\ hand gesture\end{tabular}  & \begin{tabular}[c]{@{}c@{}}18 (Opp)\\ 12 (hand)\end{tabular} & \begin{tabular}[c]{@{}c@{}}S1, S2 \\ (1 for each)\end{tabular}               & \begin{tabular}[c]{@{}c@{}}Opportunity\\ Hand Gesture\end{tabular}                   \\ \midrule
% {[}2{]}  & leave for later    &     &  & &  &   \\ \midrule
{\cite{cnn12}} & C-C-P-C-C-P-FC  & 1~$\times$~8  & hand motion classification & 10    & S4     & \begin{tabular}[c]{@{}c@{}}Rami EMG\\Dataset\end{tabular}       \\ \midrule
% {\cite{cnn11}} & C-P-C-P-FC-FC-SVM     &  &  & &     &     \\ \midrule
{\cite{cnn17}} & \begin{tabular}[c]{@{}c@{}}C-C-P-C-C-\\P-FC-FC-S \\ (one branch \\ for each sensor)\end{tabular} & 1~$\times$~5             & \begin{tabular}[c]{@{}c@{}}daily activities,\\  locomotion activities,\\  industrial ordering \\ picking recognition task\end{tabular} & \begin{tabular}[c]{@{}c@{}}18 (Opp)\\ 12 (PAMAP2)\end{tabular}   &   S1, S2, S3     & \begin{tabular}[c]{@{}@{}c@{}}Opportunity,\\PAMAP2,\\ Order Picking\end{tabular} \\ \midrule
% {[}20{]} &   &                 &   &   &   &      \\ \midrule
% {[}37{]} &   &                 &   &   &   &  \\ \midrule
{\cite{cnn35}} & \begin{tabular}[c]{@{}c@{}}C-P-C-P-C-P-\\ FC-FC-FC-S\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1~$\times$~4, 1~$\times$~10,\\ 1~$\times$~15\end{tabular}  & locomotion activities  & 6   & S1, S2, S3 & Self   \\ \midrule
\end{tabular}

\label{tab:CNN}
\end{table}
% \end{adjustbox}
% \end{landscape}
% \restoregeometry
% \end{minipage}


The number of sensors used in a HAR study can vary from a single one to as many as 23~\cite{Opportunity}. In~\cite{cnn2015smc}, a single accelerometer is used to collect data from three locations on the body: Cloth pocket, trouser pocket and waist. The authors collect data on 100 subjects, including eight activities such as falling, running, jumping, walking, walking quickly, step walking, walking upstairs, and walking downstairs. 
Moreover, HAR applications can involve multiple sensors of different types. 
To account for all these different types of sensors and activities, \citet{cnn49} proposed a multi-branch CNN architecture. 
% Thus, a variety of sensor fusion designs are proposed. Typical fusion methods include uni-branch structure [66] and multi-branch structure [49]. 
% Uni-branch structure [66] ...
A multi-branch design adopts a parallel structure that trains separate kernels for each IMU sensor and concatenates the output of branches at a late stage, after which one or more fully connected layers are applied on the flattened feature representation before feeding into the final output layer. For instance, a CNN-IMU architecture contains {m} parallel branches, one per IMU. Each branch contains seven layers, then the outputs of each branch are concatenated and fed into a fully connected and a softmax output layer.
% 
\change{\citet{GAO2021107728} has introduced a novel dual attention module including channel and temporal attention to improving the representation learning ability of a CNN model. Their method has outperformed regular CNN considerably on a number of public datasets such as PAMAP2~\cite{PAMAP2}, WISDM~\cite{WISDM}, UNIMIB SHAR~\cite{SHAR}, and Opportunity~\cite{Opportunity}.}

Another advantage of DL is that the features learned in one domain can be easily generalized or transferred to other domains. The same human activities performed by different individuals can have drastically different sensor readings. To address this challenge, \citet{cnn35} adapted their activity recognition to each individual by adding a few hidden layers and customizing the weights using a small amount of individual data. They were able to show a 3\% improvement in recognition performance.



% % 
% Opportunity dataset: gesture task - 92.4 accuracy, 92.3 weighted F1. Opportunity-Locomotion - 89.8 accuracy, 89.7 weighted F1; PAMAP2 dataset - 93.1 accuracy, 93.2 weighted F1. 
% % 
% In [1], a single accelerometer is used to collect data from 3 different body parts: cloth pocket, trouser pocket and waist. Self-collected data on 100 subjects including 8 activities such as falling, running, jumping, walking, walking quickly, step walking, walking upstairs, and walking downstairs.



% In [10], a 4-layer CNN (1 convolutional layer, 1 max pooling layer, 1 FC and 1 softmax) was constructed. Data are collected from 5 participants using one accelerometer. The input is the magnitude of the 3-axis acceleration. In the convolutional layer, 3 kernel sizes are used to extract features from the acc magnitude input signal, then the output is passed through a max pooling layers, after which they are combined into a single feature vector and sent to FC and softmax layers. 


% In [5], a 7-layer CNN, including 3 convolutional layers, 2 subsampling (pooling) layers, 1 unification layer, and 1 FC layer is proposed. 
% The kernels in the 3 convolutional layers have the size of 1*5, 1*5, and 1*3. 
% A special layer called unification layer, which is a fully-connected layer for unifying the outputs of all the sensors and followed by a ReLU layer and normalization layer, is proposed to construct the CNN for HAR. 
% On two HAR dataset Opportunity and ActRecTut, improvements have been shown over traditional approaches SVM and KNN as well as the DBN method from~\cite{DBN0}.
% \zs{In [5], a special layer called unification layer, which is a fully-connected layer for unifying the outputs of all the sensors and followed by a ReLU layer and normalization layer, is proposed to construct the CNN for HAR.}


% Besides, The authors in~\cite{rokni2018personalized} has utilized a discretization layer to reduce sensitivity of the CNN model to subtle changes and increase the robustness of the model. 



% \textcolor{orange}{for shibo summary. 1d cnn}
% In [89], 3 layers of convolutional + max pooling + softmax. the authors propose to apply 1D CNN on accelerometer data in WHARF dataset to classify human activities. 


% \textcolor{orange}{for shibo summary. 1d cnn}
% In [97], researchers use tri-axial accelerometer data from WISDM dataset and apply \textbf{1D-CNN} to classify six kinds of human daily activities. 


% \zs{doubtful}
% In [111], researchers extract features from imu and audio data and feed into 1D CNN. For imu data, they achieve 91.98\% on UCI-HAR, 67.51\% on real-world Extrasensory dataset. For audio data, they achieve 92.30\% on the DCASE 2017 dataset and 35.24\% on the Extrasensory dataset. 



% \zs{In [31], instead of end-to-end training, we incorporated greedy-wise tuning starting from (the number of layers).}

% \begin{itemize}
%     \item $\mathsf{Q3:}$ \textbf{Application and dataset}
% \end{itemize}




% Some key points for each paper: \\
% \begin{itemize}
% \item INPUT: [FAZARD] What sensors and how many sensors are used? Are the input data multi-variant time series data? For example some papers use FFT and spectragram as input data. (fazard, need to briefly mention data augmentation if used) \\

% \item ARCH: [SHIBO] How many layers are used? We can draw some conclusion about the most used number of layers. What is the loss function? (shallow or deep, wide or narrow, arch, batch norm, Resnet, combined network)\\ 

% \item DATASET: [YAXUAN] What dataset are used, did they test on public dataset?\\

% \item APPlications: [YAXUAN] Identify the application and categorize them? Like Parkinson disease or infant activity recognition\\

% \item NOTES: [ALL] Is there any interesting finding in the paper?

% \end{itemize}


% \zs{In [31], instead of end-to-end training, we incorporated \textbf{greedy-wise tuning} starting from the number of layers. Dataset: HAR smartphone dataset from the UCI repository, 94.8\% accuracy. 7-layer with 3 conv layers.} 



% Modularized deep learning blocks are introduced to HAR. 
% % 
% In~\cite{innohar}, they have used GoogLeNet’s Inception module combined with GRU layer to build a HAR model. The proposed model was tested on three public dataset (Opportunity, PAMAP2 and Smartphones datasets) and better performance (F-Score) presented.

% Loss function is an important block of deep learning network.
% With respect to loss function, cross-entropy is the most widely used loss function in classification tasks. When regression model is built, mean squared error is used [11].



% Some studies explored the use of CNN in combination with other traditional classifiers. In [115], researchers proposed to use 1D CNN as feature extractor, following a LSTM module and then an extreme learning machine (ELM) classifier and outperform 8\% by other previous work. 


% \zs{transfer learning} \\
% Transfer learning  framework.
% In [20], the authors using convolutional neural networks to build a personalized activity recognition model with minimal user supervision. Having a trained network for a group of users as the source domain, we devise a personalized model by reusing the lower layers of the network and retrained the upper layer with a few number of instances in the target domain. 
% Dataset: Sport and Daily Activity (SDA) (Altun, Barshan 2010) and WISDM. 
% We showed that using representation learning, we can reuse the general features learned from available training data and construct a personalized model with only few labeled instances.
% % 
% In~\cite{rokni2018personalized}, they validated the transferrability of the trained model by re-using the lower layers of the network and re-training upper layers with a fractional number of data in target domain. 


% In addition to the applications discuss in Section XX, there are a few innovative applications for human activity recognition using CNN. 
% % 
% In [24], accurately predicting human locomotion intent is beneficial in controlling wearable robots and in assisting humans to walk smoothly on different terrains.
% % 
% Researchers in [38], attach IMU on healthy legs for obtaining data within the early swing phase to identify the motion intention by feeding data into the CNN model. Then the model can help to adaptively calibrate the control strategy for actuating powered intelligent prosthesis in advance for both unilateral amputees and the able-bodied. The results achieve 94.15\% for the able-bodied and 89.23\% for amputees on 13 classes of motion intent.
% % 
% Moreover, researchers use Steady StateVisually Evoked Potentials (SSVEP) to extract discriminated features from real-time electroencephalographic (EEG) data through CNN, which is then utilized to control the avatar to navigate and walk in an immersive virtual environment through Brain-Computer Interface (BCI). 
% % 
% In [108], the researcher installed IMUs on the healthy leg of lower limb amputees for monitoring its locomotion state and use CNN to predict the motion intent of both unilateral amputees and the able-bodied. 
% % 
% In [90], the researchers apply 1D CNN on data from a wrist-worn tri-axial accelerometer-based food and drink intake monitoring system. 
% % 
% In [2], locomotion mode recognition can contribute to precise control of active lower-limb prostheses in different environments. The strain gauge only provides one-dimensional signals and is also used in the control strategy of the robotic prosthesis. The convolutional neural network takes the raw noisy signals as inputs. Three transtibial amputee subjects were recruited in the experiments, and three locomotion modes were recognized. 6-layer with 2 convolutional layers. %Loss function: cross-entropy, Adam optimizer










% Deep Neural Network based Human Activity Recognition for the Order Picking Process\\
 
% \zs{parallel channel for each sensor: conv + mpool + conv + mpool + fc, then stack -) fc + fc + softmax}

% In [49], a CNN architecture is proposed to analyze the order picking process utilizing HAR data. Two \textbf{data augmentation} approaches are. First, gaussian noise has been added to the sensor samples. Second, samples from a given window are resampled. The CNN architecture is as follows: parallel processing blocks are used to process the IMU data independently. Each block is processed by a temporal convolution. Each channel has two 5*1 convolutions followed by 2*1 max pooling layer. Two of these blocks are combined resulting in 4 convolution layers. Then, one fully connected layer is at the end of each processing channel. Data from each IMU channel is stacked and flows in two fully connected layer followed by softmax layer.  The dataset is comprised of two warehouses and contain recording from three people. Walking, searching, picking, scanning, info, carrying, and acknowledge. 27 sensors (gyroscope, accelerometer, and magnetometer) were used to collect the sensory samples at the rate of 100Hz.  
% The proposed CNN architecture outperformed the traditional methods, Bayes, Random Forest, Linear SVM, and recent CNNs. \\


% Interpretable and Accurate Convolutional Neural Networks for Human Activity Recognition\\

% \zs{16 + 1 layer?}\textcolor{red}{Farzad: 16 Layers (4 Conv + 4 pooling + 4 Conv + 4 pooling) + 3 Layers (fully connected) -----> 19 Layers}

% This paper [61] proposed an interpretable convolutional neural network (I-CNN) to assess sensory signal importance since all the signals obtained from different sensors are not important and some could be redundant in a specific context. This is enabled by Spatial Group Lasso (SGL). The experimental results are obtained from Opportunity dataset. I-CNN is composed of two blocks of 4 layered temporal convolutions followed by two blocks of 4-layered temporal pooling. Then it comes to sensor-signal selection imposed by SGL followed by flattening and fully connected layers. This combination of spatial and temporal convolutions will assist with feature extraction and enhance the recognition performance compared to baseline CNN. It also helps remove the uninformative and redundant signals from being fed into the classification.\\


%  Deep Learning for Human Activity Recognition: A Resource Efficient Implementation on Low-Power Devices\\

% \zs{3 layer: 1 conv + 1 fully connected + 1 softmax}

% This paper [66] proposed a deep learning network for real-time classification on HAR data for resource-limited devices like smart phones. Their architecture has been tested on 4 different datasets. The datasets are WISDM v1.1, Daphnet FoG, Skoda, and their own dataset ActiveMiles. In input data is fed to spectrogram filters which provides interpretable features in obtaining intensity variability around inertial sensory samples. The spectrograms output values are fed to temporal convolution layer, a fully connected layer, and a softmax layer. This architecture outperformed classification methods such as neural network and linear classifier with the data attributed varying between 23 and 102 features using wrapper methods. Finally, computation time on several resource-limited devices are calculated.\\


% Comparison of Feature Learning Methods for Human Activity Recognition Using Wearable Sensors\\

% % \begin{figure}[h]
% % \includegraphics[width=0.5\textwidth]{final_images/feature learning.JPG}
% % \caption{\label{fig:postprocessing}On OPPORTUNITY DATASET}
% % \end{figure}
% % \begin{figure}[h]
% % \includegraphics[width=0.5\textwidth]{final_images/featurelearning results.jpg}
% % \caption{\label{fig:postprocessing}On OPPORTUNITY DATASET}
% % \end{figure}
% % \begin{figure}[h]
% % \includegraphics[width=0.5\textwidth]{final_images/feature learning unimib shar.jpg}
% % \caption{\label{fig:postprocessing}ON UNIMIBSHAR}
% % \end{figure}
% % \begin{figure}[h]
% % \includegraphics[width=0.5\textwidth]{final_images/feature learning unimib shar results.jpg}
% % \caption{\label{fig:postprocessing}ON UNIMIBSHAR}
% % \end{figure}


% This paper [57] analyzes different feature extraction/representation approaches e.g., hand-crafted feature extraction methods, codebook, multi-layer perceptron, convolutional neural nets, recurrent neural nets - LSTM, hybrid convolutional and recurrent neural nets, and autoencoders. These approaches are implemented on Opportunity and UnimiB-SHAR datasets. The paper’s selected method is the hybrid
% CNN and LSTM model (Hybrid), with a weighted F1-score of 70.86 percent on the OPPORTUNITY dataset even with different sensor modalities with various window sizes T. Also, fusing the features learnt by hybrid method with codebook approach showed further improvement as well. \\

% Transition-Aware Detection of Modes of Locomotion and Transportation Through Hierarchical Segmentation\\

% This paper [69] proposes a platform using CNN which is trained on accelerometer and gyroscope data that is converted to 2D images to account for inter-axial dependencies and feature extraction as well as signals’ temporal characteristics. After segmentation with a sliding window of 1 min long is applied on the sensory data, segmented data is fed into a 2-D CNN network directly to extract features. In parallel, it is fed into a feature extraction section to acquire the hand-crafted features with later is fed into a DNN with 128 neurons. In order to recognize different transportation locomotion mode, the segmented data’s PSD \zs{what is pSD?} \textcolor{red}{Farzad: power spectral density (PSD).
% The PSD is used as a feature to assist with distinguishing between challenging modes of motorized transportation that do not have a clear and distinct pattern in the time domain signals. e.g., standing in bus, standing in train} will be calculated and then is fed into a DNN with 128 neurons paralleled. The output of each flow is fed into This RNN is trained on the whole training dataset and learns the temporal order of activities. This RNN contains one layer with 25 long-short-term-memory (LSTM) neurons. The results are obtained on SHL dataset. Also, they proposed a search algorithm finds the transition time for change in modes transportation locomotion which reduces complexity of the algorithms compared to naïve search.
% Results are shown in three different scenarios: 
% Scenario1: Five classes as still, walk, run, bike, and vehicle. The vehicle class contains all car, bus, train, and subway activities.
% Scenario2: Six classes including still, walk, run, bike, road, and rail. The road class contains bus and car
% activities while the rail class contains train and subway activities.
% Scenario3: Eight classes considering each activity as a separate class.\\


% \begin{figure}[h]
% \includegraphics[width=0.5\textwidth]{final_images/scenarios.JPG}
% \caption{\label{fig:postprocessing}scenario}
% \end{figure}


% Environmental Features Recognition for Lower Limb Prostheses Toward Predictive Walking\\
% Sensors: IMU + Depth camera \zs{How is IMU sensor used in the framework?}\\
% Preproccessing: point cloud after offsetting + dimension reduction + binary image generation\\
% Contribution: experimental verification for the indoor and {outdoor experiments}.\\
% Network Architecture: This convolutional neural network included an image input layer, three convolutional layers, three batch normalization layers, three Relu layers, two max-pooling layers, a fully connected layer, a softmax layer,
% and a classification layer.\\
% Dataset: their own, the training dataset included 7500 images and each
% type of environments had 1500 images\\
% Classes: up stairs, down stairs, up ramp, down ramp, and level ground
% Results: The accuracy of classification results in simulation, indoor
% experiments, and outdoor experiments was 99.3percent for
% amputees, and 98.5percent amputee.\\

% Personal Authentication and Hand Motion Recognition based on Wrist EMG
% Analysis by a Convolutional Neural Network\\

% sensor: wrist EMG\\
% sampling rate: 1 KHz\\
% Preprocessing: removing hum noise, drift noise, outliers\\
% dataset: their own (hand motion recognition(3 classes) + personal authentication(8 classes))\\
% architecture: 3 conv + 1 reshape (flatten I think) + 2 fully connected \zs{Do they have pooling layers?}\\
% Accuracy: 94.6 percent hand motion, 95 percent personal authentication\\

% Toward Minimal-Sensing Locomotion Mode Recognition for a Powered Knee-Ankle Prosthesis\\
% sensors: IMU\\
% dataset: self-collected\\
% classes\\standing, walking on level ground, walking up and down ramps, and walking up and down stairs\\
% significance:This framework would potentially lead to less frequent clinical visits needed for sensor replacement and calibrations, which may save health care costs and the prosthesis user’s time and energy. \zs{Is this a benefit of all locomotion HAR app or just this paper? Did the author do anything special to gain this benefit?} \\
% Architecture: We use a DNN with three hidden layers, a stacked hidden layer, and
% an output layer. , rectified linear unit (ReLU) activation functions, and a softmax function\\




% \vspace{50pt}







\subsection{Recurrent Neural Network (RNN)}
Initially, the idea of using temporal information was proposed in 1991~\cite{rnn4} to recognize a finger alphabet consisting of 42 symbols and in 1995~\cite{rnn21} to classify 66 different hand shapes with about 98\% accuracy. 
%%%%%%%%%%% PURE RNN
Since then, the recurrent neural network (RNN) with time series as input has been widely applied to classify human activities or estimate hand gestures~\cite{rnn35, rnn6, rnn91, rnn95, rnn96, rnn104, rnn71,alessandrini2021recurrent}. 

%%%%%%%%%%%%%% Structure of RNN
Unlike feed-forward neural networks, an RNN processes the input data in a recurrent behavior. Equivalent to a directed graph, RNN exhibits dynamic behaviors and possesses the capability of modelling temporal and sequential relationships due to a hidden layer with recurrent connections. A typical structure for an RNN is shown in Figure \ref{fig:RNN_LSTM} with the current input, $x_t$, and previous hidden state, $h_{t-1}$. The network generates the current hidden state, $h_t$, and output, $y_t$, is as follows:

\begin{equation}
\begin{array}{c}
h_{t}=\mathscrbf{F}\left(W_{h} h_{t-1} + U_{h} x_{t} + b_{h}\right) \\
y_{t}=\mathscrbf{F}\left(W_{y} h_{t} + b_{y}\right)
\end{array}
\end{equation}
where $W_{h}$, $U_{h}$, and $W_{y}$ are the weights for the hidden-to-hidden recurrent connection, input-to-hidden connection, and hidden-to-output connection, respectively. $b_h$ and $b_y$ are bias terms for the hidden and output states, respectively. Furthermore, each node is associated with an element-wise non-linearity function as an activation function $\mathscrbf{F}$ such as the sigmoid, hyperbolic tangent (tanh), or rectified linear unit (ReLU).



In addition, many researchers have undertaken extensive work to improve the performance of RNN models in the context of human activity recognition and have proposed various models based on RNNs, including Independently RNN (IndRNN)~\cite{rnn5}, Continuous Time RNN (CTRNN)~\cite{rnn17}, Personalized RNN (PerRNN)~\cite{rnn64},  Colliding Bodies Optimization RNN (CBO-RNN)~\cite{rnn58}. 
Unlike previous models with one-dimension time-series input, \citet{rnn31} builds a CNN + RNN model with stacked multisensor data in each channel for fusion before feeding into the CNN layer. 
\citet{rnn74} uses an RNN to address the domain adaptation problem caused by intra-session, sensor placement, and intra-subject variances. 



%%%%%%%%%%%%%% Structure of LSTM
HAR improves with longer context information and longer temporal intervals. However, this may result in vanishing or exploding gradient problems while backpropagating gradients~\cite{bengiogradient}.
In an effort to address these challenges, long short-term memory (LSTM)-based RNNs~\cite{LSTM}, and Gated Recurrent Units (GRUs)~\cite{GRU} are introduced to model temporal sequences and their broad dependencies. 
The GRU introduces a reset and update gate to control the flow of inputs to a cell~\cite{rnn23,rnn28, rnn61, rnn48, rnn113}.
The LSTM has been shown capable of memorizing and modelling the long-term dependency in data. Therefore, LSTMs have taken a dominant role in time-series and textual data analysis. It has made substantial contributions to human activity recognition, speech recognition, handwriting recognition, natural language processing, video analysis, etc. 
As illustrated in \mbox{Figure \ref{fig:RNN_LSTM}~\cite{rnn3}}, a LSTM cell is composed of: (1) input gate, $i_t$, for controlling flow of new information; (2)~forget gate, $f_t$, setting whether to forget content according to internal state; (3) output gate, $o_t$, controlling output information flow; (4) input modulation gate, $g_t$, as main input; (5) internal state, $c_t$, dictates cell internal recurrence; (6) hidden state, $h_t$, contains information from samples encountered within the context window previously. The relationship between these variables are listed as Equation \eqref{equ:lstm}~\cite{rnn3}. 

\begin{equation}
\left\{ 
\begin{array}{c}
i_{t}=\sigma\left(b_{i} + U_{i} x_{t} + W_{i} h_{t-1}\right) \\
f_{t}=\sigma\left(b_{f} + U_{f} x_{t} + W_{f} x_{t-1}\right) \\
o_{t}=\sigma\left(b_{o} + U_{o} x_{t} + W_{o} h_{t-1}\right) \\
g_{t}=\sigma\left(b_{g} + U_{g} x_{t} + W_{g} h_{t-1}\right) \\
c_{t}=f_{t} c_{t-1} + g_{t} i_{t} \\
h_{t}=\tanh \left(c_{t}\right) o_{t}
\end{array}
\right.
\label{equ:lstm}
\end{equation}

% \clearpage
\vspace{-6pt}
% \end{paracol}
\begin{figure}[h!]
\centering
  \includegraphics[width=.8\linewidth]{rnn_img/rnn_lstm_structure.png}
  \caption{Schematic diagram of an RNN node and LSTM cell~\cite{rnn3}. Left: RNN node where $h_{t-1}$ is the previous hidden state, $x_t$ is the current input sample data, $h_t$ is the current hidden state, $y_t$ is the current output, and $\mathscrbf{F}$ is the activation function. Right: LSTM cell with internal recurrence $c_t$ and outer recurrence $h_t$.}%
  \label{fig:RNN_LSTM}
\end{figure}
% \begin{paracol}{2}
% \linenumbers
% \switchcolumn




As shown in Figure \ref{fig:lstm}, the input time series data is segmented into windows and fed into the LSTM model. For each time step, the model computes class prediction scores, which are then merged via late-fusion and used to calculate class membership probabilities through the softmax layer. 
Previous studies have shown that LSTMs have high performance in wearable HAR~\cite{rnn61, rnn3, rnn76}.
Researchers in~\cite{hammerla2016deep} rigorously examine the impact of hyperparameters in LSTM with the fANOVA framework across three representative datasets, containing movement data captured by wearable sensors. 
The authors assessed thousands of settings with random hyperparameters and provided guidelines for practitioners seeking to apply deep learning to their own problem scenarios~\cite{hammerla2016deep}. Bidirectional LSTMs, having both past and future recurrent connections, were used in~\cite{rnn30, rnn80} to classify activities.

\vspace{-6pt}
% \end{paracol}
\begin{figure}[h!]
\centering
  \includegraphics[width=0.85\linewidth]{rnn_img/lstm.png}
  \caption{The structure of LSTM and bi-directional LSTM model~\cite{hammerla2016deep}. (\textbf{a}). LSTM network hidden layers containing LSTM cells and a final softmax layer at the top. (\textbf{b}) bi-directional LSTM network with two parallel tracks in both future (green) and past (red) directions.}
  \label{fig:lstm}
\end{figure}
% \begin{paracol}{2}
% \linenumbers
% \switchcolumn



Researchers have also explored other architectures involving LSTMs to improve benchmarks on HAR datasets. Residual networks possess the advantage that they are much easier to train as the addition operator enables gradients to pass through more directly. Residual connections do not impede gradients and could help to refine the output of layers. For example,~\cite{rnn48} proposes a harmonic loss function and~\cite{rnn16} combines LSTM with batch normalization to achieve 92\% accuracy with raw accelerometer and gyroscope data.
Ref.~\cite{lstm7} proposes a hybrid CNN and LSTM model (DeepConvLSTM) for activity recognition using multimodal wearable sensor data. DeepConvLSTM performed significantly better in distinguishing closely-related activities, such as ``Open/Close Door'' and ``Open/Close Drawer''.
Moreover, Multitask LSTM is developed in~\cite{lstm38} to first extract features with shared weight, and then classify activities and estimate intensity in separate branches. Qin \etal proposed a deep-learning algorithm that combines CNN and LSTM networks~\cite{lstm114}. They achieved 98.1\% accuracy on the SHL transportation mode classification dataset with CNN-extracted and hand-crafted features as input. Similarly, other researchers~\cite{lstm25, lstm26, lstm12, lstm133, lstm130, lstm121, lstm100, lstm64,saha2021deep} have also developed the CNN-LSTM model in various application scenarios by taking advantage of the feature extraction ability of CNN and the time-series data reasoning ability of LSTM. 
\change{Interestingly, utilizing CNN and LSTM combined model, researchers in~\cite{saha2021deep} attempt to eliminate sampling rate variability, missing data, and misaligned data timestamps with data augmentation when using multiple on-body sensors. Researchers in~\cite{mekruksavanich2021placement} explored the placement effect of motion sensors and discovered that the chest position is ideal for physical activity identification.}



\textls[-15]{Raw IMU and EMG time series data are commonly used as inputs to RNNs~\cite{rnn1, rnn26, rnn41, rnn55, rnn74, rnn121}}. A number of major datasets used to train and evaluate RNN models have been created, including the Sussex-Huawei Locomotion-Transportation (SHL)~\cite{rnn5, rnn28}, PAMAP2~\cite{rnn27, rnn31} and Opporunity\cite{rnn76}. In addition to raw time series data~\cite{rnn61}, 
Besides raw time series data, custom features are also commonly used as inputs to RNNs.~\cite{rnn23} showed that training an RNN with raw data and with simple custom features yielded similar performance for gesture recognition (96.89\% vs 93.38\%).

However, long time series may have many sources of noise and irrelevant information. 
The concept of attention mechanism was proposed in the domain of neural machine translation to address the problem of RNNs being unable to remember long-term relationships. The attention module mimics human visual attention to building direct mappings between the words/phrases that represent the same meaning in two languages. It eliminates the interference from unrelated parts of the input when predicting the output. This is similar to what we as humans perform when we translate a sentence or see a picture for the first time; we tend to focus on the most prominent and central parts of the picture. An RNN encoder attention module is centred around a vector of importance weights. The weight vector is computed with a trainable feedforward network and is combined with RNN outputs at all the time steps through the dot product. The feedforward network takes all the RNN immediate outputs as input to learn the weights for each time step. 
\cite{rnn113} utilizes attention in combination with a 1D CNN Gated Recurrent Units (GRUs), achieving HAR performances of 96.5\% ± 1.0\%, 93.1\% ± 2.2\%, and 89.3\% ± 1.3\% on Heterogeneous~\cite{Stisen}, Skoda~\cite{Skoda}, and PAMAP2~\cite{PAMAP2} datasets, respectively. 
\cite{rnn27} applies temporal attention and sensor attention into LSTM to improve the overall activity recognition accuracy by adaptively focusing on important time windows and sensor modalities.


In recent years, block-based modularized DL networks have been gaining traction. Some examples are GoogLeNet with an Inception module and Resnet with residual blocks. The HAR community is also actively exploring the application of block-based networks. In~\cite{innohar}, the authors have used GoogLeNet’s Inception module combined with a GRU layer to build a HAR model. The proposed model was showed performance improvements on three public datasets (Opportunity, PAMAP2 and Smartphones datasets). \change{\citet{qian2019novel} developed the model with $SMM_{AR}$ in a statistical module to learn all orders of moments statistics as features, LSTM in a spatial module to learn correlations among sensors placements, and LSTM + CNN in a temporal module to learn temporal sequence dependencies along the \mbox{time scale.}
}










% \textbf{Farzad's papers:} \\
% \textcolor{blue}{Orange Labs Contribution to the Sussex-Huawei Locomotion-Transportation Recognition Challenge \zs{RNN}}\\
% \textcolor{blue}{In [41], Orange Labs proposed an LSTM and GRU recurrent neural network on Sussex-Huawei Locomotion Transportation (SHL) dataset. SHL dataset is created by using multi-model smartphone sensors. This dataset contains 8 modes of transportation in real-life settings with 3 different participants which is composed of 750 h of labelled locomotion data i.e., Car (88 h), Bus (107 h), Train (115 h), Subway (89 h), Walk (127 h), Run (21 h), Bike (79 h), and still (127 h) in 2017. 
% The input data batch size is selected to include 32 observations and each observation is composed of a 2-dimensional signal \zs{which two dimensions?} of 500 time steps. The RNN network includes 2 bidirectional LSTM layers and each layer has 128 neurons. 
% The preliminary results show that the proposed method reaches the accuracy of 60.4 percent for the user transportation mode recognition by using hand validation data as testing data.}\\

\subsection{Deep Reinforcement Learning (DRL)}

AE, DBN, CNN\changezs{, and RNN} fall within the realm of supervised or unsupervised learning. Reinforcement learning is another paradigm where an agent attempts to learn optimal policies for making decisions in an environment. At each time step, the {agent} takes an {action} and then receives a {reward} from the {environment}. The {state} of the environment accordingly changes with the action made by the agent. The goal of the agent is to learn the (near) optimal policy (or probability of action, state pairs) through the interaction with the environment in order to maximize a cumulative long-term reward. The two entities---agent and environment---and the three key elements---action, state and reward---collectively form the paradigm of RL. The structure of RL is shown in Figure~\ref{fig:rl}. 

\vspace{-6pt}
\begin{figure}[h!]
\centering
  \includegraphics[width=0.7\columnwidth]{final_images/RL.png}
  \caption{A typical structure of a reinforcement learning network~\cite{rl-img}.}
  \label{fig:rl}
\end{figure}

% Arguably, supervised learning can be reduced to reinforcement learning. When viewing the classifier as an agent, the classifier giving a prediction to each sample as an action, and the evaluation of the prediction as the reward, supervised learning is transformed to be a simplified version or a specific case of reinforcement learning. 

In the domain of HAR,~\cite{rl11} uses DRL to predict arm movements with 98.33\% accuracy.
Ref. \cite{rl2}~developed a reinforcement learning model for imitating the walking pattern of a lower-limb amputee on a musculoskeletal model. The system showed 98.02\% locomotion mode recognition accuracy. Having a high locomotion recognition accuracy is critical because it helps lower-limb amputees prevent secondary impairments during rehabilitation.
In~\cite{bhat2018online}, Bhat et al. propose a HAR online learning framework that takes advantage of reinforcement learning utilizing a policy gradient algorithm for faster convergence achieving 97.7\% in recognizing six activities. 


\subsection{Generative Adversarial Network (GAN)}
\label{sec:gan}



% \begin{figure*}[H]
% \centering
% 
%   \includegraphics[width=0.8\linewidth]{final_images/GAN.png}
%   \caption{The structure of generative adversarial network}
%   \label{fig:gan}
% \end{figure*}



% \yx{new}
Originally proposed to generate credible fake images that resemble the images in the training set, %with the same statistics as the training image set, 
GAN is a type of deep generative model, which is able to create new samples after learning from real data~\cite{goodfellow2014generative}. 
It comprises two networks, the generator ($\mathbf{G}$) and the discriminator ($\mathbf{D}$), competing against each other in a zero-sum game framework as shown in Figure \ref{fig:gan}. During the training phase, the generator takes as input a random vector $\mathbf{z}$ and transforms $\mathbf{z}\in \mathbb{R^\mathbf{n}}$ to plausible synthetic samples $\mathbf{\hat{x}}$ to challenge the discriminator to differentiate between original samples $\mathbf{x}$ and fake samples $\mathbf{\hat{x}}$. In this process, the generator strives to make the output probability $\mathbf{D(G(z))}$ approach one, in contrast with the discriminator, which tries to make the function's output probability as close to zero as possible. The two adversarial rivals are optimized by finding the Nash equilibrium of the game in a zero-sum game setting, which means the adversarial rivals' gains would be maintained regardless of what strategies are selected. However, it is not theoretically guaranteed that GAN zero-sum games reach Nash Equilibria~\cite{farnia2020gans}.



GAN model has shown remarkable performance in generating synthetic data with high quality and rich details~\cite{springenberg2015unsupervised, odena2016semi}. In the field of HAR, GAN has been applied as a semi-supervised learning approach to deal with unlabeled or partially labelled data for improving performance by learning representations from the unlabeled data, which later will be utilized by the network to generalize to the unseen data distribution~\cite{shi2021gan}. 
Afterwards, GAN has shown the ability to generate balanced and realistic synthetic sensor data. 
\citet{SensoryGANs} utilized GANs with a customized network to generate synthetic data from the public HAR dataset HASC2010corpus~\cite{HASC2011corpus}. 
Similarly, \citet{gan78} assessed synthetic data with CNN or LSTM models as a generator. In two public datasets, Sussex-Huawei Locomotion (SHL) and Smoking Activity Dataset (SAD), the discriminator was built with CNN layers, and the results demonstrated synthetic data with high quality and diversity with two public datasets. Moreover, by oversampling and adding synthetic sensor data into the training, researchers augmented and alleviated the originally imbalanced training set to achieve better performance. 
In~\cite{gan26, gan69}, they generated verisimilar data of different activities, and \citet{gan27} used the Boulic kinematic model, which aims to capture the three-dimensional positioning trend to synthesize personified walking data.
%%%%%
\change{Due to the ability to generate new data, GAN has been widely applied in transfer learning in HAR to help with the dramatic performance drop when the pre-trained model are tested against unseen data from new users.
In transfer learning techniques, the learned knowledge from the source domain (subject) is transferred to the target domain to decrease the lack of performance of the models within the target domain. 
Moreover,~\cite{soleimani2021cross} is an attempt that utilized GAN to perform cross-subject transfer learning for HAR since collecting data for each new user was infeasible. 
With the same idea, cross-subject transfer learning based on GAN outperformed those without GAN on Opportunity benchmark dataset in~\cite{soleimani2021cross} and outperformed unsupervised learning on UCI and USC-HAD dataset~\cite{abedin2021guidedgan}. Even more, transfer learning under conditions of cross-body, cross-user, and cross-sensor has been demonstrated superior performance in~\cite{sanabria2021contrasgan}.}



However, much more effort is needed in generating verisimilar data to alleviate the burden and cost of collecting sufficient user data.
Additionally, it is typically challenging to obtain well-trained GAN models owing to the wide variability in amplitude, frequency, and period of the signals obtained from different types of activities.




% \end{paracol}
\begin{figure}[h!]	

\includegraphics[width=1\linewidth]{final_images/GAN.png}
\caption{The structure of generative adversarial network.}
\label{fig:gan}
\end{figure}  
% \begin{paracol}{2}
% \linenumbers
% \switchcolumn




\subsection{\change{Hybrid Models}}
\label{sec:hybrid}

\change{
As an advancement of machine learning models, researchers take advantage of different methods and propose hybrid models.
The combination of CNN and LSTM endows the model capability of extracting local features as well as long-term dependencies in sequential data, especially for HAR time series data. For example, \citet{challa2021multibranch} proposed a hybrid of CNN and bidirectional long short-term memory (BiLSTM). The accuracy on UCI-HAR, WISDM~\cite{WISDM}, and PAMAP2~\cite{PAMAP2} datasets achieved 96.37\%, 96.05\%, and 94.29\%, respectively. \citet{dua2021multi} proposed a model with CNN combined with GRU and obtained an accuracy of 96.20\%, 97.21\%, and 95.27\% on UCI-HAR, WISDM \cite{WISDM}, and PAMAP2~\cite{PAMAP2} datasets, respectively.
% 
In order to have a straightforward view of the functionality of hybrid models, we list several papers with CNN only, LSTM only, CNN + GRU, and CNN + LSTM in \mbox{Tables \ref{tab:UCI-HAR_hybrid} and  \ref{tab:PAMAP2_hybrid}}.
In addition, \citet{RL1} proposed to combine reinforcement learning and LSTM model to improve the adaptability of different kinds of sensors, including EEG (EID dataset), RFID (RSSI dataset)~\cite{yao2017compressive}, and wearable IMU (PAMAP2 dataset)~\cite{PAMAP2}.
\mbox{Ref. \cite{zhang2019know}} employed CNN for feature extraction and a reinforced selective attention model to automatically choose the most characteristic information from multiple channels.
}

\begin{table}[h!]
\centering
\renewcommand\tabcolsep{28.2pt} 
    
     \caption{\change{Comparison of models on UCI-HAR dataset.}}
    \begin{tabular}{lcc}
    \toprule
    \textbf{Model} & \textbf{F1-Score (\%) }&\textbf{ Accuracy (\%) } \\
    \midrule
    CNN~\cite{wan2020deep} &	92.93 &	92.71 \\
    Res-LSTM~\cite{zhao2018deep} & 91.50 & 91.60  \\
    Stacked-LSTM~\cite{ullah2019stacked} &	-- &	93.13 \\
    CNN-LSTM~\cite{lstm130} & -- &	92.13 \\
    Bidir-LSTM~\cite{hernandez2019human}  &	-- &	92.67 \\
    Residual-BiLSTM~\cite{zhao2018deep} &	93.5 &	93.6 \\
    LSTM-CNN~\cite{lstm25}  &	-- &	95.78 \\ 
    % Dilated-TCN &	93.8 &	93.8 \\
    CNN‑GRU~\cite{dua2021multi} &	-- & 96.20 \\
    CNN‑GRU~\cite{challa2021multibranch} &	94.54 & 94.58 \\
    CNN-LSTM~\cite{challa2021multibranch} & 94.76 & 94.80 \\
    CNN‑BiLSTM~\cite{challa2021multibranch} &	96.31 &	96.37 \\
    \bottomrule
    \end{tabular}
    \label{tab:UCI-HAR_hybrid}


\end{table}
\vspace{-9pt}
\begin{table}[h!]
\centering
    \renewcommand\tabcolsep{31.5pt} 
     \caption{\change{Comparison of models on PAMAP2 dataset.}}
    \begin{tabular}{lcc}
    \toprule
    \textbf{Model} & \textbf{F1-Score (\%)} & \textbf{Accuracy (\%)}  \\
    \midrule
    CNN\cite{wan2020deep} & 91.16 & 91.00 \\
    BiLSTM~\cite{hernandez2019human} & 89.40 & 89.52   \\
    % ARC-NET  &	90.76  &90.91 \\
    LSTM-F~\cite{hammerla2016deep}  &	 92.90  & -- \\
    COND-CNN~\cite{cheng2020real} &	--  &94.01 \\
    CNN‑GRU~\cite{dua2021multi} & 	-- & 95.27 \\
    CNN‑GRU~\cite{challa2021multibranch} &	93.16 & 93.20 \\
    CNN-LSTM~\cite{challa2021multibranch} & 92.77 & 92.81 \\
    CNN‑BiLSTM~\cite{challa2021multibranch} &	94.27  & 94.29 \\
    \bottomrule
    \end{tabular}    
    \label{tab:PAMAP2_hybrid}


\end{table}












% \subsection{\textcolor{red}{Benchmarking on Public Datasets}}
% \label{sec:Benchmark}

% \change{Traditionally, there are a large number of application scenarios and contexts, thus it is difficult to make a head-to-head performance comparison of different approaches. Owing to the popularity of public datasets in HAR field, we could possibly evaluate these different approaches easily on a standard test bed. Here we compare different DL approaches in aspect of the prediction performance with two selected public datasets - {Opportunity} and {Skoda} as shown in Figure~\ref{fig:opp_gesture_papers} and \ref{fig:skoda_papers}. As we can observe from the figure, the F1 score achieve 88\% in 2016 since the development of CNN model. Afterwards, the models combing CNN and LSTM outperform CNN only with F1 score of over 90\%. Similar trends can also be observed from the performance of Skoda dataset in Figure \ref{fig:skoda_papers}.
% }
% % \textcolor{red}{(TO CONTINUE}


% %
% \begin{figure}
% \centering
%   \includegraphics[width=0.75\columnwidth]{img/opp_gesture.pdf}
%   \caption{Performance (weighted F1-Score) comparison on Opportunity (gesture) dataset. \textcolor{red}{(NEEDS MODIFICATION)}}~\label{fig:opp_gesture_papers}
% \end{figure}
% %

% \begin{figure}
% \centering
%   \includegraphics[width=0.75\columnwidth]{img/skoda.pdf}
%   \caption{Performance (weighted F1-Score) comparison on Skoda dataset. \textcolor{red}{(NEEDS MODIFICATION)}}~\label{fig:skoda_papers}
% \end{figure}
%

\subsection{Summary and Selection of Suitable Methods }
% \textcolor{green}{Stephen - How about this?}
\label{sec:summary}

\change{
Since the last decade, DL methods have gradually dominated a number of artificial intelligence areas, including sensor-based human activity recognition, due to its automatic feature extraction capability, strong expressive power, and the high performance rendered. 
% 
When a sufficient amount of data are available, we are becoming prone to turn to DL methods. 
% 
With all these types of available DL approaches discussed above, we need to get a full understanding of the pros and cons of these approaches in order to select the appropriate approach wisely. To this end, we briefly analyze the characteristics of each approach and attempt to give readers high-level guidance on how to choose the DL approach according to the needs and requirements.} 

\change{The most salient characteristic of auto-encoder is that it does not require any annotation. Therefore, it is widely adopted in the paradigm of unsupervised learning. Due to its exceptional capability in dimension reduction and noise suppression, it is often leveraged to extract low-dimensional feature representation from raw input. However, auto-encoders may not necessarily learn the correct and relevant characteristics of the problem at hand. There is also generally little insight that can be gained for sensor-based auto-encoders, making it difficult to know which parameters to adjust during training.
% 
Deep belief networks are a generative model generally used for solving unsupervised tasks by learning low-dimensional features. Today, DBNs have been less often chosen compared with other DL approaches and are rarely used due to the tedious training process and increased training difficulty with DBN when the network goes deeper~\cite{Goodfellow-et-al-2016}.
}

\change{ 
CNN architecture is powerful to extract hierarchical features owing to its layer-by-layer hierarchical structure. 
When compared with other approaches like RNN and GAN, CNN is relatively easy to implement. 
Besides, as one of the most studied DL approaches in image processing and computer vision,  there is a large range of CNN variants existing that we can choose from to transfer to sensor-based HAR applications. 
When sensor data are represented as two-dimensional input, we can directly start with pre-trained models on a large image dataset (e.g., ImageNet) to fasten the convergence process and achieve better performance. 
% 
Therefore, adapting the CNN approach enjoys a higher degree of flexibility in the available network architecture (e.g., GoogLeNet, MobileNet, ResNet, etc) than other DL approaches.
% 
However, CNN architecture has the requirement of fixed-sized input, in contrast to RNN, which accepts flexible input size.
% 
% ... More CONS of CNN?
In addition, compared with unsupervised learning methods such as auto-encoder and DBN, a large number of annotated data are required, which usually demands expensive labelling resources and human effort to prepare the dataset. 
% 
The biggest advantage of RNN and LSTMs is that they can model time series data (nearly all sensor data) and temporal relationships very well. Additionally, RNN and LSTMs can accept flexible input data size. The factors that prevent RNN and LSTMs from becoming the de facto method in DL-based HAR is that they are difficult to train in multiple aspects. They require a long training time and are very susceptible to diminishing/exploding gradients. It is also difficult to train them to efficiently model long time series.
}

\change{
GAN, as a generative model, can be used as a data augmentation method. Because it has a strong expressive capability to learn and imitate the latent data distribution of the targeted data, it outperforms traditional data augmentation methods~\cite{parkinson_augmentation}. 
% 
Owing to its inherent data augmentation ability, GAN has the advantage of alleviating data demands at the beginning. 
%
However, GAN is often considered as hard to train because it alternatively trains a generator and a discriminator. Many variants of GAN and special training techniques have been proposed to tackle the converging issue~\cite{arjovsky2017wasserstein, gulrajani2017improved, che2016mode}.
}

\change{
Reinforcement learning is a relatively new area that is being explored for select areas in HAR, such as modelling muscle and arm movements~\cite{rl11, rl2}. Reinforcement learning is a type of unsupervised learning because it does not require explicit labels. Additionally, due to its online nature, reinforcement learning agents can be trained online while deployed in a real system. However, reinforcement learning agents are often difficult and time-consuming to train. Additionally, in the realm of DL-based HAR, the reward of the agent has to be given by a human, as in the case of~\cite{rl11,bhat2018online}. In other words, even though people do not have to give explicit labels, humans are still required to provide something akin to a label (the reward) to train the agent.
}

\change{
When starting to choose a DL approach, we have a list of factors to consider, including the complexity of the target problem, dataset size, the availability and size of annotation, data quality, available computing resource, as well as the requirement of training time. 
% 
% === complexity of targeted problem ===
Firstly, we have to evaluate and examine the problem complexity to decide upon promising venues of machine learning methods. For example, if the problem is simple enough to resolve with the provided sensor modality, it's very likely that manual feature engineering and traditional machine learning method can provide satisfying results thus no DL method is needed. 
% 
% === dataset size ===
Secondly, before we choose the routine of DL, we would like to make sure the dataset size is sufficient to support a DL method. 
The lack of a sufficiently large corpus of labelled high-quality data is a major reason why DL methods cannot produce an expected result.
Normally, when training a DL model with a limited dataset size, the model will be prone to overfitting, and the generalizability will be sacrificed, thus using a very deep network may not be a good choice. One option is to go for a shallow neural network or a traditional ML approach. Another option is to utilize specific algorithms to make the most out of the data. To be specific, data augmentation methods such as GAN can be readily implemented.
% 
% === availability and size of annotation ===
Thirdly, another determining factor is the availability and size of annotation. When there is a large corpus of unlabeled sensor data at hand, a semi-supervised learning scheme is a promising direction one could consider, which will be discussed later in this work. 
% 
% === data quality ===
Besides the availability of sensor data, the data quality also influences the network design. If the sensor is vulnerable to environmental noise, inducing a small SNR, some type of denoising structure (e.g., denoising auto-encoder) and increasing depth of the model can be considered to increase the noise-resiliency of the DL model.
% 
% === available computing resource and the requirement of training time
At last, a full evaluation of available computing resources and expected model training time cannot be more important for developers and researchers to choose a suitable DL approach.
}

\section{Challenges and Opportunities} \label{sec:challenges}
% %
% HOW TO CONSTRUCT THIS CHAPTER SURROUNDING DEEP LEARNING

Though HAR has seen rapid growth, there are still a number of challenges that, if addressed, could further improve the status quo, leading to increased adoption of novel HAR techniques in existing and future wearables. In this section, we discuss these challenges and opportunities in HAR. 
Note that the issues discussed here are applicable to general HAR, not only DL-based HAR. We look to discuss and analyze the following \change{four questions under our research question $\mathsf{Q3}$ (challenges and opportunities)}, which overlap with the \change{four major constituents} of machine learning.
%from general HAR domain, not only DL-based HAR, and we give an overview of the current methods and progress with an emphasis on DL-based solutions. 
%In accordance with the three composites in machine learning applications: data, label, and model, we formulate this section in the following three questions.

\begin{itemize}
    \item $\mathsf{Q3.1:}$ What are the challenges in data acquisition? How do we resolve them? 
    \item $\mathsf{Q3.2:}$ What are the challenges in label acquisition? What are the current methods? 
    \item $\mathsf{Q3.3:}$ What are the challenges in modeling? What are potential solutions?
    \item $\mathsf{Q3.4:}$ \change{What are the challenges in model deployment? What are potential opportunities?}
\end{itemize}


\subsection{Challenges in Data Acquisition}

Data is the cornerstone of artificial intelligence. \minorrevision{Models only perform as well as the quality of the training data. To build generalizable models, careful attention should be paid to data collection, ensuring the participants are representative of the population of interest. Moreover, determining a sufficient training dataset size is important in HAR. Currently, there is no well-defined method for determining the sample size of training data. However, showing the convergence of the error rate as a function of training data size is one approach shown by Yang \etal~\cite{voice_in_ear}. Acquiring a massive amount of high-quality data at a low cost is critical in every domain. 
% There have been extensive efforts to create public datasets in some domains, such as computer vision and natural language processing. However, 
In HAR, collecting raw data is labor-intensive considering a large number of different wearables. Therefore, proposing and developing innovative approaches to augmenting data with high quality is imperative for the growth of \mbox{HAR research.}} 
% To address this challenge, research in methods to simplify or improve HAR sensors and their robust performance in real-world scenarios are needed to enable modeling of humans in the real-world. 

\subsubsection{The Need for More Data}
\label{subsubsec:the_need_for_more_data}

\minorrevision{Data collection requires a considerable amount of effort in HAR. Particularly when researchers propose their original hardware, it is inevitable to collect data on users. 
Data augmentation is commonly used to generate synthetic training data when there is a data shortage. 
Synthetic noise is applied to real data to obtain new training samples. In general, using the dataset augmented with synthetic training samples yields higher classification accuracy when compared to using the original dataset \cite{parkinson_augmentation, lstm_augmentation, resnet_augmentation, shoes}}. %MDPI: Please confirm if this change is correct. -- It's correct. Thanks.
 Giorgi \etal augmented their dataset by varying each signal sample with translation drawn from a small uniform distribution and showed improvements in accuracy using this augmented dataset~\cite{shoes}. 
\minorrevision{
\citet{resnet_augmentation} utilized Dynamic Time Warping to augment data and tested on UCR archive~\cite{UCRArchive}.
Deep learning methods are also used to augment the datasets to improve performance~\cite{T-CGAN, SensoryGANs, SenseGen}. 
\citet{SenseGen} and \citet{SensoryGANs} employed GAN to synthesize sensor data using existing sensor data. 
\citet{T-CGAN} designed a conditional GAN-based framework to generate new irregularly-sampled time series to augment unbalanced data sets.
% To address this challenge, research is needed in quantifying the benefits of different data augmentation methods to assess their benefits and limitations as a function of different data sets.
Several works extracted 3D motion information from videos and transferred the knowledge to synthesize virtual on-body IMU sensor data~\cite{IMUTube,vid2finger}. In this way, they realized cross-modal IMU sensor data generation using traditional computer vision and graphics methods.
% 
\textbf{Opportunity:} %%%Is the bold necessary? Shibo: we regard it as necessary for easy understanding
We have listed some of the most recent works focusing on cross-modal sensor data synthesis. However, few researchers (if any) used a deep generative model to build a video-sensor multi-modal system. If we take a broader view, many works are using cross-modal deep generative models (such as GAN) in data synthesis, such as from video to audio~\cite{visual2sound}, from text to image and vice versa~\cite{imagecaptioning,text2image}. Therefore, taking advantage of the cutting-edge deep generative models may contribute to addressing the wearable sensor data scarcity issue~\cite{DeepGenAccSynth}}.
\changezs{Another avenue of research is to utilize transfer learning, borrowing well-trained models from domains with high performing classifiers (i.e., images), and adapting them using a few samples of sensor data.}

%\textcolor{red}{(Stephen, DO WE HAVE MORE THOUGHTS ABOUT THE POTENTIAL SOLUTION???)}



\subsubsection{Data Quality and Missing Data}

\minorrevision{The quality of models is highly dependent on the quality of the training data. Many real-world collection scenarios introduce different sources of noise that degrade data quality, such as electromagnetic interference or uncertainty in task scheduling for devices that perform sampling~\cite{mDebugger}.
% 
In addition to improving hardware systems, multiple algorithms have been proposed to clean or impute poor-quality data.} Data imputation is one of the most common methods to replace poor quality data or fill in missing data when sampling rates fluctuate greatly. For example, Cao \etal introduced a bi-directional recurrent neural network to impute time series data on the UCI localization dataset~\cite{NIPS_BRITS}. Luo \etal utilized a GAN to infer missing time series data~\cite{NIPS2018_GAN}. Saeed \etal proposed an adversarial autoencoder (AAE) framework to perform data imputation~\cite{autoencoder_graph}. \textbf{Opportunity:} To address this challenge, more research into automated methods for evaluating and quantifying the quality is needed to identify better, remove, and/or correct for poor quality data. \changezs{Additionally, it has been experimentally shown that deep neural networks have the ability to learn well even if trained with noisy data, given that the networks are large enough and the dataset is large enough~\cite{rolnick2017DL}. This motivates the need for HAR researchers to focus on other areas of importance, such as how to deploy larger models in real systems efficiently (Section~\ref{subsec:challenges_in_model_deployment}) and generate more data (Section~\ref{subsubsec:the_need_for_more_data}), which could potentially aid in solving this problem.}

%\textcolor{red}{(Stephen, DO WE HAVE MORE THOUGHTS ABOUT THE POTENTIAL SOLUTION???)}


\subsubsection{\changezs{Privacy Protection}}

% FULL MATERIALS: sight (vision), hearing (audition), taste (gustation), smell (olfaction) and touch (somatosensation), as well as temperature (thermoception), kinesthetic sense (proprioception), (equilibrioception), vibration (mechanoreception), etc.
%
\minorrevision{The privacy issue has become a concern among users~\cite{chen2021deep}. In general, the more inference potential a sensor has, the less willing a person is to agree to its data collection.
% 
% For example, human obtain over 70\% information from vision, meanwhile, video camera is also the most unaccepted sensor from a list of existing pervasive sensors.
%
Multiple works have proposed privacy preservation methods while classifying human activities, including the replacement auto-encoder, the guardian, estimator, and neutralizer (GEN) architecture~\cite{AE6}, and the anonymizing autoencoder~\cite{AE7}.} For example, replacement auto-encoders learn to replace features of time-series data that correspond to sensitive inferences with values that correspond to non-sensitive inferences. Ultimately, these works obfuscate features that can identify the individual while preserving features common to each activity or movement. 
% 
\changezs{
Federated learning is a trending approach to resolve privacy issues in learning problems~\cite{mothukuri2021survey, briggs2021review, sozinov2018human, Meta-HAR}. It can enable the collaborative learning of a global model without the need to expose users' raw data. 
% 
~\citet{XIAO2021107338} realized a federated averaging method combined with a perceptive extraction network to improve the performance of the federated learning system.
% 
~\citet{tu2021feddl} designed a dynamic
layer sharing scheme, which assisted the merging of local models to speed up the model convergence and achieved dynamic aggregation of models. 
% 
~\citet{bettini2021personalized} presented a personalized semi-supervised federated learning method that built a global activity model and leveraged transfer learning for user personalization.
% 
Besides,~\citet{gudur2021resource} implemented on-device federated learning using model distillation update and so-called weighted $\alpha$-updates strategies to resolve model heterogeneities on a resource-limited embedded system (Raspberry Pi), which proved its effectiveness and efficiency. 
}
% 
\textbf{Opportunity:} 
% 
\minorrevision{Blockchain is a new hot topic around the world. Blockchain, as a peer-to-peer network without the need for centralized authority, has been explored to facilitate the privacy-preserving data collection and sharing~\cite{8001731, bdiwi2018blockchain, 10.3389/fbloc.2020.497985, CHEN2021102011}.} 
% 
% \citet{CHEN2021102011} reviewed mobile crowdsourcing solutions with blockchain technology to resolve the data quality, privacy, and security issues. 
% \textcolor{red}{DEEP LEARNING} 
The combination of federated learning and blockchain is also a potential solution towards privacy protection~\cite{nguyen2021federated} and is currently still in its very early stage. 
\minorrevision{More collaboration between ubiquitous computing community and networking community should be encouraged to prosper in-depth research in novel directions.}


%===================================================================
\subsection{Challenges in Label Acquisition}

Labelled data is crucial for deep supervised learning. 
\minorrevision{
Image and audio data is generally easy to label by visual or aural confirmation. % confirming or hearing the images or audio streams, respectively. 
% However, labelling and distinguishing different types of human activities simply by looking at different time series from HAR sensors is difficult as unique patterns in raw data can be difficult to identify, especially as the number of potential confounding activities increases. 
However, labelling human activities by looking at time series from HAR sensors is difficult or even impossible.
% Therefore, ground truth acquisition for HAR sensors generally requires an extra wearable or sensing source to provide video or audio data combined with synchronization methods to align timestamps from the ground truth video/audio with the HAR sensor data. 
Therefore, label acquisition for HAR sensors generally requires additional sensing sources to provide video or audio data to determine the ground truth,
making label acquisition for HAR more labor-intensive. Moreover, accurate time synchronization between wearables and video/audio devices is challenging because different devices are equipped with independent (and often drifting) clocks. Several attempts have been made to address this issue, such as SyncWISE~\cite{SyncWISE} and~\cite{SynchronizationLex}. 
Two areas that require more research by the DL-HAR community are shortage in labelled data and difficulty in obtaining data from real-world scenarios.}
% \textcolor{red}{(Stephen,can you expand this part??).} \textcolor{green}{Stephen - Why don't we remove this? There are a bunch of subsubsections later that present opportunities.}


\subsubsection{Shortage of Labeled Data}
As annotating large quantities of data is expensive, there have been great efforts to develop various methods to reduce the need for annotation, including data augmentation, semi-supervised learning, weakly supervised learning, and active learning to overcome this challenge.
% 
Semi-supervised learning utilizes both labelled data and unlabeled data to learn more generalizable feature representations. Zeng \etal presented two semi-supervised CNN methods that utilize unlabeled data during training: The convolutional encoder-decoder and the convolutional ladder network~\cite{semi1} and showed an 18\% higher F1-score using the convolutional ladder network on the ActiTracker dataset. %They showed that the convolutional ladder network had a better classification performance, achieving 18\% F1-score improvement compared to the supervised CNN approach on ActiTracker dataset.
% 
Dmitrijs demonstrated on the SHL dataset, with a CNN and AAE architecture, that semi-supervised learning on unlabeled data could achieve high accuracy~\cite{AE422}. \changezs{Chen \etal proposed an encoder-decoder-based method that reduces distribution discrepancies between labelled and unlabeled data that arise due to differences in biology and behavior from different people while preserving the inherent similarities of different people performing the same task~\cite{chen2019people}.}
% 
%~\cite{semisupervised_DL}
%~\cite{Semiunsupervised0}
%~\cite{eatingsemisupervised2018}

% \textcolor{purple}{Self-supervised learning is another kind of semi-supervised learning. Saeed \etal designed~\cite{self-supervised}.}

% \item Active Learning
% {(b) Active Learning}
\minorrevision{Active learning is a special type of semi-supervised learning that selectively chooses unlabeled data based on an objective function that selects data with low prediction confidence for a human annotator to label. Recently, researchers have tried to combine DL approaches with active learning to benefit from establishing labels on the fly while leveraging the extraordinary classification capability of DL. Gudur \etal utilized active learning by combining a CNN with Bayesian techniques to represent model uncertainties (B-CNN)~\cite{DAL1}.
\changezs{Bettini \etal combined active learning and federated learning to proactively annotate the unlabeled sensor data and build personalized models in order to cope with data scarcity problem~\cite{bettini2021personalized}.}}
%As a specialized version of semi-supervised learning, active learning builds model using a relatively small-sized labeled dataset while implicitly takes advantage of the data distribution of unlabeled data corpus. 
%Active learning is an advanced ground-truthing technique that, based on an objective function, selectively chooses unlabeled data for a human-in-the-loop annotator to label. 
%\minorrevision{
%During training, the model generates a confidence measurement along with the class label. Samples with low prediction confidence are sent to annotators to provide labels. Recently, researchers have tried to combine DL approaches with active learning, in order to gain the benefit of establishing labels on-the-fly while leveraging the extraordinary classification capability of DL. Gudur \etal utilized active learning by combining a CNN with Bayesian techniques to represent model uncertainties (B-CNN)~\cite{DAL1}.
%\changezs{Bettini \etal combined active learning and federated learning to proactively annotate the unlabeled sensor data and build personalized models in order to cope with data scarcity problem~\cite{bettini2021personalized}.}
%}
\textbf{Opportunity:} 
Though active learning has demonstrated that fewer labels are needed to build an effective deep neural network model, 
% it is unknown if this method of working with an oracle to select the best data samples truly saves annotator time and cost. 
a real-world study with time-cost analysis would better demonstrate the benefits of active learning. Moreover, given the many existing labelled datasets, another area of opportunity is developing methods that \minorrevision{leverage characteristics of labelled datasets to generate labels for unlabeled datasets such as transfer learning or pseudo-label method~\cite{pseudolabel}.}

% \textcolor{purple}{A non-DL active learning work. Deep Active Learning~\cite{DeActive}.}

% Multi-modal active learning and active learning for personalized models are possible promising directions. 

% \subsubsection{Label Quality}
% {Weakly Supervised Learning}
% % Weakly Supervised Human Activity Recognition from Wearable Sensors by Recurrent Attention Learning
%~\cite{Weakly_Attention} He \etal 

% explored the weakly supervised dataset~\cite{Weakly_Supervised}. 

% Attention model is utilized to learn from weakly labeled data and locate the activity part. 

% Inspired by~\cite{2018learn}, which applied a attention-based CNN model on image recognition,~\cite{Attention_CNN_weaklylabel} only needs a big chunk of time series data to be labeled as if there is a specific human activity in it and does not require the location of the activity in the time series. 

% Combined with CNN extracted representative features, .....
% \end{enumerate}



\subsubsection{Issues of In-the-field Dataset}
\minorrevision{
Traditionally, HAR research has been conducted primarily in lab. Recently, HAR research has been moving towards in-field experiments. Unlike in-lab settings, where the ground truth can be captured by surveillance cameras, in-field experiments may have subjects moving around in daily life, where static camera deployment is not sufficient any more. Alharbi \etal used wearable cameras placed at the wrist, chest, and shoulder to record subject's activities as they moved around outside of a lab setting~\cite{barriers} and studied the feasibility of wearable cameras.} 
\textbf{Opportunity:} More research in leveraging human-in-the-loop to provide in-field labelling is required to generate more robust datasets for in situ activities. 
\minorrevision{Besides, one possible solution is to utilize existing in-the-field human activity video datasets and cross-modal deep generative models. If high-fidelity synthetic wearable sensor data can be generated from the available real-world video datasets (such as Stanford-ECM dataset~\cite{stanford_ecm}) or online video corpus, it may help alleviate the in-the-field data scarcity issue.} 
Additionally, there are opportunities for semi-supervised learning methods that leverage the sparse labels provided by humans-in-the-loop to generate high-quality labels for the rest of the dataset. 


% % 
% In~\cite{sensecam}, 
% In~\cite{Laput2}, the authors adopt using ...

% \subsubsection{Sensor Synchronization}
% The temporally-precise annotation of sensor data is necessary in order to build models that can passively sense and infer behavior from sensor signals. For behaviors involving limb movements, such as smoking, eating, and brushing, video-recordings from wearable cameras are increasingly being used to obtain temporally-precise ground truth labels.



%===================================================================

% \subsubsection{Transfer learning}
% As we discussed in \ref{DTL}, transfer learning 
% UnTran: Recognizing Unseen Activities with Unlabeled Data Using Transfer Learning~\cite{UnTran}
% Deep Convolutional Feature Transfer Across Mobile Activity Recognition Domains, Sensor Modalities and Locations~\cite{TL_CNN}
% Transfer Learning for sEMG Hand Gestures Recognition Using Convolutional Neural Networks~\cite{TL_CNN2}


%===================================================================
%===================================================================
\subsection{Challenges in Modeling}

\changezs{
In this section, we discuss the challenges and opportunities in the modelling process in several aspects, including data segmentation, semantically complex activity recognition, model generalizability, as well as model robustness. 
}

\subsubsection{Data Segmentation}

As discussed in~\cite{review_Plotz}, many methods segment time series using traditional static sliding window methods. A static time window may either be too large, \minorrevision{capturing more than necessary to detect certain activities, or too small and not capturing enough series to detect long movements}. Recently, researchers have been looking to segment time series data more optimally. Zhang \etal used reinforcement learning to find more optimal activity segments to boost HAR performance~\cite{RL1}. 
\change{\citet{qian2021weakly} proposed weakly-supervised sensor-based activity segmentation and recognition method.}
\textbf{Opportunity:} More experimentation and research into dynamic activity segments or methods that leverage both short term and long term features (i.e., wavelets) are needed to create robust models at all timescales. \changezs{While neural networks such as RNNs and LSTMs can model time series data with flexible time scales and automatically learn relevant features, their inherent issues such as exploding/vanishing gradients and training difficulty, make widespread adoption difficult. As such, more research into other methods that account for these issues is necessary.}
% \textcolor{red}{Shibo:FINAL THINKING TO ADD SOMETHING...}

%===================================================================
\subsubsection{Semantically Complex Activity Recognition}

\minorrevision{Current HAR methods achieve high performance for simple activities such as running. However, complex activities such as eating, which can involve a variety of movements, remain difficult.} To tackle this challenge, Kyritsis \etal break down complex gestures into a series of simpler (atomic) gestures that, when combined, form the complex gesture~\cite{eatingmicromovement2019}. Liu \etal propose a hierarchical architecture that constructs high-level human activities from low-level activities~\cite{hierarchical2016}. Peng \etal proposes AROMA, a complex human activity recognition method that leverages deep multi-task learning to learn simple activities that make up more complex \minorrevision{movements}~\cite{aroma}. \textbf{Opportunity:} Though hierarchical methods have been introduced for various complex tasks, there are still opportunities for improvements. Additionally, novel black-box approaches to complex task recognition, where individual steps in complex actions are automatically learned and accounted for rather than specifically identified or labelled by designers, have yet to be fully explored. \minorrevision{Such a paradigm is perfectly suitable for deep learning because neural networks function on a similar principle.} Besides, graph neural network can also be explored to model the hierarchical structure of simple-to-complex human activities~\cite{gnn_survey}. 

%such a paradigm has the potential to achieve higher accuracy than methods where humans identify the higher-level attributes to learn and classify, much like the relationship between deep learning (where features are automatically learned) and classical machine learning (where features are engineered).

% zero-shot learning: Attributes’ Importance for Zero-Shot Pose-Classification Based on Wearable Sensors~\cite{zsl}
% Multi-Label Zero-Shot Human Action Recognition via Joint Latent Embedding~\cite{multilabel_zsl}


%===================================================================
\subsubsection{Model Generalizability}
% Generalization in a large population
% Intraclass variance 
% Interclass similarity
% Transfer Learning:~\cite{liang2019additive}

A model has high generalizability when it performs well on data that it has never seen before. Overfitting occurs when it performs well on training data but poorly on new data. \minorrevision{Recently, many efforts have been put into improving the generalizability of models in HAR~\cite{Stisen, Heterogeneities2, Heterogeneities3}.} 
% 
\minorrevision{
Most research on generalizability in HAR has been focused on creating models that can generalize to a larger population, which often requires a large amount of data and high model complexity. In scenarios where high model complexity and data are not bottlenecks, DL-based HAR generally outperforms and generalize better than other types of methods. In scenarios where data or model complexity is limited, DL-based methods must utilize available data more efficiently or adapt to the specific scenario online.} %Creating highly generalizable models generally requires a large amount of data and high model complexity. %We would like to point out that another direction is to adaptively adjust model parameters to new users as they use the system. Rather than having a model that has many parameters and is intensive to train, we have a smaller model that adaptively adjusts to the current user using this model.
% 
For instance, Siirtola and Röning propose an online incremental learning approach that continuously adapts the model with the user's individual data as it comes in~\cite{incremental}. \change{\citet{qian2021latent} introduce Generalizable Independent Latent Excitation (GILE), which greatly enhances the cross-person generalization capability of the model.}
\changezs{\textbf{Opportunity:} \minorrevision{An avenue of generalizability that has yet to be fully explored are new training methods that can adapt and learn predictors across multiple environments, such as invariant risk minimization~\cite{arjovsky2020invariant} or federated learning methods~\cite{konevcny2015federated}.} Incorporating these areas into DL-based HAR could not only improve the generalizability of HAR models but accomplish this in a model-agnostic way.}

%\textbf{Opportunity:} However, combining incremental learning with DL in wearable HAR systems remains an open problem. \textcolor{red}{(STEPHEN, Can we expand this?)}



%===================================================================
%===================================================================https://www.overleaf.com/project/60f453deaf3de52bcfa4a172
\subsubsection{Model Robustness}
% \subsubsection{Model Reliability}
% \textcolor{red}{(One further improvement: add more related papers)}

\changezs{
A key issue that the community is paying increasing attention to is model robustness and reliability~\cite{multisensor_review, ahad2021sensor}. %That is, how to adapt the model in a dynamic environment without significant performance degradation~\cite{multisensor_review, ahad2021sensor}. 
% 
%To tackle the model robustness issue, one feasible trending method is {multi-sensory} that increases the number of sensors and improves the model reliability by introducing sensing redundancy. 
% 
%Out of the consideration of device portability and user comfort level, a single sensor is commonly desired to achieve decent recognition performance. 
% 
%However, compared with single sensor-based activity recognition, multi-sensor systems generally have higher reliability and robustness.
% 
One common way to improve robustness is to leverage the benefits of multiple types of sensors together to create {multi-sensory systems}~\cite{abedin2021attend,Physical_Activity2021,sd_multisensory,ijcai2018-859,RL1,sena2021human}.
%Nowadays, multi-sensor based HAR and sensor fusion has become a trend to improve the robustness and generalization of recognition systems~\cite{abedin2021attend,Physical_Activity2021,sd_multisensory,ijcai2018-859,RL1,sena2021human}.
% 
\citet{Physical_Activity2021} has proposed an architecture called DeepFusionHAR to incorporate the handcrafted features and deep learning extracted features from multiple sensors to detect daily life and sports activities.
% 
\citet{sd_multisensory} proposed a multi-sensory approach for basic and complex human activity recognition that uses built-in sensors from smartphones and smartwatches to classify 20 complex actions and five basic actions.
% 
\citet{ijcai2018-859} demonstrated a mobile \minorrevision{application on a multi-sensor} mobile platform for daily living activity classification using a combination of accelerometer, gyroscope, magnetometer, microphone, and GPS. 
% 
Multi-sensory networks in some cases are integrated with attention modules to learn the most representative and discriminative sensor modality to distinguish human activities~\cite{RL1}.} 
\changezs{\textbf{Opportunity:} While there are works that utilize multiple sensors to improve robustness, \minorrevision{they} require users to \minorrevision{wear} or have access to all of the sensors they utilize. An exciting new direction is to create generalized frameworks that can adaptively utilize data from whatever sensors happen to be available, such as a smart home intelligence system~\cite{xiadia2021}. \minorrevision{For this direction, deep learning methods seem more suitable than classical machine learning methods because neural networks can be more easily tuned and adapted to different domains (i.e., different sensors) than rigid classical models, just by tuning weights or by mixing and matching different layers or embeddings.} Creating such systems would not only greatly improve the practicality of HAR-based systems but would also contribute significantly to general artificial intelligence.}


% {Multi-sensor Algorithms}

% {Multi-modal Algorithms}

% Multi-modality Sensor Data Classification with Selective Attention


% {From Video to Sensor}

% IMUTube

%===================================================================

\subsection{Challenges in Model Deployment}

\label{subsec:challenges_in_model_deployment}

%\changezs{
%There are two stages in developing deep learning applications: model training and model inference.
%Deep learning model training normally take place on powerful workstations with GPUs, while model inference can be conducted on much less powerful edge devices or on cloud servers with user data uploaded to cloud.
% 
%There are three layers in an edge device-based deep learning system: hardware, library, and algorithm. At the bottom is the hardware layer.
% 
%The major computational units in hardware infrastructure include CPU, GPU, and DSP co-processors~\cite{survey_on_device_ml}. % , and other hardware accelerators
% 
%Many of modern mobile devices integrate these units in a single chip called System-On-Chips (SOCs)~\cite{aamodt2018general}.
% 
%Nowadays there are three main CPU architectures for mobile devices (e.g., smartphones and smartwatches): ARM, ARM64, and x86. 
% 
%GPU is designed to enable and accelerate the graph processing. When designing SOC GPU architectures, great efforts are paid to improve energy efficiency and area efficiency. 
% 
%DSP co-processor is designed with signal processing operation optimization to accelerate the processing speed. 
% 
% 
%On top of the hardware layer is the library layer. Some popular neural network libraries widely used in deep learning communities include TensorFlow Lite, ONNX Runtime, CMSIS NN, etc. Each of them is compatible with certain types of CPU or GPU architecture. In most cases, developers need to select a suitable machine learning library according to the platform, API language, CPU architecture, and GPU configuration. These libraries provide users with APIs to directly manipulate the hardware to perform computing.  
% 
%On top of the library layer, researchers and developers build the algorithms. When the deep learning models are deployed in real world scenarios, mobile platforms are most commonly used out of the consideration of Internet availability and latency, energy consumption of data transfer, as well as privacy concern.}

\change{\minorrevision{There are several works focusing on deploying deep-learning-based HAR on mobile platforms.}~\citet{deepx} proposes a SOC-based architecture for optimizing deep neural network inference, while~\citet{DeepEar} and \citet{MobiRNN} utilize the smartphone's digital signal processor (DSP) and mobile GPU to improve inference time and reduce power consumption.~\citet{DeepSense} propose a lightweight CNN and RNN-based system that accounts for noisy sensor readings from smartphones and automatically learns local and global features between sensor windows to improve performance.}

\change{The second class of works focus on reducing the complexity of neural networks so that they can run on resource-limited mobile platforms.~\citet{Sparsification} reduces the amount of computation required at each layer by encoding layers into a lower-dimensional space.~\citet{Binarized-BLSTM-RNN} reduces computation by utilizing binary weights rather than fixed-point or floating weights.}

\change{Emerging trends in deploying neural networks include offloading computation onto application-specific integrated circuits (ASIC) or lower power consumption microcontrollers.~\citet{bhat2019asic, wang2008asic} developed custom integrated circuits and hardware accelerators that perform the entire HAR pipeline with significantly lower power consumption than mobile or GPU-based platforms. The downside to ASICs is that they cannot be reconfigured for other types of tasks.~\citet{islam2020zygarde} present an architecture for embedded systems that dynamically schedules DNN inference tasks to improve inference time and accuracy.}

\change{\textbf{Opportunity:} Though there are works that explore the deployment of DNNs practical systems, more research is needed for society to fully benefit from the advances in DNNs for HAR. Many of the works discussed leverage a single platform (i.e., either a smartphone or ASIC), but there are still many opportunities for improving the practical use of HAR by exploring intelligent ways to partition computation across the cloud, mobile platforms, and other edge devices. DNN-based HAR systems can largely benefit by incorporating methodologies proposed by works such as~\cite{xia2021csafe, xia2019improving, godoy2018paws, nie2020spiders, nie2021spidersplus, nie2020facial, chandrasekaran2016seus, xia2018smartphone}, that carefully partition computation and data across multiple devices and the cloud.}

\change{
Lane \etal performed a small-scale exploration into the performance of DNNs for HAR applications on mobile platforms in various configurations, including utilizing the phone's CPU and DSP and offloading computation onto remote devices~\cite{lane2015mobile}.} 
\change{This work demonstrates that mobile devices running DNN inference can scale gracefully across different compute resources available to the mobile platform and also supports the need for more research into optimal strategies for partitioning DNN inference across mobile and edge systems to improve latency, reduce power consumption, and increase the complexity of the DNNs serviceable to wearable platforms.
}





% %===================================================================
% \subsubsection{Exploration of New Machine Learning Method}

% With the rapid progression of Machine Learning, researchers invest efforts to apply new models for improving performance and extending application scenarios. 
% \textcolor{red}{I added RL papers here}



% %===================================================================
% \subsection{Topics in HAR}
% \subsubsection{Sensor Fusion}
% Sensor fusion is a popular and significant topic in human activity recognition. Existing fusion paradigms are categorized into 3 classes including early fusion, middle fusion, and late fusion. 
% % 
% Early fusion is often data-level fusion, which combines multiple data resources from heterogeneous sensors and homogeneous sensors.
% % 
% Late fusion decision level.
% % 
% Middle fusion includes feature levels and ...



%===================================================================
% \subsubsection{On-device Deployment}








%===================================================================

% ===================================================================
% \subsection{Interpretability of DL Algorithms}




%\input{7-future}
\section{Conclusions} \label{sec:conclusions}

% CNN stems from CV. RNN/LSTM stems from NLP. Can we expect an algorithm that originates from sensors so that fully suits the characteristics of sensory data?

% a fairly huge amount of labeled data is desired by deep learning algorithm to achieve better performance

Human activity recognition in wearables has provided us with many conveniences and avenues to monitor and improve our life quality. AI and ML have played a vital role in enabling HAR in wearables. 
In recent years, DL has pushed the boundary of wearables-based HAR, bringing activity recognition performance to an all-time high. 
% 
\change{In this paper, we provided our answers to the three research questions we proposed in Section %MDPI: Please consider this suggested change. --Confirmed
\ref{sec:method}. We firstly gave an overall picture of the real-life applications, mainstream sensors, and popular public datasets of HAR. Then we gave a review of the advances of the deep learning approaches used in the field of wearable HAR and provided guidelines and insights about how to choose an appropriate DL approach after comparing the advantages and disadvantages of them. At last, we discussed the current road blockers in three aspects---data-wise, label-wise, and model-wise---for each of which we provide potential opportunities.
We further identify the open challenges and finally provide suggestions for future avenues of research in this field. 
% 
By categorizing and summarizing existing works that apply DL approaches to wearable sensor-based HAR, we aim to provide new engineers and researchers entering this field an overall picture of the existing research work and remaining challenges. We would also like to benefit experienced researchers by analyzing and discussing the developing trends, major barriers, cutting-edge frontiers, and potential future directions.
% By \changezs{\st{systematically}} categorizing and summarizing existing works that apply DL approaches to wearable sensors based HAR, we aim to provide new engineers and researchers entering this field an overall picture of the existing research work and remaining challenges. We would also like to benefit experienced researchers by analyzing and discussing about the developing trends, major barriers, cutting-edge frontiers, and potential future directions.
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



